Harnessing TI Feeds for Exploitation Detection

Many organizations rely on Threat Intelligence (TI) feeds to assess the risk associated with security threats. Due to the volume and heterogeneity of data, it is prohibitive to manually analyze the threat information available in different loosely structured TI feeds. Thus, there is a need to develop automated methods to vet and extract actionable information from TI feeds. To this end, we present a machine learning pipeline to automatically detect vulnerability exploitation from TI feeds. We first model threat vocabulary in loosely structured TI feeds using state-of-the-art embedding techniques (Doc2Vec and BERT) and then use it to train a supervised machine learning classifier to detect exploitation of security vulnerabilities. We use our approach to identify exploitation events in 191 different TI feeds. Our longitudinal evaluation shows that it is able to accurately identify exploitation events from TI feeds only using past data for training and even on TI feeds withheld from training. Our proposed approach is useful for a variety of downstream tasks such as data-driven vulnerability risk assessment.

==> Makefile <==
# Makefile for LaTeX files

# Original file from  http://www.acoustics.hut.fi/u/mairas/UltimateLatexMakefile
# please check http://www.takeonthecity.nl/roels-latex-makefile/ (Roel)
# current version http://gist.github.com/503886 (John)
# Copyright (c) 2009,2010 (in order of appearance):
#   Roel Meeuws <r.j.meeuws@gmail.com>
#   John Stowers <john.stowers@gmail.com>

# ChangeLog:
#
# 2010-07-01 - version 1.2.2
#   - don't loop forever if there is undefined references
#   - add forgotten gif->pdf rule
#   - make naming of VIEW* executable shell variables consistent
#   - add default target and help
#   - add wordcount target for gettin a very approximate wordcount...
# 2010-07-01 - version 1.2.1
#   - fixed bug in viewing code thanks to John Stowers
#   - fixed bug in using bash shell thanks to John Stowers
# 2009-10-07 - version 1.2
#   - Added support for vector format .svg files
#   - Added support for PGF/TikZ .tikz files which is basically a latex 
#     tikzpicture environment block in a separate file (begin and end
#     tag should be in file too!)
#   - font embedding using 'make embedpdf' although, this should not happen
#     using this makefile and xetex... 
#   - Fix of font embedding when converting .fig files. 
#   - OpenDocument Drawing file (*.odg) format supported (requires unoconv 
#     and OpenOffice.org)
#   - Remove all beamer temporary files when cleaning up
#   - Add rule for installing prerequisites 'make get-requirements' 
# 2009-07-02 - version 1.1
# 	- Added support for gnuplot .gpi files
# 	- Added support for graphviz .dot files
# 	- Added support for xfig .fig files
# 	- Fixed the handling of metapost pictures. We now support multiple figures
# 	  per metapost file 
# 	- Added Google latex makefile error detection and coloring.
# 	- Replaced manual coloring with colored print routines for better
#  	  readability and modularization
#  	- fixed rules for backup directory 
#  	- use XeTex instead of PDFLaTeX for generating pdfs for better font support
# 2009-06-11 - version 1.0
# 	- First version published.

# Copyright notice from original file:
# Copyright (c) 2005,2006 (in order of appearance):
#	Matti Airas <Matti.Airas@hut.fi>
# 	Rainer Jung
#	Antoine Chambert-Loir
#	Timo Kiravuo

# Permission is hereby granted, free of charge, to any person obtaining
# a copy of this software and associated documentation files (the
# "Software"), to deal in the Software without restriction, including
# without limitation the rights to use, copy, modify, merge, publish,
# distribute, sublicense, and/or sell copies of the Software, and to
# permit persons to whom the Software is furnished to do so, subject to
# the following conditions: 

# The above copyright notice and this permission notice shall be
# included in all copies or substantial portions of the Software. 

# THE SOFTWARE IS PROVIDED "AS IS", WITHOUT WARRANTY OF ANY KIND,
# EXPRESS OR IMPLIED, INCLUDING BUT NOT LIMITED TO THE WARRANTIES OF
# MERCHANTABILITY, FITNESS FOR A PARTICULAR PURPOSE AND NONINFRINGEMENT.
# IN NO EVENT SHALL THE AUTHORS OR COPYRIGHT HOLDERS BE LIABLE FOR ANY
# CLAIM, DAMAGES OR OTHER LIABILITY, WHETHER IN AN ACTION OF CONTRACT,
# TORT OR OTHERWISE, ARISING FROM, OUT OF OR IN CONNECTION WITH THE
# SOFTWARE OR THE USE OR OTHER DEALINGS IN THE SOFTWARE. 

#Viewers
VIEWPS	= evince
VIEWPDF = evince
VIEWDJVU= evince
VIEWDVI	= xdvi -gamma 4

#Default targets for make and view (pdf,dvi,ps,djvu)
default : pdf
view	: showpdf

################################################################################
# NO NEED TO EDIT BELOW HERE
################################################################################

#JOHN: If builds stop working then switch to xetex/xelatex
#LATEX	= xelatex -interaction=batchmode
LATEX	= latex -interaction=batchmode
BIBTEX	= bibtex
MAKEINDEX = makeindex
DVIPS	= dvips
DVIPDF  = dvipdft
MAKEDJVU= pdf2djvu -q
L2H	= mk4ht xhmlatex 
CONVERT= convert
GZIP = gzip --best
SED = sed
SHELL = /bin/bash

RERUN = "(Rerun to get (cross-references|the bars) right)"
RERUNBIB = "No file.*\.bbl|Citation.*undefined"
MAKEIDX = "^[^%]*\\makeindex"
MPRINT = "^[^%]*print"
USETHUMBS = "^[^%]*thumbpdf"
FIGDIR = generated
BACKUPDIR=backups
LTITLE = LaTeX
DATE=$(shell date +%Y-%m-%d)

COPY = if test -r $(<:%.tex=%.toc); then cp $(<:%.tex=%.toc) $(<:%.tex=%.toc.bak); fi > /dev/null
RM = rm -f
QUIET= &>/dev/null
DISPLAYERROR= || ($(call echo-error,Errors encountered:) && $(call colorize-latex-errors, $(<:%.tex=%.log)))

#&& perl -0 -ne '$$now=0;$$previous=0;@matches=/(![^.]*[.]\s*\n(?:[^l].*\n)*(l[.][0-9]+.*)\n)/g;foreach $$text (@matches) { if ($$text =~ /^l[.][0-9]+.*$$/) { $$previous = $$text } else { $$text =~ /\n(l[.][0-9]+.*)/; $$now=$$1; if ( $$previous ne  $$now ) { print "\n$$text\n" } } }' $(<:%.tex=%.log) && false )

SRC	?= $(shell egrep -l '^[^%]*\\begin\{document\}' *.tex)
DVI	:= $(SRC:%.tex=%.dvi)
PSF	:= $(SRC:%.tex=%.ps)
PSZ	:= $(SRC:%.tex=%.ps.gz)
PDF	:= $(SRC:%.tex=%.pdf)
DJVU:= $(SRC:%.tex=%.djvu)

# Terminal color definitions

ifdef NO_COLOR
tput		=
else
tput		= $(shell tput $1)
endif

black	:= $(call tput,setaf 0)
red		:= $(call tput,setaf 1)
green	:= $(call tput,setaf 2)
yellow	:= $(call tput,setaf 3)
blue	:= $(call tput,setaf 4)
magenta	:= $(call tput,setaf 5)
cyan	:= $(call tput,setaf 6)
white	:= $(call tput,setaf 7)
bold	:= $(call tput,bold)
uline	:= $(call tput,smul)
reset	:= $(call tput,sgr0)
#
#
# User-settable definitions
#
LATEX_COLOR_WARNING	?= magenta
LATEX_COLOR_ERROR	?= red
LATEX_COLOR_INFO	?= green
LATEX_COLOR_UNDERFULL	?= magenta
LATEX_COLOR_OVERFULL	?= red bold
LATEX_COLOR_PAGES	?= bold
LATEX_COLOR_BUILD	?= blue
LATEX_COLOR_GRAPHIC	?= yellow
LATEX_COLOR_DEP		?= green
LATEX_COLOR_SUCCESS	?= green bold
LATEX_COLOR_FAILURE	?= red bold
LATEX_COLOR_FILENAME?= black bold
LATEX_COLOR_PROGNAME?= black bold

# Gets the real color from a simple textual definition like those above
# $(call get-color,ALL_CAPS_COLOR_NAME)
# e.g., $(call get-color,WARNING)
get-color	= $(subst $(space),,$(foreach c,$(LATEX_COLOR_$1),$($c)))

#
# STANDARD COLORS
#
C_WARNING	:= $(call get-color,WARNING)
C_ERROR		:= $(call get-color,ERROR)
C_INFO		:= $(call get-color,INFO)
C_UNDERFULL	:= $(call get-color,UNDERFULL)
C_OVERFULL	:= $(call get-color,OVERFULL)
C_PAGES		:= $(call get-color,PAGES)
C_BUILD		:= $(call get-color,BUILD)
C_GRAPHIC	:= $(call get-color,GRAPHIC)
C_DEP		:= $(call get-color,DEP)
C_SUCCESS	:= $(call get-color,SUCCESS)
C_FAILURE	:= $(call get-color,FAILURE)
C_FILENAME  := $(call get-color,FILENAME)
C_PROGNAME  := $(call get-color,PROGNAME)
C_RESET		:= $(reset)



echo-img      = echo -e "$(C_BUILD)====> $(C_INFO)Generating figure $(C_FILENAME)$1$(C_RESET)$(if $2, | $(red)Step $2$(C_RESET),)"
echo-cpy      = echo -e "$(C_BUILD)====> $(C_INFO)Copying figure $(C_FILENAME)$1$(C_RESET)$(if $2, | $(red)Step $2$(C_RESET),)"
echo-tex-step = echo -e "$(C_BUILD)====> $(C_INFO)$1 $(C_PROGNAME)$2 $(C_RESET)| $(red)$3$(C_RESET)"
echo-gen      = echo -e "$(C_BUILD)====> $(C_INFO)Generating $1 $(C_RESET)"
echo-do       = echo -e "$(C_BUILD)====> $(C_INFO)$1 $(C_FILENAME)$(if $2,$2,)$(C_RESET)"
echo-error    = echo -e "$(C_BUILD)====> $(C_ERROR)$1 $(C_FILENAME)$(if $2,$2,)$(C_RESET)"
echo-warning  = echo -e "$(C_BUILD)====> $(C_WARNING)$1 $(C_FILENAME)$(if $2,$2,)$(C_RESET)"
echo-finish   = echo -e "$(C_BUILD)====> $(blue)Finished $(C_RESET)$1$(C_INFO)$(if $2, in $(red)$2$(blue) runs,)$(C_RESET)"



# Colorizes real, honest-to-goodness LaTeX errors that can't be overcome with
# recompilation.
#
# Note that we only ignore file not found errors for things that we know how to
# build, like graphics files.
#
# $(call colorize-latex-errors,<log file>)
define colorize-latex-errors
$(SED) \
-e '/^! LaTeX Error: File .*eps'"'"' not found\.$$/d' \
-e '/^! LaTeX Error: Cannot determine size/d' \
-e '/^! /,/^$$/{' \
-e '  H' \
-e '  /^$$/{' \
-e '    x' \
-e '    s/^.*$$/$(C_ERROR)&$(C_RESET)/' \
-e '    p' \
-e '  }' \
-e '}' \
-e 'd' \
$1
endef

define run-latex
	$(COPY) $(QUIET);\
	$(call echo-tex-step,Running,$(LTITLE),First Run);\
	$(LATEX) $< $(QUIET) $(DISPLAYERROR) ; runs=1; \
	if egrep $(MAKEIDX) $< $(QUIET);\
	then\
		$(call echo-gen,index);\
		$(MAKEINDEX) $(<:%.tex=%) $(QUIET);\
		$(COPY) $(QUIET);\
		$(call echo-tex-step,Running,$(LTITLE),Including Index);\
		$(LATEX) $< $(QUIET) $(DISPLAYERROR); let "runs=runs+1"; \
    fi;\
	bibrun=1;\
	while egrep -c $(RERUNBIB) $(<:%.tex=%.log) $(QUIET);\
	do\
		test "$$bibrun" -eq "5" && break;\
		if [ "$$bibrun" -eq "1" ];\
		then\
			$(call echo-do,Parsing Bibliography);\
			$(BIBTEX) $(<:%.tex=%) $(QUIET);\
		fi;\
		$(call echo-tex-step,Running,$(LTITLE),Applying bibliography (run $$bibrun));\
		$(COPY) $(QUIET);\
		$(LATEX) $< $(QUIET) $(DISPLAYERROR);\
		let "bibrun=bibrun+1";\
	done;\
	try=1;\
	while egrep -c $(RERUN) $(<:%.tex=%.log) $(QUIET);\
	do\
		test "$$try" -eq "5" && break;\
		$(call echo-tex-step,Running,$(LTITLE),Solving References (run $$try));\
		$(COPY) $(QUIET);\
		$(LATEX) $< $(QUIET) $(DISPLAYERROR);\
		let "try=try+1"; \
	done;\
	let "runs=runs + bibrun + try - 2";\
	if cmp -s $(<:%.tex=%.toc) $(<:%.tex=%.toc.bak) $(QUIET);\
	then\
		true;\
	else \
		if test -r $(<:%.tex=%.toc.bak); \
		then \
			$(call echo-tex-step,Running,$(LTITLE),Solving References (run $$try));\
			$(LATEX) $< $(QUIET) $(DISPLAYERROR);\
			let "runs=runs+1";\
		fi;\
	fi;\
	$(RM) $(<:%.tex=%.toc.bak) $(QUIET);\
	$(call echo-finish,$(LTITLE),$$runs);\
	$(call echo-warning,Undefined references and citations:);\
	echo -n "$(C_WARNING)" && egrep -i "(Reference|Citation).*undefined" $(<:%.tex=%.log) && echo -n -e "$(C_RESET)" || echo -e "$(C_INFO)None.$(C_RESET)";\
	true;
endef

define get_dependencies
	deps=`perl -ne '($$_)=/^[^%]*\\\(?:include|input)\{(.*?)\}/;@_=split /,/;foreach $$t (@_) {print "$$t.tex "}' $<`
endef

define get_dependent_dirs
	depdirs=`echo -n ". "; for dir in $$(for file in $$(perl -ne '($$_)=/^[^%]*\\\(?:include|input)\{(.*?)\}/;@_=split /,/;foreach $$t (@_) {print "$$t.tex "}' $<);do echo $$(dirname $$file); done | sort -u); do echo -n $$dir; echo -n " "; done`
endef

define getbibs
	bibs=`perl -ne '($$_)=/^[^%]*\\\bibliography\{(.*?)\}/;@_=split /,/;foreach $$b (@_) {print "$$b.bib "}' $< $$deps`
endef

define getepss
	epss=`perl -ne '@foo=/^[^%]*\\\(includegraphics|begin\{overpic\}|psfig|[a-zA-Z]+WallPaper\{[0-9]*\.?[0-9]*\})(\[.*?\])?\{(.*?)\}/g;if (defined($$foo[2])) { if ($$foo[2] =~ /.eps$$/) { print "$(FIGDIR)/$$foo[2]\n"; } else { print "$(FIGDIR)/$$foo[2].eps\n"; }}' $< $$deps | sort -u | sed ':begin;N;s/\n/ /;t begin'`
endef

define getpdfs
	pdfs=`perl -ne '@foo=/^[^%]*\\\(includegraphics|begin\{overpic\}|[a-zA-Z]+WallPaper\{[0-9]*\.?[0-9]*\})(\[.*?\])?\{(.*?)\}/g;if (defined($$foo[2])) { if ($$foo[2] =~ /.pdf$$/) { print "$(FIGDIR)/$$foo[2]\n"; } else { print "$(FIGDIR)/$$foo[2].pdf\n"; }}' $< $$deps | sort -u | sed ':begin;N;s/\n/ /;t begin'`
endef

define getfigdirs
	dirs="";\
	for file in $$epss $$pdfs;\
	do\
		dir=`dirname $$file`;\
		if (echo -e $$dirs | egrep -c $$dir) > /dev/null;\
		then\
			true;\
		else\
			dirs="$$dirs $$dir ";\
		fi\
	done
endef

define manconf
	mandeps=`if test -r $(basename $@).cnf ; then cat $(basename $@).cnf |tr -d '\n\r' ; fi`
endef


# $(DEP) $(EPSPICS) $(BIBFILE)
$(DVI)	: %.dvi : %.tex %.d
	@$(run-latex)


$(PSF)	: %.ps : %.dvi %.d
	@$(call echo-do,Generating,$@)
	@$(DVIPS) $< -o $@ $(QUIET)

$(PSZ) : %.ps.gz : %.ps
	@$(call echo-do,Compressing,$@)
	@$(GZIP) -c $< > $@


#JOHN: If builds stop working then switch to xetex/xelatex
#$(PDF)	: LATEX = xelatex -interaction=batchmode -file-line-error-style
#$(PDF)	: LTITLE = XeTeX
$(PDF)	: LATEX = pdflatex -interaction=batchmode -file-line-error-style
$(PDF)	: LTITLE = PDFLaTeX
$(PDF)	: %.pdf : %.tex %.d
	@$(run-latex)

$(PDF:.pdf=.embedded.pdf): $(PDF)
	@$(call echo-do,Embedding fonts,$*)
	@$(call echo-warning,This operation removes any hyperlinks in,$@)
	@$(call echo-warning,This operation may increase file size of,$@)
	@(pdftops $< $<.ps)
	@(ps2pdf -dPDFSETTINGS=/prepress $<.ps $@)
	@-rm $<.ps

$(DJVU): %.djvu : %.pdf
	@$(call echo-gen,$@)
	@($(MAKEDJVU) -o $@ $< ) $(QUIET)

# image conversion rules
generated/%.eps	: 	%.png
	@$(call echo-img,$@)
	@$(CONVERT) -compress zip $< eps3:$@ 2> /dev/null 1> /dev/null

generated/%.eps	: 	%.tiff
	@$(call echo-img,$@)
	@$(CONVERT) -compress zip $< eps3:$@ 2> /dev/null 1> /dev/null

generated/%.eps	: 	%.jpg
	@$(call echo-img,$@)
	@$(CONVERT) -compress zip $< eps3:$@ 2> /dev/null 1> /dev/null

generated/%.eps	: 	%.bmp
	@$(call echo-img,$@)
	@$(CONVERT) -compress zip $< eps3:$@ 2> /dev/null 1> /dev/null

generated/%.eps	: 	%.gif
	@$(call echo-img,$@)
	@$(CONVERT) -compress zip $< eps3:$@ 2> /dev/null 1> /dev/null

generated/%.eps	:	%.pdf
	@$(call echo-img,$@)
	@pdftops -eps -level3 $< $@ 2> /dev/null 1> /dev/null


generated/%.eps	:	%.ps
	@$(call echo-img,$@)
	@ps2eps -l -q $<
	@mv $*.eps $@ 

generated/%.eps	:	%.eps
	@$(call echo-cpy,$@)
	@cp $< $@

mpfignum = $(shell echo $1 | sed 's/.*-\([0-9]\+\)\.\(eps\|pdf\)/\1/')
# this is now done in generated dependencies file
#generated/%.eps	: $(call mpfigname,$@)
#	@$(call echo-img,$@)
#	@echo $<
#	@mpost $<
#	@mv $*.$(call mpfignum,$@) $@

generated/%.eps :	%.fig
	@$(call echo-img,$@)
	@fig2dev -L eps $< > $@ 2> /dev/null

generated/%.eps :	%.dia
	@$(call echo-img,$@)
	@dia --export=$@ --filter=eps $< 2> /dev/null 1> /dev/null

generated/%.eps : %.gpi
	@$(call echo-img,$@)
	@(echo set terminal postscript eps enhanced color; cat $<) | gnuplot > $@

generated/%.eps : %.dot
	@$(call echo-img,$@)
	@dot -Teps $< > $@

generated/%.eps : %.svg
	@$(call echo-img,$@)
	@inkscape -z --file=$< --export-eps=$@ $(QUIET)

generated/%.eps: %.tikz
	@$(call echo-img,$@)
	@tikz2pdf -o $< $(QUIET)
	@mv tikz2pdf_temp.pdf $*.pdf
	@pdftops -eps -level3 $*.pdf $@ 2> /dev/null 1> /dev/null
	@-rm $*.pdf

generated/%.eps: %.odg
	@$(call echo-img,$@)
	@unoconv -d graphics -f eps --stdout $< > $@

generated/%.pdf	:	%.pdf
	@$(call echo-cpy,$@)
	@cp $< $@

generated/%.pdf :	%.eps
	@$(call echo-img,$@)
	@epstopdf --outfile=$@ $< 2> /dev/null 1> /dev/null

generated/%.pdf :	%.fig
	@$(call echo-img,$@)
	@cd $(dir $<);fig2mpdf $(notdir $<) 2> /dev/null 1> /dev/null
	@pdftops $*.pdf $*.ps
	@ps2pdf -dPDFSETTINGS=/prepress $*.ps $*.pdf
	@-rm -rf $*.ps
	@mv $*.pdf $@

generated/%.pdf :	%.dia
	@$(call echo-img,$@,1)
	@dia --export=$(<:.dia=.eps) --filter=eps $< 2> /dev/null 1> /dev/null
	@$(call echo-img,$@,2)
	@epstopdf --outfile=$@ $(<:.dia=.eps) 2> /dev/null 1> /dev/null
	@-rm -rf $(<:.dia=.eps) &> /dev/null

generated/%.pdf :	%.ps
	@$(call echo-img,$@)
	@ps2pdf14 -dPDFSETTINGS=/prepress $< $@ 2> /dev/null 1> /dev/null

generated/%.pdf :	%.bmp
	@$(call echo-img,$@)
	@$(CONVERT) $< $@

generated/%.pdf	: 	%.gif
	@$(call echo-img,$@)
	@$(CONVERT) $< $@

generated/%.pdf :	%.png
	@$(call echo-img,$@)
	@$(CONVERT) $< $@

generated/%.pdf :	%.jpg
	@$(call echo-img,$@)
	@$(CONVERT) $< $@

generated/%.pdf :	%.tif
	@$(call echo-img,$@)
	@$(CONVERT) $< $@

generated/%.pdf :	%.tiff
	@$(call echo-img,$@)
	@$(CONVERT) $< $@

# this is now done in generated dependencies file
#generated/%.pdf	:	%.mp
#	@$(call echo-img,$@)
#	@mptopdf $< &> /dev/null
#	@rm $*.1
#	@mv $*-1.pdf $@

generated/%.pdf : %.gpi
	@$(call echo-img,$@,1)
	@(echo set terminal mp color; cat $<) | gnuplot > $(<:.gpi=.mp)
	@$(call echo-img,$@,2)
	@cd $(dir $<);mptopdf $(notdir $(<:.gpi=.mp)) &> /dev/null
	@mv $*-0.pdf $@
	@-rm -rf $(<:.gpi=.mp)* $*-*  $*.0 $*.log &> /dev/null

generated/%.pdf : %.dot
	@$(call echo-img,$@)
	@dot -Tpdf $< > $@

generated/%.pdf : %.svg
	@$(call echo-img,$@)
	@inkscape -z --file=$< --export-pdf=$@ $(QUIET)

generated/%.pdf : %.tikz
	@$(call echo-img,$@)
	@tikz2pdf -o $< $(QUIET)
	@mv tikz2pdf_temp.pdf $@

generated/%.pdf: %.odg
	@$(call echo-img,$@)
	@unoconv -d graphics -f pdf --stdout $< > $@

#generated/%.pdf : %.r
#	@$(call echo-img,$@)
#	@echo pdf(file="$$(pwd)/$@") >> /tmp/$
#	@R -slave -f $<
#	@

# This is a rule to generate a file of prerequisites for a given .tex file
%.d	: %.tex
	@$(call echo-do,Determining dependencies);\
	$(get_dependencies) ; \
	$(getbibs) ; \
	$(getepss) ; \
	$(getpdfs) ; \
	$(getfigdirs) ;\
	$(get_dependent_dirs) ;\
	$(manconf) ;\
	echo -e "$*.dvi $*.pdf $@ : $< $$deps $$bibs $$mandeps $(EXTRAS)" > $@ ; echo "" >> $@ ; \
	echo -e "$*.dvi : $$dirs $$epss" >> $@ ; echo "" >> $@ ; \
	echo -e "$*.pdf : $$dirs $$pdfs" >> $@ ; echo "" >> $@ ; \
	for file in $$epss $$pdfs; \
	do \
	    mpsrc=$$(echo $$file | sed 's/^generated\/\(.*\)-[0-9]\+.\(pdf\|eps\)/\1.mp/g'); \
		mpsrc=$$(echo $$mpsrc | grep [.]mp); \
		if [ $$mpsrc=="" ]; then continue; fi; \
		if [ -f $$mpsrc ]; \
		then \
			echo -e "$$file: $$mpsrc" >> $@; \
			echo -e "\t@\$$(call echo-img,\$$@)" >> $@; \
			if [ $${file##*.} != "pdf" ]; \
			then \
				echo -e "\t@cd \$$(dir \$$<);mpost \$$(notdir \$$<) \$$(QUIET)" >> $@; \
				echo -e "\t@mv \$$(basename \$$<).\$$(call mpfignum,\$$@) \$$@" >> $@; \
			else \
				echo -e "\t@cd \$$(dir \$$<);mptopdf \$$(notdir \$$<) &> /dev/null" >> $@; \
				echo -e "\t@mv \$$(basename \$$<)-\$$(call mpfignum,\$$@).pdf \$$@" >> $@; \
				echo -e "\t@rm -f \$$(basename \$$<).\$$(call mpfignum,\$$@) \$$<?* \$$(basename \$$<)-* \$$(basename \$$<).log mpgraph.mp" >> $@; \
			fi; \
		fi; \
	done; \
	echo "" >> $@; \
	echo -e "DEPDIRS=$$depdirs" >> $@ ; echo "" >> $@ ; \
	if [[ $$dirs != "" ]]; then\
		echo -e "$$dirs	:" >> $@ ;\
		echo -e "\t@\$$(call echo-do,Creating directory,\$$@)" >> $@ ;\
		echo -e "	@mkdir -p \$$@" >> $@ ;\
	fi


.PHONY	: all show clean ps pdf embedpdf html showps showpdf tidy verytidy clean-images pristine backup backupdir wordcount

all		: default
show	: view

viewdjvu: showdjvu
showdjvu: djvu
	@for i in $(DJVU) ; do \
		$(call echo-do, Viewing,$<: $$i); \
		$(VIEWDJVU) $$i; \
	done

viewdvi : showdvi
showdvi	: $(DVI)
	@for i in $(DVI) ; do \
		$(call echo-do, Viewing,$<: $$i); \
		$(VIEWDVI) $$i; \
	done

viewps	: showps
showps	: ps
	@for i in $(PSF) ; do \
		$(call echo-do, Viewing,$<: $$i); \
		$(VIEWPS) $$i; \
	done

viewpdf	: showpdf
showpdf	: pdf
	@for i in $(PDF) ; do \
		$(call echo-do, Viewing,$<: $$i); \
		$(VIEWPDF) $$i; \
	done

psgz: $(PSZ)

postscript: ps
ps	: $(PSF) 

pdf	: $(PDF)

embedpdf: $(PDF:.pdf=.embedded.pdf)

djvu: pdf $(DJVU)

dvi : $(DVI)

$(BACKUPDIR):
	@$(call echo-do, Creating Backup Directory)
	@mkdir -p $(BACKUPDIR)

backupdir: $(BACKUPDIR)

backup: clean backupdir
	@$(call echo-do, Backing up project)
	@export NUM=`ls backup/ | grep backup.tar.bz2 | wc -l` && tar jcvf ` echo -e "backup/backup.tar.bz2."$$NUM` `find ./ -not -type d -a -not -regex .*backup.* -a -not -regex .*svn.* | tail -n +2`


# TODO: This probably needs fixing
html: $(DEP) $(EPSPICS)
	@$(L2H) $(SRC) $(QUIET)

refresh:
	rm -rf *.d

help:
	@echo -n "Make ["
	@echo -n {view,}{pdf,dvi,ps,djvu},
	@echo -n " clean, backup, wordcount"
	@echo "]"

tidy	:
	@$(call echo-do, Cleaning up temporary files)
	@-rm -f $(DVI:%.dvi=%.bbl) $(DVI:%.dvi=%.blg) $(DVI:%.dvi=%.log) $(DVI:%.dvi=%.out) $(DVI:%.dvi=%.idx) $(DVI:%.dvi=%.ilg) $(DVI:%.dvi=%.ind) $(DVI:%.dvi=%.toc) $(DVI:%.dvi=%.d) $(DVI:%.dvi=%.nav) $(DVI:%.dvi=%.snm)

clean-images:
	@$(call echo-do, Cleaning up generated images)
	@-rm -rf $(FIGDIR)

verytidy: tidy clean-images
	@$(call echo-do, Cleaning up intermediate files)
	@for dir in $(DEPDIRS); do cd $$dir && rm -f *.log *.aux *.dvi *.bbl *.blg *.ilg *.toc *.lof *.lot *.lol *.idx *.ind *.ps *.d *.gz *fls *fdb_latexmk *.d *~ && cd - > /dev/null; done

clean:	verytidy
	@$(call echo-do, Cleaning up output files)
	@-rm -f $(DVI) $(PSF) $(PSZ) $(PDF) $(DJVU)

pristine: clean
	@$(call echo-do, Removing backups)
	@-rm -rf $(BACKUPDIR)

get-requirements:
	@$(call echo-do, Fetching required packages using apt-get)
	@sudo apt-get install imagemagick gnuplot unoconv pdf2djvu $(VIEWDJVU) $(VIEWPDF) $(VIEWPS) bash dia xfig graphviz inkscape perl gzip ps2eps psutils pdfjam pdftk ghostscript ttf-lyx

get-requirements-tex: get-requirements
	@$(call echo-do, Fetching required packages and LaTeX distribution using apt-get)
	@sudo apt-get install texlive-base texlive-xetex texlive-science texlive-publishers texlive-pstricks texlive-metapost texlive-math-extra texlive-latex-extra texlive-latex-recommended texlive-generic-recommended

wordcount: $(SRC)
	@detex $< | wc -w

-include $(SRC:.tex=.d)


==> docs/BigTableOld.tex <==
\begin{table}[!t]
\precaption
\caption{Classification accuracy results. Each tuple represents (precision, recall, F1 score). The highest accuracy tuple is highlighted in bold.}
\label{table: results}
\centering
\scalebox{0.88}{
\scriptsize
\begin{tabular}{|c|c|c|c|c|c|}
\hline
\textbf{Feature }     & \multicolumn{1}{c|}{\textbf{Feature }}             & \textbf{Naive Bayes} & \textbf{Decision Tree} & \textbf{AdaBoost}  & \textbf{Average} \\ 
\textbf{ Extraction}       & \multicolumn{1}{c|}{\textbf{ Selection}}      & \textbf{} & \textbf{} & \textbf{}  & \textbf{} \\ 
\specialrule{1.5pt}{1pt}{1pt}
\multirow{6}{*}{\makecell{Binary}}
								&100         & (0.49, 0.98, 0.65)  & (0.63, 0.37, 0.46)   & (0.61, 0.54, 0.55) & (0.57, 0.63, 0.55)\\ \cline{2-6} 
                                &300		 &(0.52, 0.98, 0.68)  &(0.82, 0.21, 0.32)		&(0.70, 0.67, 0.68) & (0.68, 0.62, 0.56)\\ \cline{2-6}
                                & 500       & (0.53, 0.98, 0.68) &(0.61, 0.82, 0.61)    & (0.72, 0.73, 0.73)  & (0.61, 0.54, 0.55)\\ \cline{2-6}
                                &1000      &(0.53, 0.97, 0.68)  & (0.61, 0.82, 0.61)& (0.72, 0.76, 0.74) & (0.62, 0.85, 0.67) \\ \cline{2-6} 
                                &   Average    &(0.53, 0.97, 0.68) & (0.61, 0.82, 0.61)  & (0.72, 0.76, 0.74) & (0.61, 0.54, 0.55) \\ \cline{2-6} \specialrule{1.25pt}{1pt}{1pt}
\multirow{3}{*}{\makecell{TF-IDF}}    
								& 100           & (0.50, 0.98, 0.66) & (0.82, 0.41, 0.54)  & (0.74, 0.60, 0.67)& (0.68, 0.66, 0.62)\\ \cline{2-6} 
                                &300		    &(0.50, 0.98, 0.66)   &(0.83, 0.36, 0.50) & (0.76, 0.73, 0.74)	& (0.70, 0.69, 0.63)\\ \cline{2-6}
                                & 500           & (0.50, 0.97, 0.66)     &(0.83, 0.36, 0.50) & (0.76, 0.74, 0.75) & ( 0.69, 0.69, 0.63)\\ \cline{2-6}
                                & 1000         & (0.50, 0.97,  0.66)  & (0.83, 0.36, 0.50) & (0.75, 0.75, 0.75) & (0.69, 0.69, 0.63) \\ \cline{2-6}
                                & Average  & (0.50, 0.98,  0.66)  & (0.83, 0.37, 0.51) & (0.75, 0.70, 0.73) & (0.69, 0.68, 0.63) \\ \cline{2-6} \specialrule{1.25pt}{1pt}{1pt}
                                
\multirow{3}{*}{\makecell{TI2vec}} 
								& 100           &  (0.57, 0.93 , 0.71)  & (0.69, 0.72, 0.70)  & (0.77, 0.76, 0.76)& (0.67, 0.80, 0.72)\\ \cline{2-6} 
								& 300           &   (0.57, 0.85, 0.68)  &  (0.67, 0.67, 0.66) &   (0.76, 0.76, 0.76) &   (0.66, 0.76, 0.70)\\ \cline{2-6}
                                & 500            & (0.60, 0.87, 0.71)  & (0.68, 0.59, 0.63) & (0.75, 0.75, 0.75) & (0.67, 0.73, 0.70)\\ \cline{2-6}
                                & 1000          & (0.63, 0.84, 0.72) & (0.63, 0.58, 0.61)  & \textbf{(0.78, 0.77, 0.78)} &(0.68, 0.73, 0.70)\\ \cline{2-6} &Average  &(0.59, 0.87, 0.71)  & (0.67, 0.64, 0.65) &   (0.77, 0.76, 0.76) & (0.67, 0.76, 0.71)\\ \cline{2-6} \specialrule{1.25pt}{1pt}{1pt}
                                
\multirow{1}{*}{\makecell{Doc2Vec }}
								& 300    & (0.61, 0.56, 0.58)  & (0.61, 0.45, 0.52)   & (0.67, 0.66, 0.66) & (0.63, 0.56, 0.59) \\
					\cline{2-6} \specialrule{1.25pt}{1pt}{1pt}		
								%\cline{2-6} %\specialrule{1.25pt}{1pt}{1pt}

\end{tabular}
\centering
	}
\postcaption	
\end{table}

==> docs/background.tex <==
\section{Related Work}
\label{sec: background}
 
There is growing interest in the research community to better understand the value of information in TI feeds. 
%
Early work focused on TI feeds that targeted specific threat niches \cite{feal2021blocklist,Sheng09phishingblacklists,Pitsillidis12spamfeeds,Ramanathan20blacklists}.
% while recent efforts seem to focus more on the extraction of Tactics, Techniques and Procedures (TTP) from TI reports \cite {rcATT, TTPDrill, ACtionMiner, Ayode et al, unfetter Insight and MITRE TRAM.}
%
%
%%
%
Phishing and spamming, for instance,  are classical themes in the realm of TI feeds~\cite{Sheng09phishingblacklists, Pitsillidis12spamfeeds,liao2016acing,bouwman2020different}.
Sheng et al. \cite{Sheng09phishingblacklists} analyzed the effectiveness of 8 different phishing URL blacklists. 
%
They found that the quality of different blacklists varies with respect to coverage and information freshness.
%
%Some offer better coverage than others while some are updated faster than others. 
%
Pitsillidis et al. \cite{Pitsillidis12spamfeeds} analyzed the effectiveness of 10 different spam feeds. 
%
They  discovered %that the quality of different spam feeds significantly varied, with 
that some low volume feeds capture the vast majority of spam domains. 
%
% They also reported biases in some feeds towards certain types of spam, suggesting their complementarity with respect to coverage. 
%
More recently, Li et al.~\cite{li19tealeaves} analyzed 47 different TI feeds including Facebook ThreatExchange, and %aligned with the above studies 
also pointed that 
%
%They also reported that 
the quantity and quality of information across different TI feeds varies substantially.
%
In conclusion, the main takeaway from prior work on empirical analysis of TI feeds is that they vary widely in terms of the quantity, quality and coverage of data \cite{tounsi2018survey}.


%%
%Prior work has investigated 

%The combination of information from different TI feeds can produce high quality data with broad coverage~\cite{helping_hands,Thomas16threatexchanges, Ramanathan20blacklists, feal2021blocklist}. % these issues.  
%

% Combining information from seemingly unrelated services can improve the overall TI feed coverage~\cite{Ramanathan20blacklists,helping_hands}.
% Ramanathan et al. \cite{Ramanathan20blacklists}, for instance, analyzed 157 different IP blacklists. 
%
% They showed that aggregating different IP blacklists can improve the overall quality of information. {Similar findings in the realm of the   COVID-19 Cyber Threat Coalition were reported} in~\cite{helping_hands}.
%%
%Thomas et al. \cite{Thomas16threatexchanges} designed and analyzed Babel threat exchange by combining abuse incident information from 6 different Google services. 
%
%They also showed that 


%%
Our work builds on prior research in this space by analyzing 191 different general purpose TI feeds. 
%
However, instead of a similar comparative analysis of different TI feeds, our main goal is to develop an automated approach to identify vulnerability exploitation events from TI feeds.  
%
% As we discuss next, vulnerability exploitation is particularly useful in risk-aware patch management. 

 
Different sources of information can be used for predicting various states in a vulnerability's lifecycle, such as discovery, weaponization, exploitation, reporting and patching~\cite{householder2020historical,yin2022vulnerability,Sabottke15exploitsocial,Almukaynizi17identificationexploits,Wang17patchingICs,Almukaynizi19predictexploit}.
%
%
{Models for vulnerability lifecycles  are instrumental to parametrize CVSS/EPSS~\cite{varela2022feature,fuhrmann2022cyber}.  Whereas  CVSS/EPSS are vulnerability-oriented, requiring a CVE ID to assess its exploitability/risk~\cite{shahid2021cvss}, our work is TI event-oriented. Our work (1) aims at determining if a given event corresponds to an exploitation event, (2) is event-driven, leveraging the description of security incidents for that matter, and (3) relies on a dataset in which very few incidents explicitly refer to  CVE IDs. 
TIBERT's detection of exploitation events in the wild essentially provides the ground truth for EPSS scores. 
} 

%%
Sabottke et al. \cite{Sabottke15exploitsocial} and Suciu et al.~\cite{suciu2021expected} showed that  social media data can be leveraged to detect vulnerability exploits in the wild. 
%
They trained a machine learning classifier using keyword and other metadata features to detect proof-of-concept and real-world exploits. 
%
Complementary to those works, Almukaynizi et al.~\cite{Almukaynizi17identificationexploits,Almukaynizi19predictexploit} showed that data from darknet web forums and other traditional sources can be combined to detect vulnerability exploitation.
%
They trained various machine learning classifiers to predict the likelihood of vulnerability exploitation.
%
%Wang et al. \cite{Wang17patchingICs} used the TI feed from Shodan to measure patch deployment in the wild. 
%
%Xiao et al. \cite{Xiao18discoverexploit} later combined information from spam TI feeds with patch deployment measurements to detect vulnerability exploitation in the wild. 
%
%They showed that combining threat information and patching measurements can enable early detection of vulnerability exploits. 
%
%Zhu et al. \cite{Zhu18chainsmith} trained a machine learning classifier to detect  malware campaign stages (e.g., baiting, installation) using TI feeds. 



%Despite the fact that most TI feed events are not matched against CVE ids, we envision that it is possible to establish such matching, in retrospect, for a fraction of the events.  In that case, the methodology introduced in our work, to classify events, is instrumental to build ground-truth for EPSS and to parametrize CVSS temporal scores that capture exploit maturity.


%%
Our work is similar in spirit to this line of research on training  classifiers to predict different stages of a vulnerability's lifecycle.
%
Differently from prior work, we focus on training machine learning models to specifically detect instances of vulnerability exploitation from  loosely structured TI feeds.


\begin{comment}

\subsection{Attack embeddings}
Another related line of research focuses on building novel attack representations 
\cite{Mezzour14threatdescriptions,Tavabi18darkembed,shen2019attack2vec,sleeman2020temporal,Fang20fastembed}.
The challenges of this endeavour stem from  threat feeds containing information that is inconsistently structured and organized in fields that may differ  across  organizations. Indeed, those aspects together with the fact that a significant portion of the data is made available within free-form text fields  make it  difficult to process TI feeds automatically.




%
Mezzour et al. \cite{Mezzour14threatdescriptions} analyzed two Symantec threat feeds using keyword analysis to identify attack and family names.
%
Recent work has focused on learning purpose-built representations (or embeddings) for various downstream tasks. 
%
Tavabi et al. \cite{Tavabi18darkembed} trained a paragraph embedding to predict whether a vulnerability discussed on darknet web forums will be exploited. 
%
Shen et al. \cite{shen2019attack2vec} trained temporal word embeddings to detect different steps in complex attacks.
%
Fang et al.~\cite{Fang20fastembed} used a pre-trained fastText  embedding for exploit prediction, whereas Perry et al.~\cite{perry2019no} proposed a novel embedding for identifying the entity responsible for an attack.




%%
Our work builds on this line of research by evaluating keywords and embeddings to detect vulnerability exploitation from TI feeds. In addition, we conform to temporal constraints while evaluating the considered classifiers, and assess how knowledge transfer relates to the natural flow of information across TI feeds.

%
% Our results show that customized word embeddings outperform simple keyword approaches and pre-trained word embeddings. 


\end{comment}



%\subsection{Background}
%We introduce basic terminology used throughout this work.  A \textbf{TI feed} is a collection of events.  Each feed is maintained by a \textbf{provider}, and is fed by multiple  \textbf{organizations}, each of  which may be a non-profit, government or private organization.  Examples of providers include CERT-bund and CIRCL.  The list of default MISP feeds, for instance, comprises 35 feeds, and is fed by a number of different organizations. In this work, we use data provided by 191 organizations.  In the remainder of this work, we map each organization to a separate feed, comprising a total of 191 TI feeds, and allowing us to refer to providers, organizations and TI feeds interchangeably. 
%An \textbf{event} comprises a set of attributes, and each \textbf{attribute} is associated to a value. When the value serves to detect compromise of a system, it is referred to as \textbf{indicator of compromise} (IoC).

%In addition to general attributes, one can also  add \textbf{tags} to the events.   Tags must follow taxonomies, and one of such tags  is referred to as the traffic light protocol (tlp) tag. %The pair of an attribute and a value is referred to as a \textbf{tag}.  
%In this work, we share information tagged as  \textbf{tlp:white}, i.e., information that  can be  shared with the general public.  However, we   refrain to disclose the  attribution of organizations (sources) that reported the events, and anonymize the organization names for that matter.  




\begin{comment}

Many organizations use threat intelligence (TI) feeds to assist in data-driven risk assessment of cyber threats \cite{bromiley2016threat}.
%
A TI feed is a general term used to describe a curated source of information such as IP addresses, file hashes, textual threat description, and other indicating features of existing and potential cyber threats. 
%
All these features are collectively referred to as \textit{Indicators of Compromise} or ``IOCs.''
% 
TI feeds can be sourced from both public and private entities. 
%
\InnoTecSystem \cite{InnoTec} is a private TI feed organization while \CIRCL (Computer Incident Response Center Luxembourg) \cite{\CIRCL} is run by a government organization. 
%
%In our data we use both public and private TI feeds.
%Payment is irrelevant maybe remove unless can support benefit of paid or unpaid

%quantify costs of TI feeds and compare paid vs free 
%Establish payment of threat feeds is non-trivial
%%

There are two key challenges in effectively leveraging threat information from various TI feeds.


\begin{enumerate}

\item \textbf{Data quantity.}
As the role TI feeds play in cybersecurity increases, more threat data is being collected from a variety of sources.
%
New IOCs are found and regularly published, sometimes in excess of millions per day.
%
As volume increases, there is a growing need to sift through this information. 
%
However, sifting through many millions of IOCs for what is useful and what is useless is infeasible.
%
There is simply far too much data for human analysis \cite{trost2014threat}.


\item \textbf{Data quality.}
Organizations risk spending valuable resources on poor quality TI feeds, where the quantity of information is increasing faster then the capability to validate the quality of the collected information \cite{tounsi2018survey}.
%
For TI feeds to be useful, they must contain credible and actionable data about real-world cybersecurity threats. 

\end{enumerate}


%%
Thus, the usefulness of a TI feed is a function of both quantity and quality of data. \cite{tounsi2018survey}
%
In a recent study, Li et al. \cite{tealeaves} reported that the quantity of information in TI feeds varies by several orders of magnitude.
%
They also showed that the quality of information in TI feeds also varies widely and that data was often ambiguously labeled or unlabeled altogether.
%
%Furthermore, in the same study it was found that some data such as IP addresses have little to no overlap, making it difficult to find relationships or generalizations with the data.  
%
Due to large variations in data quantity and quality across different TI feeds, it is imperative to develop automated methods to systematically sift through TI feeds to identify credible and actionable information about real-world cybersecurity threats. In order to accomplish this the data used to develop this automated system should reflect the diversity of data found from TI feeds. 


\end{comment}




==> docs/conclusion.tex <==
\section{Conclusion \& Future Work}
\label{sec:conclusion}


%The machine learning approaches considered in this paper show promise for  automated  analysis of loosely structured information in TI feeds.
% In particular, we demonstrate the utility of our purpose-built TI2Vec word embedding in accurately detecting vulnerability exploitation events from TI feeds. 
We proposed a machine learning pipeline for automated analysis of loosely structured information in TI feeds. 
%
Then, aiming towards detecting vulnerability exploitation events from TI feeds, we proposed  TIBERT, that can be used to  automatically update CVSS/EPSS scores by leveraging rich temporal data from TI feeds. This paves the way toward improving the quality of CVSS/EPSS scores with minimal effort from security experts~\cite{jacobs2021exploit}.
%%
We envision that our work opens up a number of  opportunities for future research.  In particular,  %  enhanced embeddings may  further increase the accuracy of the considered classifiers.  
%
%For example, there is opportunity to fine-tune a pre-trained embedding for specific tasks in a supervised or semi-supervised manner. 
%
%As another example, 
there is opportunity to train the considered  embeddings on a larger corpus of threat information  to improve their coverage and diversity of vocabulary. 
As another direction for future work, our machine learning pipeline can be readily adapted to detect other relevant vulnerability lifecycle events, e.g., related to  increase in    weaponization maturity.
%to track vulnerability exploitation in the wild from a variety of measurement sources beyond TI feeds.

%  not only from TI feeds but also online and darknet forums \cite{Almukaynizi17identificationexploits,Almukaynizi19predictexploit}, relevant blogs~\cite{liao2016acing} and social media posts~\cite{Sabottke15exploitsocial}, and even research literature~\cite{zhu2016featuresmith}







%Fifth, there are opportunities to re-purpose our proposed machine learning pipeline in other downstream security tasks such as risk-aware patch management. 
%Specifically, the exploitation events detected from TI feeds can be incorporated in alternative data-driven risk assessment and decision making models.  
%

%%
%While we cannot share TI feeds due to licensing restrictions, 
%To foster follow-up research, we plan to openly release all code as well as trained embeddings and machine learning models.

%to foster followup research on automated analysis of TI feeds.




%\noindent \textbf{Limitations.}
%- ``truly generalize'' cross-time, cross-feed evaluation
%- Statement about njrat and darkcomet: that’s an interesting insight, but it’s also biased by the choice of feeds (e.g. containing more malware blacklist feeds than, let’s say, manually-handled incident reports) and by the timeframe considered (same feeds 5 years before would have probably returned a different malware that was “hotter” back then ��)… I think this is an interesting consideration for the results


% such as web crawls of open and darknet forums \cite{Tavabi18darkembed,Almukaynizi19predictexploit} as well as social media \cite{Sabottke15exploitsocial}

%Zubair: see if you can highlight that the embedding is useful in other downstream security tasks

%- future ML/NLP refinements: 
%fine-tune a pre-trained embedding
%supervised fine-tuning








%We believe this is a first step towards a deeper understanding on how exploitation events can be tracked in the wild.  
%As next steps in this endeavor, we envision to  analyze textual information from black hat forums and, more broadly, from large scale Internet measurements,  through  the lenses of the  {TI2vec} embedding produced in this work.
%



%The volume of TI feeds and their unstructured nature render them unwieldy for manually sift, calling for automated methods to extract actionable exploitation information.     
%As much as standardization is desired, and sometimes partially imposed within the individual communities, different groups may have different goals and thus different requirements about the intelligence to be shared among participants.  
%In the foreseen horizon, TI feeds will continue to organically grow with research opportunities related to their measurement, analysis and characterization.  


% with respect to measurements posing their own challenges  

%It is also common for each participant to use its own structure and taxonomies to store and label the intel it shares. 


% rapm crucial pieces of puzzle -- exploitation -- tweaking cvss scores

%
%
% rapm whether knowing or not occured is useful
%

%
%
% more threats, more organizatoins, less structure, near future we do not expect to have structure
%
%
% first step -- solution that needs to be continuously refined in the  
%
%
%
% all code will be available -- reproducible -- brief paper
%
% feeds are not open source -- data is sensitive and proprietry 
%
% names of sources are anonymized because they are proprietary 
%
%
%
%
% send message to Sami
%
%

==> docs/danielcomments.tex <==
restate the challenges, the goal and problem statement

connect with sectoin 3 --highlighted secton 3

big volume
need for automated methods
cannot sift through it


===> 

rapm crucial pieces of puzzle -- exploitation -- tweaking cvss scores


==


move attack embeddings to methodology

last paragraph from section 2

===

section 4

TI2vec must be emphasized

attack2vec -- main contribution

general purpose -- exploitation prediction -- can be repurposed for other security tasks -- ti2vec piece is reusable

===


restate the challenges, the goal and problem statement

connect with sectoin 3 --highlighted secton 3

big volume
need for automated methods
cannot sift through it


===> 

rapm crucial pieces of puzzle -- exploitation -- tweaking cvss scores


==


move attack embeddings to methodology

last paragraph from section 2

===



==> docs/data.tex <==
\section{TI Feed Characterization}
\label{sec: data}


\textbf{Basics.}
A TI feed is a general term used to describe a curated source of information such as IP addresses, file hashes, textual threat description, and other indicating features of existing and potential threats. 
%
All these features are collectively referred to as \textit{Indicators of Compromise} (or IoCs).
%
Each TI feed, from a public or private provider, contains a list of \textit{events}.
%
An event could be a security incident such as a phishing attack or a botnet attack, or a security advisory regarding a software vulnerability. 
%
Each event is timestamped and usually includes a short textual description about what occurred.
%
Each event further includes a collection IoCs that are individually timestamped based on when the IoCs are added or updated.
%
Further, each IoC pertains to a data type such as network activity, payload delivery, and external analysis.
%
It is noteworthy that different TI feeds may follow different naming conventions and use different languages in describing IoCs. 



%%Enrico comment (data model)
%While the description is rather generic, beware that what you are describing here is the MISP data model... other sources may use different artifacts and data models... however, the way you describe it can be interpreted as you defining your own concepts, so I guess it's fine...

%%enrico.lovat: VERY IMPORTANT I did a quick check and I couldn't find many of the sources you mention here (CERT BUND, \Crimeware, \DCSO...) as part of osint feeds. Make sure the sources you explicitly mention in the paper are public (misp-priv is not, but the standard misp feeds are) otherwise you MUST anonymize them. As this paper will probably be posted on the internet somewhen, you can't write any tlp:green info here, only tlp:white. So said, I believe it won't take away anything from your work to anonimize the sources, as you don't seem to use any information about the nature of the source organization in your work. and anonymizing them may even prevent some potential attacks concerning biases in the choice of sources (e.g., as a reviewer, my first comment to your njRat finding would have been "doesn't that depends on the fact that you looked at certain malware feeds instead of others?") in my opinion, a brief discussion about the nature of the anonimized sources and the inherent bias that comes with their selection/availability would even generalize/improve the final work. nothing too complex, e.g. were all the event descriptions in English? how did you treat other langauges? and stuff like that...


\noindent \textbf{Statistics.}
Our collection of 191 TI feeds comes from a variety of public and private providers, whose names   have been anonymized to comply with licensing agreements.
%
The dataset contains a total of 14,000 threat events and 866,541 IoCs from mostly between 2016-2019.
%
%
%
%
Table \ref{table: statistics} lists key statistics of top-10 TI feeds ranked based on the number of IoCs. 
%
The largest contributor is Feed~1 (by a government organization) which contributes 274,368 IoCs for 644 events.
%
We note that some TI feeds such as Feed~1 have hundreds of IoCs per event on average while others such as Feed~4 have less than 10. 
%
We also note that that average event timespan significantly varies across different TI feeds. 
%
Some TI feeds such as Feed~1 have shorter average event timespans of at most a couple of days while others such as Feed~5 have longer average event timespans of several weeks or even months. 



 \begin{table}[!t]
    \centering
\precaption        \caption{Statistics of TI feeds in our dataset.}
    \scriptsize
    \begin{tabular}{|c|c|c|c|c|c|}
        \hline
        TI  & \#  & \#  & IoCs  & Event  & Dominant IoC \\ 
         vendor & Events & IoCs & per Event & Timespan  & Category (\%) \\ 

        \hline
        \hline %Feed 1 
        \CERTBund 
        & 644 & 276.841 & 429 & 1.77 & network activity (69.65\%) \\
        \hline %Feed 2
        \CIRCL 
        & 1.234 & 165.292 & 134 & 45.86 & network activity (43.35\%) \\
        \hline %Feed 3 
        \inThreat 
        & 130 & 129.852 & 1076 & 21.29 & network activity (84.43\%) \\
        \hline %Feed 4 
        \InnoTecSystem 
        & 6.955 & 52.803 & 8 & 0.72 & network activity (98.51\%) \\
        \hline %Feed 5 
        \CthulhuSPRL  
        & 120 & 48.952 & 408 & 90.62 & network activity (84.73\%) \\
        \hline %Feed 6 
        \DCSO 
        & 230 & 27.375 & 119 & 14.12 & network activity (56.62\%) \\
        \hline %Feed 7 
        \Barncat  
        & 1.623 & 16.056 & 10 & 0.09 & external analysis (100\%) \\
        \hline %Feed 8 
        \Cryptolaemus 
        & 613 & 15.953 & 26 & 0 & network activity (82.94\%) \\
        \hline %Feed 9 
        \Crimeware 
        & 138 & 14.028 & 102 & 99.85 & payload delivery (81.10\%) \\
        \hline %Feed 10 
        \INCIBE 
        & 55 & 11.448 & 208 & 49.62 & payload delivery (68.52\%) \\
        \hline
    \end{tabular}
    \label{table: statistics}
    \postcaption
\end{table}



\noindent \textbf{IoC categories.}
Different TI feeds are geared towards different types of IoCs.
%
Specifically, each IoC in our data is classified into one of several IoC categories.\footnote{IoC categories are self-reported by each TI provider. We do not expect different TI feeds to use exactly the same categorization procedure.}
%
Table \ref{table: statistics} shows the most dominant IoC category for top-10 TI feeds in our data.
%
We note that a majority of popular TI feeds contain mostly network activity related IoCs while others contain IoCs related to payload delivery and external analysis. 
%
Network activity IoCs generally consist of IP addresses, hostnames, domains, and URLs. 
%
Payload delivery IoCs generally consist of filenames, hashes, and malware samples.
%
External analysis IoCs generally consist of textual analysis by security experts and links to other organizations.



\begin{figure}[!t]
    \centering
    %\includegraphics[width=1\columnwidth]{docs/IOC categories.png}
    \hspace{-0.2in}
    \includegraphics[width=1.05\columnwidth]{docs/updated_IoC_categories.png}
    \precaption
    \caption{Contribution of  TI feeds to popular IoC categories.}
    \label{fig: FeatureCounts}
    \postcaption
\end{figure}

%%
Next, we analyze the relative contribution of different TI feeds for popular IoC categories. 
%
Figure \ref{fig:FeatureCounts} plots the percentage of IoCs contributed by different TI feeds across popular IoC categories. 
%
We limit our analysis to top-3 IoC categories that comprise 87\% of the IoCs in our data.\footnote{Smaller IoC categories are categories such as artifacts dropped, social networks, support tools and other; these categories are sparsely used by TI feeds.}
%
%{\bf what do we mean by the following?}Note that IoC categories may not contain all TI feeds because {\bf can we start the sentence here?}some TI feeds do not have any IoCs for a particular category. 
%
The largest IoC category is network activity, which accounts for 557,532 IoCs.  
%
Across different TI feeds, Feed 1 and Feed 3 together contribute more than 50\% of network activity IoCs. 
%
The second largest IoC category is payload delivery, which accounts for 220,321 IoCs. 
%
Across different TI feeds, Feed~1 and Feed~2 each contribute about 30\% of payload delivery IoCs. 
%
The third largest IoC category is external analysis, which accounts for 38,531 IoCs. 
%
Across different TI feeds, Feed 7 and Feed 2 each contribute almost 40\% of external analysis IoCs. 

\begin{figure}[!t]
    \centering
    \includegraphics[width=\columnwidth]{docs/figures/ioc-by-day.png}
    \includegraphics[width=\columnwidth]{docs/figures/ioc-by-month.png}
    \precaption
    \caption{IoC Frequency By Day of Week and By Month Across Top 10 Feeds.}
    \label{fig:DayAndMonthTemporal}
    \postcaption
\end{figure}


\noindent \textbf{Temporal analysis.}
Next, we conduct analyses to understand the category breakdown of IoCs on a year-by-year basis for each of the top 10 feeds. It was found that certain feeds (e.g., \CIRCL, \CthulhuSPRL , and \DCSO) contained IoCs from a greater range of categories and this trend persisted each year. Other feeds had much greater uniformity in terms of these categories. For example, \Barncat  only contained External Analysis IoCs and \InnoTecSystem only had IoCs categorized as either Network Activity or Payload Delivery. The category percent changes across years for each feed do indicate that for most years, Network Activity remains the most common IoC category, but beyond this, there does not seem to be any other consistent trend, as feeds widely vary in their IoC category composition each year.

In order to gain further granular insight into IoC frequency, analysis was done on IoC count by Month and by Day of Week, respectively. It was found that IoCs tended to surface in the top 10 feeds significantly more during the months of March and July. Furthermore, IoCs were more frequently seen on Mondays and Thursdays as compared to the other days of the week.

\begin{figure}[!t]
    \centering
    \includegraphics[width=1.1\columnwidth]{docs/ioc-category-breakdown.png}
       \precaption
    \caption{Year-by-year category breakdown for top 10 feeds}
    \label{fig:TemporalCategoryBreakdown}
    \postcaption
\end{figure}


\begin{table}[!t]
    \centering
\precaption        \caption{Analysis of optional comment fields within the top ten TI feeds.}
    \scriptsize
    \begin{tabular}{|c|c|c|c|c|}
        \hline
        TI   & \# & Events having at least one & IoCs without & Average Length \\ 
        vendor  & IoCs  & IoC with a Comment (\%) & Comment (\%) & of Comment \\ 
        \hline
        \hline %Feed 1 
        \CERTBund 
        & 276,841 & 67.9\% & 36.5\% & 56.2 \\
        \hline %Feed 2
        \CIRCL 
        & 165,292 & 85.7\% & 28.9\% & 49.3 \\
        \hline %Feed 3 
        \inThreat 
        & 129,852 & 90.8\% & 3.20\% & 12.9 \\
        \hline %Feed 4 
        \InnoTecSystem 
        & 52,803 & 0.0\%& 100\% & 0.00 \\
        \hline %Feed 5 
        \CthulhuSPRL   
        & 48,952 &  63.3\% &  86.3\% & 42.3 \\
        \hline %Feed 6 
        \DCSO 
        & 27,375 & 97.4\% & 12.2\% & 19.8 \\
        \hline %Feed 7 
        \Barncat  
        & 16,056 & 100\% & 30.3\% & 9.40\\
        \hline %Feed 8 
        \Cryptolaemus 
        &15,953 & 100\% & 0.00\% & 10.7 \\
        \hline %Feed 9 
        \Crimeware 
        & 14,028 & 99.3\% & 4.18\% & 46.0\\
        \hline %Feed 10 
        \INCIBE 
        & 11,448 & 63.6\% & 27.9\% & 30.5 \\
        \hline
    \end{tabular}
    \label{table: statistics}
    \postcaption
\end{table}

\noindent \textbf{IoC comment fields.}
%- comments fields for each IoC
Throughout the TI Feeds in our dataset, there exists an optional comment field for each IoC in an event. We analyze the contribution of comments to our top ten feeds in terms of quantity and length. Each row of Table 2 shows each feed’s absence of comment fields, average character length across all IoCs, and percentage of events having at least one IoC with a comment field. Based on our findings, the majority of feeds had at least one comment per event (above 60\% of events). Among the IoCs in each feed, the majority of feeds also contained 1 comment per IoC and an average length above 10 characters. Since most feeds have IoCs with comments, we analyze the value these comments add to each feed.

As each comment could vary from one word to an entire paragraph of characters, we characterize a comment into three categories: additional description of an attack, format of the IoC, or logistical upload information. An IoC within the \DCSO feed had an additional information comment: “Kill switch domain. Monitor, do not block. (Source: Cisco Umbrella)”. Containing advice from a security expert, this comment could be utilized in determining how to proceed when combating an attack. On the other hand, a comment containing the format of an IoC is quite useful as well. The \Barncat  feed consists of textual IoCs which are difficult to classify due to their freeform formatting and length; however, their corresponding comment fields may help to pinpoint the key information. For instance, \Barncat ’s textual IoC containing the comment “RAT name” indicates the importance of analyzing the text relating to a specific remote access trojan. As this supplementary information could be utilized to provide deeper insight about existing incidents, the existence of comments may increase a feed’s extensiveness. Without comments correlating to each IoC, a feed loses further understanding of a security incident necessary for classification or patching. Thus, we conclude that feeds with a greater percentage of IoCs with comments are not only more extensive, but also may be of higher quality.


%- comment IoCs


\noindent \textbf{Overlap.}
Next, we analyze the overlap between IoCs across pairs of TI feeds.  To this end,  we restrict ourselves to IP and Hash IoCs overlapping across at least  one pair of TI feeds.
%
%To this end, in this section we restrict our analysis to IoCs overlapping across at least two out of  the top-10 feeds.
%
For \(n\) total feeds, the percentage of overlap between Feed 1 (row value) and Feed 2 (column value) in each cell in Figure~\ref{fig:feed_overlap} is calculated in the following manner:

\[ \frac{(Feed \thinspace 1 \cap Feed \thinspace 2)}{(Feed \thinspace 1 \cap Feed \thinspace 3) \cup (Feed \thinspace 1 \cap Feed  \thinspace 4) \cup \cdots \cup (Feed \thinspace 1 \cap Feed \thinspace n)} \]

Note that, in the above formula, the denominator does not contain the overlap between two identical feeds.
%

Figure~\ref{fig:feed_overlap} shows, for instance, that among the IP and Hash IoCs that are shared with another feed by \CIRCL,  25.4\% of these shared IoCs specifically have the same value as an IoC generated by \DCSO, e.g., the same IP address or Hash value.
% 
%Note that the overlap matrix is asymmetric as it is row normalized.
%
The dark vertical lines show that many TI feeds tend to share a greater fraction of their shared IP and Hash IoCs with a few popular TI feeds.
%
For example, four TI feeds (\inThreat, \InnoTecSystem, \CthulhuSPRL , \INCIBE) share a majority of their shared IP and Hash IoCs with \CIRCL. 
%
Two other feeds (\DCSO, \Cryptolaemus) share a majority of their shared IP and Hash IoCs with \CERTBund.
%
Such overlap is expected and has been reported in prior work on IP blacklists~\cite{li19tealeaves,Ramanathan20blacklists}.
%The overlap is because different TI feeds use the same source or when a large TI feed simply aggregates multiple smaller feeds.



\begin{figure}[!t]
    \centering
    \includegraphics[width=1.1\columnwidth]{docs/overlap_matrix_updated.png}
       \precaption
    \caption{IoC overlap across top-10 TI feeds for IPs and Hashes. Note that some TI feeds, in particular Feed 2, share common IoCs with several other TI feeds. (only considered hashes and ips)}
    \label{fig:feed_overlap}
    \postcaption
\end{figure}

\begin{figure}[!t]
    \centering
    \includegraphics[width=1.1\columnwidth]{docs/figures/similarity-heatmap.png}
       \precaption
    \caption{URL, Link, and Domain similarity across top-10 TI feeds}
    \label{fig:similarity_heatmap}
%    \postcaption
\end{figure}



%%
To further understand the differential contribution of different TI feeds, we analyze the flow (or temporal ordering) of common IoCs across TI feeds. 
%
Figure~\ref{figure:sankey} plots a Sankey diagram to visualize the flow of IoCs across the top-10 TI feeds. Similar to as was done for Figure~\ref{fig:feed_overlap}, analysis was restricted to IP and Hash IoCs. 
%
We make several observations. 
%
First, some TI feeds are mainly the source of common IoCs. 
%
For example, \CERTBund is the source of approximately 84.8\% (1923/2268) of its common IoCs.
%
Second, some TI feeds are mainly the sink of common IoCs. 
%
For example, \DCSO is mainly the sink of specific IoCs from \CERTBund and \CIRCL. 
%
This shows that \DCSO basically aggregates a subset of IoCs from multiple TI feeds.
%
Third, other feeds are more symmetric in being the sources/sinks of common IoCs.
%
For example, \CIRCL is the source of 68\% (2347/3442) of  common IoCs.
%
Thus, we conclude that these TI feeds complement each other in terms of timing (or information freshness).

\noindent \textbf{IoC Similarity.}
Next, we analyze the IoC similarity across the top 10 feeds. For this purpose, we focus on IoCs of categories url, link, or domain. We define similarity as when two IoCs share the same "base domain" value (e.g., a value of http://efax.pfdregistry.org/efax/37486.zip would have a "base domain" of efax.pfdregistry.org).

Figure~\ref{fig:similarity_heatmap} shows that feeds tend to share many IoCs of the same "base domains," even if the exact values differ. Some of the most common "base domains" across the top 10 feeds include virustotal.com, 185.234.216.52, ..., b4ckdoorarchive.com, and dropbox.com. In particular, it is interesting to note that \CIRCL shares significant similarity of url, link, and domain IoCs with nearly each of the other top 10 feeds, respectively. This is in sharp contrast to the other feeds, which share a much less uniform distribution of similarity with other feeds in terms of "base domains".


\begin{table}[!t]
    \centering
\precaption        \caption{Statistics of highest risk events across top-10 feeds.}
    \scriptsize
    \begin{tabular}{|c|c|c|c|}
        \hline
        TI  & Threat Level 1& Dominant IoC & Dominant IoC \\ 
         vendor & Events (\#) & Category (\%) & Type (\%)  \\ 
        \hline
        
        \hline %Feed 3 
        \CIRCL 
        & 30 & artifacts dropped (52.97\%) & filename|sha256 (38.81\%) \\
        \hline %Feed 5 
        \CthulhuSPRL  
        & 24 & network activity (96.82\%) & domain (96.11\%) \\
         \hline %Feed 6 
        \INCIBE
        & 17 & payload delivery (70.60\%) & sha256 (23.96\%) \\
        \hline %Feed 7 
        NCIRC
        & 12 & network activity (95.82\%) & ip-dst (93.87\%)\\
        \hline %Feed 2
        CERT-EU
        & 12 & network activity (68.61\%) & ip-src (63.50\%) \\
        \hline %Feed 1 
        \CERTBund 
        & 11 & payload delivery (56.61\%) & domain (23.66\%) \\
        \hline %Feed 10 
        TDC.dk 
        & 10 & payload installation (24.21\%) & filename (23.23\%)\\
        \hline %Feed 8 
        NCSC-NL
        & 8 & network activity (48.75\%) & domain (34.38\%) \\
        \hline %Feed 4 
        CUDESO
        & 7 & network activity (37.45\%) & ip-dst (19.34\%) \\
        \hline %Feed 9 
        SwissPost 
        & 6 & payload delivery (63.23\%) & md5 (48.18\%)\\
        \hline
    \end{tabular}
    \label{table: statistics}
  %  \postcaption
\end{table}

\noindent \textbf{Threat analysis.}
A similarity we notice between events per feed was their assigned threat level. Next, we analyze the threat level ID assigned to each event by its feed organization. The following threat levels provide the risk level of an attack: 4 (undefined risk), 3 (low risk general malware), 2 (medium risk advanced persistent threats (APT)), and 1 (high risk sophisticated APTs and zero day attacks). Across all feeds, there are 212 level 1 events, 1026 level 2 events, 11612 level 3 events, and 1148 level 4 events. % Add comparison and contrast with CVSS risk scores

Table 3 consists of ten feeds with the greatest quantity of threat level 1 events and their respective dominant IoC categories/types. Dominant IoC category/type pertains to the greatest IoC category/type percentage within that feed’s threat level 1 events. Based on this table, these feeds mostly contain IoCs within payload delivery and network analysis categories as shown by their over 50\% dominance in almost every feed. This is expected as hashes, domains, and ip addresses are common signs of compromise. Our data confirms this as the dominant IoC type column conveys the 4-type pattern the feeds follow: domain, filename, hashing algorithms, and IP address. In the \INCIBE, NCSC-NL, and \CIRCL feeds, IoCs of types sha1 “4bc2bbd1809c8b66eecd7c28ac319b948577de7b”, domain “myvalidation.info”, and ip-dst “83.229.62.212” report BlackEnergy malware, observed credential harvesting, and Turla command and control malware respectively. On the other hand, “nelis.at” is a phishing domain belonging to a level 3 event in the \CIRCL feed. As credential harvesting has a much higher vulnerability risk than a phishing domain, the distinction between level 1 and level 3 events is evident. By classifying the above events as threat level 1, organizations can prioritize patching attacks with the highest risk and monitor future IoC types/categories with similar activity. Thus, we conclude that high risk events tend to be classified as the above mentioned categories or types and recommend that specifically combating these types of IoCs may yield a more secure system. 

\begin{figure}[!t]
    \centering
    \includegraphics[width=1.1\columnwidth]{docs/tag-frequency-breakdown.png}
       \precaption
    \caption{Top feeds breakdown for frequency of tags}
    \label{fig:FrequencyTagBreakdown}
    \postcaption
\end{figure}

\noindent \textbf{Tag analysis.}
Throughout the TI feed in our dataset, there is a list of machine tags pertaining to each event. Composed of a namespace, predicate, and optional value, a machine tag can be utilized to further classify an event. These machine tags are apart of the MISP Taxonomies which allows various organizations to adopt common classification vocabulary. In our dataset a frequent tag was "tlp:white" indicating that the information included could be shared publicly and had no risk of misuse. 
Further, we analyze the distribution of tags to our largest feeds. This analysis was restricted to the top 9 feeds as they contain the majority of events in our dataset. Figure # consists of a breakdown indicating the number of tags per event for each feed. In most feeds, the events typically contain 2-3 tags with the most common being circl:incident-classification="malware", 'tlp:white', and misp-galaxy:banker="zeus". Since, most events have at least two descriptive tags, we conclude that this additional classification can aid in determining highest priority incidents. 


\noindent \textbf{Takeaway.}
Our analysis  shows that TI feeds complement each other by providing differing amounts and types of IoCs. 
%
As we discuss next, there is a need to develop automated methods to analyze loosely structured threat data in TI feeds. 





%
%Intuitively, the fact that  IoC categories and values  occur at multiple feeds  suggests that they can be used to  automatically process TI feed events.  
%
%In the following sections, we confirm that intuition by showing the feasibility of IoC-based text mining for classification of events  across  TI feeds.  


%The analysis of the rest of the feeds suggests that other TI feeds complement each other.
%Specifically, sometimes they are roughly equally the sources/sinks of common IoCs.
%For example, 
%and 60\% (1448/2429) 

%The analysis in this section  suggests that TI feeds   complement each other to the extent that they share   IoC categories (Table~\ref{table: statistics}) and  IoC values (Figures~\ref{fig:feed_overlap} and~\ref{figure:sankey}).  



%of its common IoCs while Feed 2 is the source of 83\% (1500/1807) of its common IoCs
%


%The overlap is because different TI feeds use the same source or when a large TI feed simply aggregates multiple smaller feeds.


%We define the flow between TI feeds $A$ and $B$ to be the number of common IoCs that are published by $A$ before $B$. 
%
%%%% The plot shows that smaller TI feeds often publish IoCs before larger TI feeds, which seem to be simply aggregating information from multiple smaller feeds.
%
%For example, ?? is the source of IoCs in CRICL and \CERTBund.
%
%%%% Thus, we conclude that while large TI feeds seem to subsume smaller TI feeds the latter are often the source of new IoCs. 
%
%%%% Thus, larger and smaller TI feeds complement each other in terms of coverage and speed. 
%The plot shows that there are  cycles of length two between certain  feeds, e.g., %, reflecting a balance between those pairs.  
%For instance, we find one such cycle between two of the top-3 feeds, as 
%

%zubair: can't figure our how to get these numbers from fig. 3
%Feed 0 publishes 166 IoCs before Feed 1 and, conversely, Feed 1 publishes 115 IoCs before Feed 0, reflecting a balance between that pair.  
%
%
%and
% We also find cycles of length greater than two, e.g., between   Feed 0, Feed 5, Feed 1 and Feed 0, that form a cycle of length three.

%forwards IoCs to Feed 5, which serves as a relay  to Feed 1, eventually forwarding IoCs back to Feed 0.




%With this visualization, it's possible to identify organizations that tend to be the first to publish IoCs. 

%This could be useful for pointing the contributors known for publishing inedited IoCs. We can also assess whether a contributor generates a concentrated flow or a branchy one, that is, the degree of collaborativeness. It's also possible to check for contributors that published
% many IoCs after many other sources. This characteristic is interesting for those who seek a source 
% that can summarize the IoCs already available out there.
 
 


%There is overlap, but who is the source
%- flow/sequence analysis
%- big feeds are not always the source


\begin{comment}
 We show diagrams for the following types of IoCs: artifacts dropped, payload installation, network activity and payload delivery.
Among the most important contributors, we highlight \CIRCL. It is the source with the higher amount of published inedited artifacts dropped. 
It also has one of the main roles on the flow of payloads installations. It's very interesting to observe that, for the types 
payload delivery and network activity, \CIRCL contributes to many organizations (i.e. publishes IoCs before them), and is benefited
from a variety of sources (publishes after them). Thus, \CIRCL is an essential contributor for two reasons: 
1) it is a good inaugurator of IoCs
2) it also relies on several other sources, being diverse

We envision that having such a strong contributor with these two characteristics enriches our dataset in terms of generalization.
We believe that \CIRCL, among other important organizations in our dataset, has a good representative power of IoCs reported 
on TI Feeds in the wild.
 
\end{comment}


\begin{comment}
\begin{figure}
  \begin{subfigure}[t]{0.57\columnwidth}
    \centering
    \includegraphics[width=1\columnwidth]{docs/figures/sankeys/artifacts_dropped.png}
    \caption{\textbf{Artifacts Dropped}}
  \end{subfigure}
  \hfill
  \begin{subfigure}[t]{0.57\columnwidth}
    \centering
    \includegraphics[width=\linewidth]{docs/figures/sankeys/network_activity.png}
    \caption{\textbf{Network Activity}}
  \end{subfigure}

  \medskip

  \begin{subfigure}[t]{0.57\columnwidth}
    \centering
    \includegraphics[width=\linewidth]{docs/figures/sankeys/payload_delivery_flow.png}
    \caption{\textbf{Payload Delivery} }
  \end{subfigure}
  \hfill
  \begin{subfigure}[t]{0.57\columnwidth}
    \centering
    \includegraphics[width=\linewidth]{docs/figures/sankeys/payload_installation.png}
    \caption{\textbf{Payload Installation}}
  \end{subfigure}
\end{figure}

\end{comment}






%TI feeds can be sourced from both public and private entities. 
%For example, \InnoTecSystem \cite{InnoTec} is a private TI feed source while \CIRCL (Computer Incident Response Center Luxembourg) \cite{\CIRCL} is run by a government organization. 
%


%The time period of our data spans from 2013 to 2019, with 99.76 percent from the years of 2016-2019. 
%The breakdown of those years are as follows: 41.33\% from 2019, 29.11\% from 2018, 17.51\% from 2017, and 11.81\% from 2016.
%
%who are top TI vendors (public or private)rewrite for the top 10 
%\textbf{TI Vendors (public vs. private).}
%






%These timestamps are useful as there is a temporal aspect to cyberthreats \cite{sleeman2020temporal}. 


%
%In the case of events, the timestamp is consistent across the event. 
%While in the case of IOCs, the time stamps are individually generated. 
%Each IOC timestamp is generated in the range of the event it relates to. 
%
%




%
%This is of consideration as the event provides context for the IOCs, and the IOCs provide details for the event. 
%This balancing is important for a TI source that is both contextually rich and functionally detailed for a the purpose of containing actionable insights.
%


%\textbf{Event timespan.}



%each IoC is timestamped
%Discuss table1
%Correlation coef


%
%The amount of IOCs and the events they belong to are independent. 
%As shown in table 1 some TI feeds contain very few events with many IOCs, such as \inThreat.
%While others contain many events with few IOCs, such as \InnoTecSystem. 



%With assessing the volume of a feed the metric that used is distinct count of IOCs. 
%
%We chose this approach because the largest impact on our data are the IOCs and not the threat events themselves. 
%Altough the threat events provide context for the user, IOCs are the details of that event, and as such we determine that a higher volume of details is of greater importance when determining threats. 
%




%Of our top 10 IOC contributors the largest by volume are listed below in order from largest to smallest. 

\begin{comment}


\begin{enumerate}
  \item \CERTBund is a government run agency in Germany, it has been in operation since 2001. 
  \item \CIRCL (Computer Incident Response Luxembourg) is a government run agency from Luxembourg, and has been in operation since 2008. 
  \item \inThreat is a privately run organization from France that has been in operation since 2008. 
  \item \InnoTecSystem is a privately run organization from Spain that has been in operation since 2002. 
  \item \CthulhuSPRL  is a privately run organization from France that is currently in the provess of liquidation. 
  \item \DCSO is a privately run organization from Germany that has been in operation since 2015. It specializes in cyber espionage and theft.  
  \item \Barncat  is privately run company from the United States that has been in operation since 2002.
  \item Cryptylaemus is an cybersecurity research group that is famous for its work on EMOTET. 
  \item \Crimeware? no information found (will ask matheus about this)
  \item \INCIBE is a government run organization from brazil that has been in operation since 2014
  
\end{enumerate}




\begin{enumerate}

\item \emph{Network activity} has data types consisting of IP addresses, hostnames, domains, and URLs. 

\item \emph{Payload delivery} consists of data types such as filenames, hashes, malware samples, and IP addresses.


\item \emph{External analysis} consists of data such as links to other organizations and their analysis of a particular IOC. 


\item \emph{Payload installation} contains hashes and filenames as well as expert textual description describing what was executed, what group or organization was responsible for the threat, and what campaign the samples are from. 


\item \emph{Artifacts dropped} are filenames and signatures resulting from a threat event. 

\end{enumerate}

%
%
%
%



%%IoT Categories (dominant IoC category)
%Figure 1; Table 1 (last column)
As we discuss next, the events in different TI feeds are geared towards different types of IOCs.
%
For instance, some TI feeds mostly contain network activity related IOCs such as IP addresses while others contain more rich textual analysis by security experts. 
Each IOC in our data is classified by category. In figure 1 the top 5 IOC categories are shown. These categories are self reported from each TI vendor, due to this self reporting and varying standards there is some ambiguity with these categories. 

Because of this we analysed the raw data to determine the meaning of these categories in the context of the data. Generally, with the top features there is very little variation with the IOC categories and raw data. However, with smaller IOC categories such as social networks, support tools and other; these categories are sparsely used by the majority of TI feeds.  These small categories contain raw data that is difficult to differentiate their meaning in context to larger categories. Although present in the data the volume of these ambiguous categories total less then 0.19\% of the total amount of IOCs. With this small of a percentage we are confident that the integrity of the remaining IOC categories is uncompromised. 


\end{comment}



%\subsubsection{Derived Features}A challenge with the use of hashes as IOCs is many are only unique to one event, that is they are not generalizable. As many threats have polymorphic capabilities to mask the file signature. To extract better information from this we created a derived feature from the hash data. This derived feature was made by counting how many times hashes appeared in a event. In addition to this derived feature we included other features that is not explicitly an IOC. This includes time stamps, related events, and number of total number of IOCs within each threat event.

%In contrast to the use of only TI feeds in developing threat intelligence, some researchers have gone to the forums where hackers share threat information and discuss exploits. There is evidence to suggest that these hacker forums may also have valuable threat data. \cite{nunes2016darknet}



%Payload delivery is similar to network activity but also includes file names and signatures. Payload delivery contains data from where the payload was from such as a URL, and the signature of the file delivered. Some of these IOCs contain descriptions if the payload delivery is a part of a greater campaign. This description provides better context for these features when compared to network activity that has little context description.

%\item xternal analysis is the third largest category in our data, at 38,531 IOCs. External analysis contains data that describes the behaviour or exist CVEs related to that sample. Some of this data may explain what ports were used to communicate or what system files were changed. Many of these are generated from virus total, amongst other services. External analysis overlaps with payload delivery and payload installation. As external analysis is performed on delivered or executed samples. 

%\item The fourth largest category is artifacts dropped, at 24,824 IOCs. %This category is similar to payload installation however the data is usually pieces from malicious activity. These can contain file samples, files that are potentially compromised, or other traces that some persistent threats leave behind. Although not as descriptive as payload installation this data has IOCs relating to novel threats. This is useful for finding previously unknown exploits. 

%\item The fifth largest category is payload installation, at 15,002 IOCs. Payload installation is similar in some aspects to payload delivery. The data types are similar, consisting of hashes and filenames. However payload installation differs to payload delivery by containing more expert textual description. Of all the categories payload installation has the most textual description. Explaining what the IOC does, what campaign it may be a part of, or what was the target of the threat. This is useful for existing exploits by finding similar behaviours and their corresponding exploits.  



==> docs/data_daniel.tex <==
% \vfill\eject

% 100.json --> exploit 


\section{TI Feed Characterization}
\label{sec: data}
In this section, we analyze TI feeds in our dataset with respect to IoC categories as well as their temporal and spatial characteristics. Our findings indicate that automated methods are needed to efficiently interpret loosely-structured threat data for various downstream security tasks. 

\vspace{.05in} \noindent \textbf{Preliminaries.} 
A \emph{TI feed} is a general term used to describe a curated source of information such as IP addresses, file hashes, textual threat description, and other features providing context to existing and potential threats. 
%
All of these features are collectively referred to as \emph{Indicators of Compromise} (or IoCs).
%
Each TI feed, from a public or private provider,\footnote{In general, it is not always the case that there is a one-to-one correspondence between TI feeds and providers, as some TI feeds may contain events from multiple providers. In this work, however, as we anonymize providers (also known as organizations) we refer to feeds and providers interchangeably, with each provider corresponding to its own feed.} contains a list of \emph{events} and each event includes a collection of IoCs. %Listing \ref{listing: json-example} in Appendix~\ref{app:exampleevent} is 
%In  our Supplementary Material~\cite{supplementarymaterial} we illustrate  an event from our dataset and the "Attributes" field includes its IoCs.
%
An event could be a security incident such as a phishing attack, a botnet attack, or a security advisory regarding a software vulnerability.
%
Each event also includes timestamps indicating when the event was created and last modified.  
%
The IoCs within an event are also individually timestamped based on when they are created or last modified.  
%
The \emph{event timespan} is the difference in days between the latest and earliest IoC timestamps associated to that event. 
%
Each IoC is accompanied by a comment field which contains free-form textual description of the IoC as well as an IoC category. 
%
An event may also contain a comment field typically summarizing the security analyst's assessment of the event.
%
The list of IoCs, comments, and timestamps together constitute the \emph{attributes} of the event.
%
In addition to these attributes, an event may be assigned \emph{tags} by a security analyst. 
%
Tags follow standardized taxonomies.  
%
An event tagged as \emph{tlp:white}, for example,  contains information that can be shared with the general public according to the Traffic Light Protocol (tlp), whereas an event tagged as \emph{type:osint} contains information that is considered Open Source Intelligence (OSINT). 

\begin{table}[!t]
    \centering \vspace{0.05in}
       \caption{Top-10 TI feeds ranked based on IoC count}
        {
        \resizebox{0.49\textwidth}{!}{
            \begin{tabular}{|l|r|r|r|r|c|l|}
            \hline
            Provider & Event count &  IoC count & Average number  & Average event~\    & Dominant IoC category (\%)  \\ 
            & &   ~\ ~\  & of IoCs per event & timespan (days)  &  \\
              %&  &  &  &   &  \\ 
            \hline
            \hline %Feed 1 
            {\CERTBund}
            & 644 & 276,481 & 429.3 & 1.77 & network activity (69.65\%)  \\
            \hline %Feed 2
            {\CIRCL} 
            & 1,234 & 165,292 & 133.9 & 45.86 & network activity (43.35\%)  \\
            \hline %Feed 3 
            {\inThreat} 
            & 130 & 139,852 & 1,075.8 & 21.29 & network activity (84.43\%)  \\
            \hline %Feed 4 
            {\InnoTecSystem} 
            & 6,955 & 52,803 & 7.6 & 0.72 & network activity (98.51\%)  \\
            \hline %Feed 5 
            {\CthulhuSPRL}   
            & 120 & 48,952 & 407.9 & 90.62 & network activity (84.73\%)  \\
            \hline %Feed 6 
            {\DCSO} 
            & 230 & 27,376 & 119.0 & 14.12 & network activity (56.62\%)   \\
            \hline %Feed 7 
            {\Barncat}  
            & 1,623 & 16,056 & 9.9 & 0.09 & external analysis (100\%)  \\
            \hline %Feed 8 
            {\Cryptolaemus} 
            & 613 & 15,953 & 26.0 & 0.00 & network activity (82.94\%)  \\
            \hline %Feed 9 
            {\Crimeware} 
            & 138 & 14,028 & 101.7 & 99.85 & payload delivery (81.10\%) \\
            \hline %Feed 10 
            {\INCIBE} 
            & 55 & 11,448 & 208.1 & 49.62 & payload delivery (68.52\%)  \\
            \hline
            {Other feeds} 
            & 2256 & 98,305 & 6.6 & 4.32 & network activity (45.98\%)  \\
            \hline
        \end{tabular}
        }
        }
        \label{table: statistics}
    \end{table}
    


%%
\begin{figure}[!t]
    \centering
     \includegraphics[width=\columnwidth]{docs/figures/IoC_Count_CDF.pdf}
    \caption{CDFs of   number of IoCs per event for   top 10 feeds.}
     \label{fig: iocs per event}
    \postcaption
\end{figure}


\vspace{.05in} \noindent \textbf{Summary statistics.} 
Our dataset is comprised of  a collection of 191 TI feeds that come from a variety of public and private providers.
%
In total, our dataset contains about 14 thousand events and 866,541 IoCs over the duration of 7 years (2013-2019).
%
Table \ref{table: statistics} lists key statistics of top-10 TI feeds ranked based on the number of IoCs.%\footnote{In our Supplementary Material~\cite{supplementarymaterial} we provide  a general description of TI feed providers.} 
%
The largest contributor is {\CERTBund}{} (a government organization) which contributes 276,481 IoC references with an average of 429 IoCs per event.
%
We note that the number of IoCs per event vary by several orders of magnitude across different feeds. 
%
Some feeds such as {\inThreat} have more than a thousand IoCs per event on average while others such as {\InnoTecSystem} have less than 10. 
%
Figure \ref{fig: iocs per event} further plots the distribution of the number of IoCs per event across different feeds. 
%
We note that even for feeds with a high average number of IoCs per event, the majority of events contain only a handful of IoCs.
%
For example, each of the top 10 feeds have at least 70\% of their events having no more than 200 IoCs each.
%
Further, all of the top 10 feeds, except {\Crimeware}, have at least 60\% of their events having no more than 100 IoCs each.




\subsection{IoC Categories}
Different TI feeds are geared towards different types of IoCs.
%
Specifically, each IoC is classified by the feed vendor into one of several IoC categories.\footnote{IoC categories are self-reported by each TI feed vendor. We do not expect different TI feeds to use exactly the same categorization procedure.}
%
Table \ref{table: statistics} shows the most dominant IoC categories for top-10 TI feeds in our data.
%
We note that a majority of popular TI feeds contain mostly network activity related IoCs while others contain IoCs related to payload delivery and external analysis. 
%
Network activity IoCs generally consist of IP addresses, hostnames, domains, and URLs.
%
Payload delivery IoCs generally consist of filenames, hashes (e.g., sha1, sha256 and md5), and malware samples.
%
External analysis IoCs generally consist of textual analysis by security experts and links to other pertinent organizations.







\begin{figure}[!t]
    \centering
     \includegraphics[width=0.9\columnwidth]{docs/figures/Figure1.pdf}
    \caption{Contribution of  TI feeds to popular IoC categories.}
     \label{fig:FeatureCounts}
     \vspace{-0.25in}
    \postcaption
\end{figure}




%%
Next, we analyze the relative contribution of different TI feeds across popular IoC categories. 
%
Figure~\ref{fig:FeatureCounts} plots the percentage of IoCs contributed by different TI feeds across popular IoC categories. 
%
We limit our analysis to top-3 IoC categories that comprise 87\% of the IoCs in our data.
%
Less popular IoC categories include artifacts dropped, social networks, support tools, etc.
%
The largest IoC category is {network activity}, which accounts for 557,532 IoCs.  
%
Across different TI feeds, {\CERTBund} and {\inThreat} together contribute more than 50\% of network activity IoCs. 
%
The second largest IoC category is {payload delivery}, which accounts for 220,321 IoCs. 
%
Across different TI feeds, {\CERTBund} and {\CIRCL} each contribute about 30\% of payload delivery IoCs. 
%
The third largest IoC category is external analysis, which accounts for 38,531 IoCs. 
%
Across different TI feeds, {\Barncat} and {\CIRCL} each contribute almost 40\% of external analysis IoCs. 






%\subsubsection{IoC comments}
Next, we analyze IoC categories with external comments. 
We find that all except one feed have a majority of events with at least one IoC with a comment. 
%
Across these feeds, on average, 67.7\% of IoCs have a comment and the comment length is 27.7 characters. 
%
We identified three categories of comments: 
additional description of an attack, format of the IoC, or logistical upload information. 
%
The first type of comments usually contain a note/advice from a security expert.
%
For example, an IoC within one of our feeds % {\DCSO} 
 had an additional information comment: ``Kill switch domain. Monitor, do not block. (Source: Cisco Umbrella).'' 
%
Such comments could be useful in determining how to proceed when responding to a security incident. 
%
The second type of comments describe the format of IoCs. 
%
For example, an IoC within one of the considered feeds  % {\Barncat}
contained the comment ``RAT name,'' thus providing useful information that the IoC mentions the name of a specific remote access trojan. 
%
The third type of comments contain other logistical information that also provide context for the IoC. 
%
For example, an IoC in one of the considered feeds % {\Crimeware} 
contained the comment ``This attribute has been automatically imported.'' 
%
This information could be necessary when prioritizing which events or IoCs need to be analyzed first. 
%
Thus, we conclude that the information in these free-form textual comments provide deeper insights into security incidents. % that might be crucial for downstream tasks such as patching. 


\begin{comment}
\subsubsection{IoC geolocation}
We next analyze the geographic distribution of threat information contained in different feeds. 
%
While IoCs are not explicitly geotagged, we attempt to localize IP addresses in IoCs using the MaxMind IP geolocation database \cite{maxmind2002geolite2}. 
%
Figure \ref{fig:geolocation} plots the distribution of geolocated IoCs in our dataset.\footnote{Note geolocated IP address maps for the remaining top-10 feeds are found in Appendix \ref{sec: appendix geolocation}.}
%
Overall, the top countries corresponding to the geolocated IP addresses are the United States, China, Russia, Germany, and India.
%
We note that there are differences in geographic distribution across different TI feeds. 
%
For example, {\CIRCL} mostly contains geolocated IP addresses in the United States while {\inThreat} contributes the largest number of  IP addresses for every top country (>1000). Although there is a distinct presence of IP addresses in the US and Russia for both {\CIRCL} and {\inThreat}, their IP address ranges  significantly differ and complement each other in those countries (IP address ranges within countries are not shown in the figure). 
As shown in Table~\ref{table: statistics},  
{\inThreat} has a higher percentage of network activity IoCs (84{\%}) when compared against {\CIRCL} (43{\%}), and  receives daily updates 
(see Table~\ref{table:iocCountByDayOfWeek}) from hundreds of contributors. \hl{Need to add why this section is relevant to ML section otherwise we should delete it. @Professor Shafiq I don't think this section is necessary to include anymore due to the page limit. Any suggestions?}


\end{comment}


\newcommand*{\MinNumberTemporal}{0}%
\newcommand*{\MaxNumberTemporal}{216714}%

\newcommand{\ApplyGradient}[1]{%
       % \pgfmathsetmacro{\PercentColor}{100.0*(#1-\MinNumber)/(\MaxNumber-\MinNumber)}
        \pgfkeys{/pgf/fpu,/pgf/fpu/output format=fixed}%
        %\pgfmathsetmacro{\PercentColor}{(#1 + 1000) / 10000 * 100}
        \pgfmathsetmacro{\PercentColor}{(#1 + 10000) / \MaxNumberTemporal * 100}%
        \edef\x{\noexpand\cellcolor{yellow!\PercentColor}}\x\textcolor{black}{#1}%
        \pgfkeys{/pgf/fpu = false}
}
\newcolumntype{R}{>{\collectcell\ApplyGradient}c<{\endcollectcell}}


\renewcommand*{\MinNumberTemporal}{0}%
\renewcommand*{\MaxNumberTemporal}{307963}%

\renewcommand{\ApplyGradient}[1]{%
       % \pgfmathsetmacro{\PercentColor}{100.0*(#1-\MinNumber)/(\MaxNumber-\MinNumber)}
        \pgfkeys{/pgf/fpu,/pgf/fpu/output format=fixed}%
        %\pgfmathsetmacro{\PercentColor}{(#1 + 1000) / 10000 * 100}
        \pgfmathsetmacro{\PercentColor}{(#1) / \MaxNumberTemporal * 100}%
        \edef\x{\noexpand\cellcolor{yellow!\PercentColor}}\x\textcolor{black}{#1}%
        \pgfkeys{/pgf/fpu = false}
}











\begin{comment}
\begin{table*}[!t]
\centering
%\scriptsize
\footnotesize
\precaption
\caption{Temporal analysis of IoC count (by year)}
\vspace{-.2in}
\begin{tabular}{l | R R R R R R R R R R R}
\toprule
\multicolumn{1}{c}{Year} &
\multicolumn{1}{c}{\CERTBund} &
\multicolumn{1}{c}{\CIRCL} &
\multicolumn{1}{c}{\inThreat} &
\multicolumn{1}{c}{\InnoTecSystem} &
\multicolumn{1}{c}{\CthulhuSPRL } &
\multicolumn{1}{c}{\DCSO} &
\multicolumn{1}{c}{\Barncat } &
\multicolumn{1}{c}{\Cryptolaemus} &
\multicolumn{1}{c}{\Crimeware} &
\multicolumn{1}{c}{\INCIBE} & 
\multicolumn{1}{c}{Total}\\
\midrule
2013  &          0 &    1044 &             0 &               0 &               0 &      0 &        0 &             0 &          0 &       0 & 1044\\
2014  &          0 &    6096 &             0 &               0 &               0 &      0 &        0 &             0 &          0 &       0 & 6096\\
2015  &         31 &    8278 &             0 &               0 &            8288 &      0 &        0 &             0 &          0 &       0 & 16597\\
2016  &        195 &   66555 &           796 &               0 &            5409 &     78 &    14490 &             0 &      10813 &    3523 & 101859\\
2017  &       2681 &   70009 &          1062 &               0 &           34574 &   3295 &        0 &             0 &       2908 &    7826 & 122355\\
2018  &     104005 &   12070 &         17003 &           52759 &             669 &   7896 &     1575 &         15953 &        307 &      99 & 212336\\
2019  &     169569 &    1240 &        120991 &              44 &              12 &  16107 &        0 &             0 &          0 &       0 & 307963\\
\bottomrule
\end{tabular}
\label{table:iocCountByYear}
\vspace{-.15in}
\end{table*}

\begin{table*}[!t]
\centering
\footnotesize
\precaption
\caption{Temporal analysis of IoC count (by month)}
\vspace{-.2in}
\begin{tabular}{l | R R R R R R R R R R R}
\toprule
\multicolumn{1}{c}{Month} &
\multicolumn{1}{c}{\CERTBund} &
\multicolumn{1}{c}{\CIRCL} &
\multicolumn{1}{c}{\inThreat} &
\multicolumn{1}{c}{\InnoTecSystem} &
\multicolumn{1}{c}{\CthulhuSPRL } &
\multicolumn{1}{c}{\DCSO} &
\multicolumn{1}{c}{\Barncat } &
\multicolumn{1}{c}{\Cryptolaemus} &
\multicolumn{1}{c}{\Crimeware} &
\multicolumn{1}{c}{\INCIBE} & 
\multicolumn{1}{c}{Total}\\
\midrule
January   &      21352 &    7349 &            76 &              10 &             299 &  16243 &        0 &             0 &       2350 &      73 & 47752 \\
February  &      42072 &    9848 &           251 &              23 &            2948 &    347 &        0 &             0 &        247 &    1932 & 57668\\
March     &      58174 &   28785 &        103897 &               0 &              20 &   1085 &    14489 &             0 &         64 &     200  & 206714\\
April     &      36913 &   40174 &         11085 &               0 &            4660 &    971 &        0 &             0 &        200 &    2494 & 96497 \\
May       &      12332 &   18777 &          6671 &              11 &              69 &   1730 &        0 &             0 &         91 &      98 & 39779 \\
June      &        500 &    5424 &           191 &               0 &             492 &    854 &     1575 &             0 &        237 &     169 & 9442 \\
July      &      32469 &    6397 &            41 &            4263 &           34256 &    726 &        0 &             0 &          0 &     558 & 78710  \\
August    &      13509 &    9301 &           145 &           48196 &            2645 &   1754 &        1 &             0 &       1337 &      35 & 76923 \\
September &      13317 &   10651 &         15170 &             169 &             154 &   1218 &        0 &             0 &       2707 &    5834 & 49220\\
October   &      11001 &   11274 &          1869 &             102 &             497 &   1484 &        0 &             0 &       2348 &      47 & 28622 \\
November  &      16030 &   10644 &           333 &              13 &            1486 &    751 &        0 &         10542 &       2202 &       8 & 42009 \\
December  &      18812 &    6668 &           123 &              16 &            1426 &    213 &        0 &          5411 &       2245 &       0  & 34914\\
\bottomrule
\end{tabular}
%\label{table:iocCountByMonth}
\vspace{-.15in}
\end{table*}
\end{comment}



\subsection{Temporal analysis}
Since an event is essentially a timeseries of IoCs, we start our temporal analysis by breaking down event timespan across different TI feeds. Recall that the \emph{event timespan} refers to the interval between the lowest and the highest timestamp of the IoCs in the event.
%
As shown in Table \ref{table: statistics}, average event timespan significantly varies across different TI feeds. 
%
Some TI feeds such as {\CERTBund} have shorter average event timespans of less than a couple of days while others such as {\CthulhuSPRL } have longer average event timespans of up to 3 months. 
%
Note that several TI feeds such as {\InnoTecSystem} and {\Barncat}  have the average event timespan of less than one day. 
%
In fact, the average timespan of {\Cryptolaemus} is zero, which means that all IoCs in each of its events have the same timestamp. 
%
Figure \ref{fig: event timespan} further plots the distribution of event timespan across different feeds. 
%
We note that 9 of the top 10 feeds have at least 70\% of their events having timespans of no more than 4 days.
%
{\Crimeware} is distinct in that its events tend to have much longer timespans, with under 30\% of its events having timespans of fewer than 30 days.



\begin{figure}[!t]
    \centering
     \includegraphics[width=\columnwidth]{docs/figures/Timespan_CDF.pdf}
    \caption{CDFs of the event timespan for the top 10 feeds.}
     \label{fig: event timespan}
    \postcaption
\end{figure}

%\subsubsection{Year}
%Table \ref{table:iocCountByYear} plots the distribution of IoCs across the top-10 feeds by year. We note that the total number of IoCs across all TI feeds has increased each year. The total number of IoCs increased to more than 300K in 2019, which represents a 45\% increase compared to 2018. Following the overall trend, the IoC counts for several feeds (e.g., {\CERTBund}, {\inThreat}, {\DCSO}) steadily increase each year, especially in the last few years. In contrast, some feeds show the opposite trend (e.g., {\Crimeware}) and other feeds such as {\InnoTecSystem}, {\CthulhuSPRL}, {\Barncat}, and {\Cryptolaemus} have a high volume of IoCs in certain years and significantly less in other years. The IoC volume for {\CIRCL} increased up to 2017 and has tapered off since then. We conclude that there is substantial temporal variability over the years across different TI feeds in our dataset. 


%\subsubsection{Month and day of the week}
%Tables \ref{table:iocCountByMonth} and \ref{table:iocCountByDayOfWeek} plot the distribution of IoCs across the top-10 feeds by month and by day of the week, respectively. While most of the feeds had IoCs evenly spread across different months of the year, a few had significant spikes in certain months. For example, {\inThreat} had a large volume of its IoCs (approximately 74\%) in March, while {\InnoTecSystem} and {\DCSO} had similar spikes in August and January, respectively. IoC volume spikes also existed for days of the week, with many feeds containing IoCs disproportionately timestamped on certain days of the week. For example, {\inThreat} had a significant portion of its IoCs timestamped for Thursday and Friday. Similarly, {\CthulhuSPRL}  had approximately 73\% of its IoCs created/updated on Monday and {\DCSO} had approximately 52\% of its IoCs timestamped for Thursday. These IoC frequency spikes in particular months and days of the week show that there may be periodic disclosures/updates to IoCs and these schedules may vary across different TI feed providers.

%
%\begin{table*}[!t]
%\centering
%\footnotesize
%\precaption
%\caption{Temporal analysis of IoC count (by day of week)}
%\vspace{-.2in}
%\begin{tabular}{l | R R R R R R R R R R R}
%\toprule
%\multicolumn{1}{c}{Month} &
%multicolumn{1}{c}{\CERTBund} &
%\multicolumn{1}{c}{\CIRCL} &
%%\multicolumn{1}{c}{\inThreat} &
%\multicolumn{1}{c}{\InnoTecSystem} &
%\multicolumn{1}{c}{\CthulhuSPRL } &
%\multicolumn{1}{c}{\DCSO} &
%\multicolumn{1}{c}{\Barncat } &
%\multicolumn{1}{c}{\Cryptolaemus} &
%\multicolumn{1}{c}{\Crimeware} &
%\multicolumn{1}{c}{\INCIBE} & 
%\multicolumn{1}{c}{Total}\\
%\midrule
%Monday    &      49351 &   24920 &         21641 &           10262 &           35588 &   6822 &     1575 &          3107 &       2487 &     362  & 156115\\
%Tuesday   &      41334 &   44215 &         15135 &            4128 &            3956 &   2313 &        1 &          2172 &       1859 &    6738 & 121851 \\
%Wednesday &      40885 &   28419 &          9551 &           10859 &            1482 &   1288 &        0 &          1821 &       3981 &     514 & 98800 \\
%Thursday  &      44271 &   23456 &         33019 &           10229 &            5867 &  14341 &    14489 &          3283 &       2973 &    1415 & 153343\\
%Friday    &      40934 &   17966 &         30931 &           13703 &            1885 &   2459 &        0 &          3968 &       2728 &    2367 & 116941 \\
%Saturday  &      36436 &    3571 &          8543 &             203 &             130 &     22 &        0 &           988 &          0 &      46 & 49939\\
%Sunday    &      23270 &   22745 &         21032 &            3419 &              44 &    131 &        0 &           614 &          0 &       6 & 71261\\
%\bottomrule
%\end{tabular}
%\label{table:iocCountByDayOfWeek}
%\vspace{-.15in}
%\end{table*}



%\subsubsection{Day of the week}
%%


\begin{comment}
\begin{figure}[!t]
    \centering
     \includegraphics[width=\columnwidth]{docs/figures/IoC_Count_Day.pdf}
    \caption{ IoC count across the top 10 feeds by day of week. }
     \label{fig: event timespan day}
    \postcaption
\end{figure}
\end{comment}

\subsection{Spatial Analysis}
Next, we analyze the IoC overlap to characterize information redundancy across TI feeds.  
%
Note that we restrict ourselves to IoCs containing specific IP addresses and hashes.
%
Some feeds share only a few IoCs with other feeds, while others share a lot of IoCs with several other feeds. % (see Supplementary Material~\cite{supplementarymaterial}  for details). 
%
%
For example, {\Cryptolaemus} shares less than 4 IoCs with all but one of the top-10 TI feeds. 
%
In contrast, many TI feeds tend to have a significant number of their IoCs in common with  particular sets of other feeds.
% %, respectively, 
For instance, {\CIRCL} shares over 250 IoCs with  each of 6 of the other top feeds, with over 900 IoCs shared with {\DCSO} and over 1000 IoCs shared with {\INCIBE}.
%
Similarly, {\CERTBund} shares upwards of 200 IoCs with {\CIRCL} and {\inThreat} and over 1700 with {\DCSO}.
%
Such overlap between different TI feeds is not surprising and has been reported in prior work on IP blocklists \cite{li19tealeaves,Ramanathan20blacklists}.




% \begin{figure}[!t]
%     \includegraphics[width=.5\columnwidth]{docs/figures/ioc_feed_overlap-crop.pdf}
%     \caption{IoC overlap across top-10 TI feeds. Note that some TI feeds, in particular {\CIRCL}, share common IoCs with several other TI feeds, noting that  overlap only accounts for  hashes and IPs.}
%     \label{fig:feed_overlap}
% \end{figure}

% \begin{figure}[!t]
%  \includegraphics[width=.5\columnwidth]{docs/figures/sankeys/sankey_anonymized.png}
%     \caption{Flow of common IoCs across top-10 TI feeds. The left side shows counts of IoC sources and the right side shows the counts of IoC sinks.}
%     \label{figure:sankey}
% \end{figure}


%\begin{figure}
% \centering
%    \includegraphics[width = 0.7\linewidth]{docs/ioc-overlap-raw-count.png}
%    \captionof{figure}{IoC overlap across top-10 TI feeds for IPs and Hashes. Note that some TI feeds, in particular {\CIRCL}, share common IoCs with several other TI feeds, noting that  overlap only accounts for  hashes and IPs.}
%    \label{fig:feed_overlap}
%\end{figure}

%\begin{figure}
%    \centering
% \includegraphics[width = 0.7\linewidth]{docs/figures/sankeys/sankey_diagram_updated_resized.png}
%    \captionof{figure}{Flow of IoCs across top-10 TI feeds. The left side shows counts of IoC sources and the right side shows the counts of IoC sinks.}
%    \label{figure:sankey}
%\end{figure}




%\begin{figure}[!t]
%    \centering
%    \includegraphics[width=1.1\columnwidth]{docs/ioc-overlap-raw-count.png}
%       \precaption
%    \caption{IoC overlap across top-10 TI feeds for IPs and Hashes. Note that some TI feeds, in particular {\CIRCL}, share common IoCs with several other TI feeds. (only considered hashes and ips)}
%    \label{fig:feed_overlap}
%    \postcaption
%\end{figure}


%%
We next analyze the flow (or temporal ordering) of common IoCs across TI feeds. 
%
Specifically, in contrast to the IoC overlap analysis above, we take into account which feed publishes a common IoC before the other.
%
Figure~\ref{figure:sankey} plots a Sankey diagram to visualize the flow of IoCs across the top-10 TI feeds in our dataset. 
%
First, we note that some TI feeds are mainly the source of common IoCs. 
%
For example, {\CERTBund} is the source of approximately 84.8\% of its common IoCs.
%
Second, some TI feeds are mainly the sink of common IoCs. 
%
For example, {\DCSO} is mainly the sink of IoCs from {\CERTBund} and {\CIRCL}. 
%
This shows that {\DCSO} basically aggregates a subset of IoCs from multiple TI feeds.
%
Third, other feeds are more symmetric in being the sources/sinks of common IoCs.
%
For example, {\CIRCL} is the source of 68\% of its common IoCs with other feeds.
%
Thus, we conclude that TI feeds may have source/sink relationships for common IoCs with other feeds.



\begin{comment}

\begin{figure}[!t]
\centering
    %\includegraphics[width=0.8\columnwidth]{docs/figures/ip_addr_world_map.png}
    \includegraphics[width=1\columnwidth]{docs/figures/geolocation-maps/ip-threat-circl.pdf}
       \precaption
    \caption{Distribution of geolocated IP addresses for {\CIRCL} (left) and {\inThreat} (right)}
    \label{fig:geolocation}
    \postcaption
\end{figure}

\end{comment}

%\begin{figure}[H]
%\centering
    %\includegraphics[width=0.8\columnwidth]{docs/figures/ip_addr_world_map.png}
 %   \includegraphics[width=1\columnwidth]{docs/figures/geolocation-maps/ip-threat-{\CIRCL}-heat-map.png}
  %     \precaption
   % \caption{IP address ranges across different feeds.}
%    \label{fig:geolocation-heat}
 %   \postcaption
%\end{figure}



%\begin{figure}[!t]
    %\centering
    %\includegraphics[width=0.8\columnwidth]{docs/tag-frequency-breakdown.png}
   %    \precaption
   % \caption{Top feeds breakdown for frequency of tags}
   % \label{fig:FrequencyTagBreakdown}
   % \postcaption
%\end{figure}







\vspace{.05in} \noindent \textbf{Takeaways.} 
Our characterization highlighted three main insights. 
%
First, TI feeds contain various categories of information about different threats in a loosely-structured format. 
%
Second, the information in TI feeds and specific events is not static---it is dynamically updated and spread over often long time intervals. 
%
Third, TI feeds complement each other by providing differing amounts and types of IoCs but do sometimes contain redundant information. 
%
As we discuss next, there is a need to develop automated methods to analyze loosely-structured, spatio-temporal threat data in different TI feeds for downstream risk assessment, incident response, and patch management tasks. 




\begin{figure}[t!]
\centering
\includegraphics[width=0.6\columnwidth]{docs/figures/sankeys/sankey_anonymized.png}
    \caption{Flow of common IoCs across top-10 TI feeds. } %The left side shows counts of IoC sources and the right side shows the counts of IoC sinks.}
    \label{figure:sankey}
    \vspace{-0.2in}
\end{figure}




%Since tags are manually added and hold pertinent information, we conclude that they can be essential in verifying the focus of an event and determining highest priority incidents. 


% Unsure if Figure 6 + below analysis is needed
%Further, we analyze the distribution of tags to our largest feeds. This analysis was restricted to the top 9 feeds as they contain the majority of events in our dataset. Figure 6 consists of a breakdown indicating the number of tags per event for each feed. In most feeds, the events typically contain 2-3 tags with the most common being circl:incident-classification="malware", 'tlp:white', and misp-galaxy:banker="zeus". Since most events have at least two descriptive tags, we conclude that this additional classification can aid in determining highest priority incidents.%







%\noindent \textbf{Threat analysis.}
%A similarity we notice between events per feed was their assigned threat level. Next, we analyze the threat level ID assigned to each event by its feed organization. The following threat levels provide the risk level of an attack: 4 (undefined risk), 3 (low risk general malware), 2 (medium risk advanced persistent threats (APT)), and 1 (high risk sophisticated APTs and zero day attacks). Across all feeds, there are 212 level 1 events, 1026 level 2 events, 11612 level 3 events, and 1148 level 4 events. % Add comparison and contrast with CVSS risk scores

%Table 3 consists of ten feeds with the greatest quantity of threat level 1 events and their respective dominant IoC categories/types. Dominant IoC category/type pertains to the greatest IoC category/type percentage within that feed’s threat level 1 events. Based on this table, these feeds mostly contain IoCs within payload delivery and network analysis categories as shown by their over 50\% dominance in almost every feed. This is expected as hashes, domains, and ip addresses are common signs of compromise. Our data confirms this as the dominant IoC type column conveys the 4-type pattern the feeds follow: domain, filename, hashing algorithms, and IP address. In the {\INCIBE}, NCSC-NL, and {\CIRCL} feeds, IoCs of types sha1 “4bc2bbd1809c8b66eecd7c28ac319b948577de7b”, domain “myvalidation.info”, and ip-dst “83.229.62.212” report BlackEnergy malware, observed credential harvesting, and Turla command and control malware respectively. On the other hand, “nelis.at” is a phishing domain belonging to a level 3 event in the {\CIRCL} feed. As credential harvesting has a much higher vulnerability risk than a phishing domain, the distinction between level 1 and level 3 events is evident. By classifying the above events as threat level 1, organizations can prioritize patching attacks with the highest risk and monitor future IoC types/categories with similar activity. Thus, we conclude that high risk events tend to be classified as the above mentioned categories or types and recommend that specifically combating these types of IoCs may yield a more secure system. %





%
%Intuitively, the fact that  IoC categories and values  occur at multiple feeds  suggests that they can be used to  automatically process TI feed events.  
%
%In the following sections, we confirm that intuition by showing the feasibility of IoC-based text mining for classification of events  across  TI feeds.  


%The analysis of the rest of the feeds suggests that other TI feeds complement each other.
%Specifically, sometimes they are roughly equally the sources/sinks of common IoCs.
%For example, 
%and 60\% (1448/2429) 

%The analysis in this section  suggests that TI feeds   complement each other to the extent that they share   IoC categories (Table~\ref{table: statistics}) and  IoC values (Figures~\ref{fig:feed_overlap} and~\ref{figure:sankey}).  



%of its common IoCs while Feed 2 is the source of 83\% (1500/1807) of its common IoCs
%


%The overlap is because different TI feeds use the same source or when a large TI feed simply aggregates multiple smaller feeds.


%We define the flow between TI feeds $A$ and $B$ to be the number of common IoCs that are published by $A$ before $B$. 
%
%%%% The plot shows that smaller TI feeds often publish IoCs before larger TI feeds, which seem to be simply aggregating information from multiple smaller feeds.
%
%For example, ?? is the source of IoCs in CRICL and {\CERTBund}.
%
%%%% Thus, we conclude that while large TI feeds seem to subsume smaller TI feeds the latter are often the source of new IoCs. 
%
%%%% Thus, larger and smaller TI feeds complement each other in terms of coverage and speed. 
%The plot shows that there are  cycles of length two between certain  feeds, e.g., %, reflecting a balance between those pairs.  
%For instance, we find one such cycle between two of the top-3 feeds, as 
%

%zubair: can't figure our how to get these numbers from fig. 3
%Feed 0 publishes 166 IoCs before Feed 1 and, conversely, Feed 1 publishes 115 IoCs before Feed 0, reflecting a balance between that pair.  
%
%
%and
% We also find cycles of length greater than two, e.g., between   Feed 0, Feed 5, Feed 1 and Feed 0, that form a cycle of length three.

%forwards IoCs to Feed 5, which serves as a relay  to Feed 1, eventually forwarding IoCs back to Feed 0.




%With this visualization, it's possible to identify organizations that tend to be the first to publish IoCs. 

%This could be useful for pointing the contributors known for publishing inedited IoCs. We can also assess whether a contributor generates a concentrated flow or a branchy one, that is, the degree of collaborativeness. It's also possible to check for contributors that published
% many IoCs after many other sources. This characteristic is interesting for those who seek a source 
% that can summarize the IoCs already available out there.
 
 


%There is overlap, but who is the source
%- flow/sequence analysis
%- big feeds are not always the source


\begin{comment}
 We show diagrams for the following types of IoCs: artifacts dropped, payload installation, network activity and payload delivery.
Among the most important contributors, we highlight {\CIRCL}. It is the source with the higher amount of published inedited artifacts dropped. 
It also has one of the main roles on the flow of payloads installations. It's very interesting to observe that, for the types 
payload delivery and network activity, {\CIRCL} contributes to many organizations (i.e. publishes IoCs before them), and is benefited
from a variety of sources (publishes after them). Thus, {\CIRCL} is an essential contributor for two reasons: 
1) it is a good inaugurator of IoCs
2) it also relies on several other sources, being diverse

We envision that having such a strong contributor with these two characteristics enriches our dataset in terms of generalization.
We believe that {\CIRCL}, among other important organizations in our dataset, has a good representative power of IoCs reported 
on TI Feeds in the wild.
 
\end{comment}


\begin{comment}
\begin{figure}
  \begin{subfigure}[t]{0.57\columnwidth}
    \centering
    \includegraphics[width=1\columnwidth]{docs/figures/sankeys/artifacts_dropped.png}
    \caption{\textbf{Artifacts Dropped}}
  \end{subfigure}
  \hfill
  \begin{subfigure}[t]{0.57\columnwidth}
    \centering
    \includegraphics[width=\linewidth]{docs/figures/sankeys/network_activity.png}
    \caption{\textbf{Network Activity}}
  \end{subfigure}

  \medskip

  \begin{subfigure}[t]{0.57\columnwidth}
    \centering
    \includegraphics[width=\linewidth]{docs/figures/sankeys/payload_delivery_flow.png}
    \caption{\textbf{Payload Delivery} }
  \end{subfigure}
  \hfill
  \begin{subfigure}[t]{0.57\columnwidth}
    \centering
    \includegraphics[width=\linewidth]{docs/figures/sankeys/payload_installation.png}
    \caption{\textbf{Payload Installation}}
  \end{subfigure}
\end{figure}

\end{comment}






%TI feeds can be sourced from both public and private entities. 
%For example, {\InnoTecSystem}s \cite{InnoTec} is a private TI feed source while {\CIRCL} (Computer Incident Response Center Luxembourg) \cite{\CIRCL} is run by a government organization. 
%


%The time period of our data spans from 2013 to 2019, with 99.76 percent from the years of 2016-2019. 
%The breakdown of those years are as follows: 41.33\% from 2019, 29.11\% from 2018, 17.51\% from 2017, and 11.81\% from 2016.
%
%who are top TI vendors (public or private)rewrite for the top 10 
%\textbf{TI Vendors (public vs. private).}
%






%These timestamps are useful as there is a temporal aspect to cyberthreats \cite{sleeman2020temporal}. 


%
%In the case of events, the timestamp is consistent across the event. 
%While in the case of IOCs, the time stamps are individually generated. 
%Each IOC timestamp is generated in the range of the event it relates to. 
%
%




%
%This is of consideration as the event provides context for the IOCs, and the IOCs provide details for the event. 
%This balancing is important for a TI source that is both contextually rich and functionally detailed for a the purpose of containing actionable insights.
%


%\textbf{Event timespan.}



%each IoC is timestamped
%Discuss table1
%Correlation coef


%
%The amount of IOCs and the events they belong to are independent. 
%As shown in table 1 some TI feeds contain very few events with many IOCs, such as {{\inThreat}}.
%While others contain many events with few IOCs, such as InnotecSystem. 



%With assessing the volume of a feed the metric that used is distinct count of IOCs. 
%
%We chose this approach because the largest impact on our data are the IOCs and not the threat events themselves. 
%Altough the threat events provide context for the user, IOCs are the details of that event, and as such we determine that a higher volume of details is of greater importance when determining threats. 
%




%Of our top 10 IOC contributors the largest by volume are listed below in order from largest to smallest. 

\begin{comment}


\begin{enumerate}
  \item {\CERTBund} is a government run agency in Germany, it has been in operation since 2001. 
  \item {\CIRCL} (Computer Incident Response Luxembourg) is a government run agency from Luxembourg, and has been in operation since 2008. 
  \item {\inThreat} is a privately run organization from France that has been in operation since 2008. 
  \item {\InnoTecSystem} is a privately run organization from Spain that has been in operation since 2002. 
  \item {\CthulhuSPRL}  is a privately run organization from France that is currently in the provess of liquidation. 
  \item {\DCSO} is a privately run organization from Germany that has been in operation since 2015. It specializes in cyber espionage and theft.  
  \item {\Barncat}  is privately run company from the United States that has been in operation since 2002.
  \item {\Cryptolaemus} is an cybersecurity research group that is famous for its work on EMOTET. 
  \item {\Crimeware}? no information found (will ask matheus about this)
  \item {\INCIBE} is a government run organization from brazil that has been in operation since 2014
  
\end{enumerate}




\begin{enumerate}

\item \emph{Network activity} has data types consisting of IP addresses, hostnames, domains, and URLs. 

\item \emph{Payload delivery} consists of data types such as filenames, hashes, malware samples, and IP addresses.


\item \emph{External analysis} consists of data such as links to other organizations and their analysis of a particular IOC. 


\item \emph{Payload installation} contains hashes and filenames as well as expert textual description describing what was executed, what group or organization was responsible for the threat, and what campaign the samples are from. 


\item \emph{Artifacts dropped} are filenames and signatures resulting from a threat event. 

\end{enumerate}

%
%
%
%



%%IoT Categories (dominant IoC category)
%Figure 1; Table 1 (last column)
As we discuss next, the events in different TI feeds are geared towards different types of IOCs.
%
For instance, some TI feeds mostly contain network activity related IOCs such as IP addresses while others contain more rich textual analysis by security experts. 
Each IOC in our data is classified by category. In figure 1 the top 5 IOC categories are shown. These categories are self reported from each TI vendor, due to this self reporting and varying standards there is some ambiguity with these categories. 

Because of this we analysed the raw data to determine the meaning of these categories in the context of the data. Generally, with the top features there is very little variation with the IOC categories and raw data. However, with smaller IOC categories such as social networks, support tools and other; these categories are sparsely used by the majority of TI feeds.  These small categories contain raw data that is difficult to differentiate their meaning in context to larger categories. Although present in the data the volume of these ambiguous categories total less then 0.19\% of the total amount of IOCs. With this small of a percentage we are confident that the integrity of the remaining IOC categories is uncompromised. 


\end{comment}



%\subsubsection{Derived Features}A challenge with the use of hashes as IOCs is many are only unique to one event, that is they are not generalizable. As many threats have polymorphic capabilities to mask the file signature. To extract better information from this we created a derived feature from the hash data. This derived feature was made by counting how many times hashes appeared in a event. In addition to this derived feature we included other features that is not explicitly an IOC. This includes time stamps, related events, and number of total number of IOCs within each threat event.

%In contrast to the use of only TI feeds in developing threat intelligence, some researchers have gone to the forums where hackers share threat information and discuss exploits. There is evidence to suggest that these hacker forums may also have valuable threat data. \cite{nunes2016darknet}



%Payload delivery is similar to network activity but also includes file names and signatures. Payload delivery contains data from where the payload was from such as a URL, and the signature of the file delivered. Some of these IOCs contain descriptions if the payload delivery is a part of a greater campaign. This description provides better context for these features when compared to network activity that has little context description.

%\item xternal analysis is the third largest category in our data, at 38,531 IOCs. External analysis contains data that describes the behaviour or exist CVEs related to that sample. Some of this data may explain what ports were used to communicate or what system files were changed. Many of these are generated from virus total, amongst other services. External analysis overlaps with payload delivery and payload installation. As external analysis is performed on delivered or executed samples. 

%\item The fourth largest category is artifacts dropped, at 24,824 IOCs. %This category is similar to payload installation however the data is usually pieces from malicious activity. These can contain file samples, files that are potentially compromised, or other traces that some persistent threats leave behind. Although not as descriptive as payload installation this data has IOCs relating to novel threats. This is useful for finding previously unknown exploits. 

%\item The fifth largest category is payload installation, at 15,002 IOCs. Payload installation is similar in some aspects to payload delivery. The data types are similar, consisting of hashes and filenames. However payload installation differs to payload delivery by containing more expert textual description. Of all the categories payload installation has the most textual description. Explaining what the IOC does, what campaign it may be a part of, or what was the target of the threat. This is useful for existing exploits by finding similar behaviours and their corresponding exploits.  





\begin{comment}
\begin{figure}[!t]
    \centering
    \includegraphics[width=1.1\columnwidth]{docs/ioc-category-breakdown.png}
       \precaption
    \caption{Year-by-year category breakdown for top 10 feeds}
    \label{fig:TemporalCategoryBreakdown}
    \postcaption
\end{figure}

\begin{figure}[!t]
    \centering
    \includegraphics[width=\columnwidth]{docs/figures/ioc-by-day.png}
    \includegraphics[width=\columnwidth]{docs/figures/ioc-by-month.png}
    \precaption
    \caption{IoC Frequency By Day of Week and By Month Across Top 10 Feeds.}
    \label{fig:DayAndMonthTemporal}
    \postcaption
\end{figure}
\end{comment}

==> docs/discussion.tex <==

\section{Discussion}

Internal threats to validity: we take a risk averse approach, assuming that whenever we find a post/threat feed related to a given vulnerability, this represents a threat


\subsection{Threat feed classification}

in this paper, we focused on the classification of posts.  Alternatively, the classification of threat feeds is also of interest, accounting for their maturity,  information freshness and reliability.  This has been performed in related work using threat feed data that contained only IPs and hashes~\cite{li2019reading}, and we envision to extend that work with our  dataset which comprises richer features including textual description and so on. 



\section{Conclusion}

\section{Reading list}

Very relevant reference about blacklists (what can we do with IPs in our dataset?):~\cite{li2019reading}

Sharing feeds:~\cite{thomas2016abuse}

MISP~\cite{wagner2016misp} and \CIRCL \cite{mokaddem2019taxonomy, schaberreiter2019quantitative, ermerins2020scoring, rantos2020interoperability}

Temporal word embeddings \cite{shen2019attack2vec}
\cite{ramanathan2015learning}
\cite{volpetti2020temporal}




\begin{comment}
\begin{figure}[htp]
\centering
%\includegraphics[width=0.7\columnwidth]{explvul.png}
\caption{Number of vulnerabilities of each type (PoC, functional, high) as classified by IBM XForce, as a function of number of exploits, as collected from ExploitDB. This figures serves to illustrate the benefits of cross-relating multiple sources of data: for some vulnerabilities marked as ...}
\end{figure}



\begin{figure}
%    \includegraphics[width=1.0\columnwidth]{HeuristicasExploitability.png}
    \caption{Heuristic decision tree to classify exploits across  maturity levels: the classification of exploits naturally leads to classification of vulnerabilities. With vulnerabilities classified, we compare different sources of data, and can obtain insights about when/why a given source is more relevant for risk assessment. }
    \label{fig:my_label}
\end{figure}

\end{comment}

==> docs/graveyard.tex <==
\newpage

\section{motivation}
\label{sec:motivation}

%Overview - We approach information poisoning by creating a threat model
%% Threat model is motivated by TT and ADN
%%Well, I found some of the citations from section 3. 
As users browse web pages, browsing history and behavior (e.g. clicks) are used by OBA to infer their interests. 
%
User interests are a fundamental component of economic success of OBA. 
%
To begin, we examine two state of the art approaches to offensive privacy, \emph{AdNauseam}\cite{HoweNissenbauam2017EngineeringPrivacy} and \emph{\url{Trackthis.link}\cite{mozillatrackthis}}
%
Adnauseam (ADN) is a browser plugin designed to disrupt OBA by attacking its decision model. 
%
Upon activating ADN within a browser, it will execute clicks on every blocked ads, in order to register visits on the ad network and confuse advertisers.
%
Trackthis.link (TT) is a novel approach for incognito, which works by opening 100 tabs in browser to build a madness user profile and fool online trackers. 
%
Currently, it provides four types of madness tabs: Hypebeast, Filthy rich, doomsday and Influencer. However, one major limitation in both AdNauseam and Trackthis is that they do not consider the impact of browsing history on OBA. 
%
Instead, they aggressively take obfuscation strategies to achieve the maximal offensiveness (e.g. click all blocked ads or create 100 madness URLs), where the effectiveness and stealthiness are questionable. 
 
Therefore, in this section, we provide a comparison analysis of bids returned under different browsing profiles, in order to demonstrate that browsing history can be used to influence the outcome of online advertising auctions. Furthermore, to quantify the offensiveness of different privacy-preserving approaches, we collect the HB bids placed by advertiser as the offensiveness measurement.
% Introduce AdNauseum
% What is it 
%What are its goals
%% What are its limitations
%ADN 1) ADN's estimation of "expression" is inaccurate. 
% ADN 1a)DN's measurement of "expression" is based upon inaccurate estimations. (latest software reflects cost per click (CPC) estimations from 2015, although new estimations are published through 2020) 
%1b) ADN explicitily choses to be "vocal", by clicking on all detected ads (default setting when clicking is enabled). 



%Threat Model: 

% Actors: OBA, Publisher websites, Users.  

% Adversary: OBA

%% What is OBA and why OBA?
%% Components of OBA
%%% AD Networks - 
% The architecture and decision making appartus necessart to perform OBA. 
% architechture: RTB pipepline ( SSP, AdX, DSP, DMPs, bidders trackers) 
% Decision making Apparatus:   
% 1) ADX: given user information which bidders do I contact 
% 2) Bidders: given user information and customer alignment (goals, product, bottom line etc) how much is the users 
%    Information worth
% 3) what is is the most effective measage to present to this users. 
%% 
%%% Why OBA: user information if coverted to $$$ -> yeilding 



% Attacker: Users
%% What does the attacker know about the adversary 
%% What are the attacker's capbilities. 
%% What are the attacker's 
% Desired Outcome: 
%% Why is our method better? 
%
% We examine two state of the art approaches to 
% %

% The purpose of this work is to demonstrate that browsing history can be used to influence the outcome of online advertising auctions. 
% % 
% To this present a threat model 

% %
% We examine the state of the art in web history obfuscation. 
% %
% Adnauseum 
% \subsubsection{Threat model, attacker ,defender, overview of attack}
 
% Adnauseum 
% \subsubsection{Metrics}
% \begin{itemize}
%     \item quantify attack 
%     \item SOA, AD, TT
%     \item leading into data collection and results. 
    
    
% \end{itemize}


\subsection{Profile Construction}
To this end, we construct profiles by varying browsing history using different obfuscation strategies and measure their impact on the header bidding (HB) bids placed by advertisers. 
Specifically, we construct a profile by visiting (1) a set of profiling sites (10 in our study), (2) a set of bidding sites (5 in our study) to gather bids placed by advertisers. Our profiling sites derive from 23 categories in four site lists: Alexa top \footnote{\noindent https://www.alexa.com/topsites/category}, TrackThis, Adnauseum, and Intent, as shown in \T\ref{tab:sites}. In addition, we select 5 popular bidding sites for bids collection: \texttt{www.speedtest.net}, \texttt{www.realtor.com}, \texttt{www.ask.com}, \texttt{www.kompas.com}, and \texttt{www.cnn.com}. 

Moreover, to investigate the effects of intent URLs on OBA, we design two types of profiles: non-intent profile and intent profile. As illustrated in \F\ref{fig:profile}, the profiling sites in each non-intent profile consist of 10 URLs randomly selected from the same non-intent category. By contrast, only $k$ of the profiling sites in each intent profile are sampled from a non-intent category, and the rest $10-k$ will be chosen from the intent category ($k\in[5,9]$).

In all, we randomly generate 10 intent profiles and 10 non-intent profiles from each site category (400 in total) and measure their impacts on the 5 fixed bidding sites.
\label{sec:methods}
\begin{figure}[!t] 
  \centering 
  \includegraphics[width=1.0 \linewidth]{docs/figures/baseline.pdf}
\precaption
  \caption{Two types of profiles we designed.} 
\label{fig:profile} 
\end{figure} 
% \begin{table}[!htbp]
% \centering
% \caption{Two types of profiles with three methods.}
% \label{tab:profile}
% \begin{threeparttable}[t]
% \begin{tabular}{|c|c|c|}
% \hline
% \diagbox[width=5em,trim=l]{Methods}{Type} & Non-intent  & Intent \\ \hline
% Alexa & 10 Alexa URLs    & k Alexa URLs + (10-k) intent URLs \\ \hline
% TT    & 10 TT URLs       & k TT URLs + (10-k) intent URLs       \\ \hline
% AD    & 10 AD URLs       & k AD URLs + (10-k) intent URLs      \\ \hline    
% \end{tabular}
%      \begin{tablenotes}
%      \item[1] TT and AD represent Trackthis and Adnauseam respectively. And $k \in [5,9]$.
%   \end{tablenotes}
% \end{threeparttable}
% \end{table}
\begin{table}[!htbp]
\centering
\caption{Profiling site lists.}
\label{tab:sites}
\fontsize{9}{9}\selectfont
\begin{tabular}{ccccc}
\hline
~List name~&  ~Alexa top~  & ~Track this~ & ~Adnauseam~ & ~Intent~\\ \hline
\# of categories  &  17   & 4    &1    &1  \\ \hline
\# of URLs        &  800  & 400  & 100 & 100\\ \hline
\end{tabular}
\end{table}

\subsection{Bid Analysis}
In this subsection, we conduct a case study on the HB bids placed by bidder \textit{appnexus} for the main banner in \texttt{www.cnn.com}. Notably, we select bidder \textit{appnexus} since it returns the largest number of bids during our crawl. And \texttt{www.cnn.com} is the last bidding site we visit.

\F\ref{fig:RTBHB} demonstrates the average HB bids returned for both non-intent (blue, left bar) and intent profiles (red, right bar) by category. For non-intent profiles, we have observed that, in general, profiles constructed with sites from Alexa top categories trigger the highest bids (0.34 USD on average), compared with profiles built from Trackthis and AdNauseam site lists (0.21 USD and 0.23 USD on average). Specifically, for Alexa top site list, profiles built from recreation category obtain higher bid values (0.65 USD) than those from other categories. While in Trackthis site list, sites selected from Hypebeast category lead to the highest bids (0.30 USD). 

Furthermore, we find that compared with non-intent profiles from the same category, intent profiles increase the bid values by 1.39$\times$, 1.41$\times$, and 3.47$\times$ on average, in Alexa top, Track this, and Adnauseam site lists respectively. However, the effects of intent URLs on bid values will vary among different categories. Take the Alexa top site lists for example, intent URLs make profiles constructed from \textit{Health} category trigger 9.28$\times$ higher bids. By constrast, in \textit{Home} category, they show negative effects on the bid values. Similarly, intent profiles built from \textit{Doom} category in Track this site list achieve 2.28$\times$ increase in bid values, while reduce the bid values by 43\% in \textit{Hypebeast} category. 

Based on the above analysis, we can conclude that the browsing history indeed has significant impacts on the outcome of online advertising actions, especially for intent profiles. Moreover, two state of the art offensive obfuscation approach without considering the varying browsing history has limited effectiveness on triggering high bids.

% \begin{itemize}
    
%     \item high and low bids among categories
%     \item high and low bids among bidders 
    
% \end{itemize}
% \subsubsection{Quantifying browsing history}

% \begin{itemize}
%     \item average column across category high and low
%     \item high and low bids among categories
%     \item high and low bids among bidders 
    
% \end{itemize}
\begin{figure*}[!t] 
  \centering 
  \includegraphics[width=1.0 \textwidth]{docs/figures/gap1.eps}
\precaption
  \caption{Average HB bids returned from the main banner in \texttt{cnn.com} by category.} 
\label{fig:RTBHB} 
\end{figure*} 
% \subsubsection{Quantifying bidding behavior}
% \subsubsection{Quantifying buying intent}

% %
% We are interested in examining whether obfuscating browsing history impacts advertising. %
% In order to answer our first research question in \cref{tab:questions}, we conducted controlled web crawls.
% %
% We disabled caching in our browser to simulate a new user for each visit. 
% %
% We visit each webpage in  \cref{tab:volume} 20 times, half with AdNauseum Enabled.  
% %

% We capture the total resources download for each visit by saving its contents as a Http ARchive file (HAR). 

% \Cref{tab:volume} displays the total download size for each configuration. 
%significance testing? 

% \begin{table}[t]
% \scriptsize
% \centering
%   \begin{tabular}{p{.35in} >{\centering\arraybackslash}p{.70in}
%     >{\centering\arraybackslash}p{.70in} >{\centering\arraybackslash}p{.70in}}
%     \toprule
%     \multirow{2}{* }{Visit Seq.} & \multicolumn{2}{c}{Page Load Volume (MB)} \\
%                              & Disabled  & Enabled\\
%     \midrule
%     1& 10.7& 12.3 \\
%     2& 9.8& 13 \\
%     3& 11& 10.9 \\
%     4& 11& 10.9 \\
%     5& 12.3& 10.4 \\
%     6& 10.5& 11.7 \\
%     7& 10.1& 10.4 \\
%     8& 11.1& 9.2 \\ 
%     9& 11.1& 10.8 \\
%     10& 11.2& 12.5 \\

%     \midrule
%     Avg.& 10.9 &11.2 \\
%     Std.& 0.2 & 0.4 \\
%     \bottomrule
%   \end{tabular}
%   \caption{AdNauseum's impact on page load performance (cnn.com). }
%   \label{tab:volume}
%   \postcaption
% \end{table}


% \paratitle{Impact of browsing history on advertising.}
% %%moved 
% To this end, we constructed profiles by varying browsing history using different obfuscation strategies and measure its impact on the bids placed by advertisers. 
% %
% More specifically, we constructed a profile by visiting (1) a set of base sites, (2) a test site, and (3) a site to gather bids placed by advertisers. 
% %
% To promote realistic history, a base set of popular sites is included for each profile constructed. 
% %
% At web crawl run time, each profile's base is fix and yet differs by its test site . 
% We constructed the set of test sites using the following 3 strategies: 16 Alexa categories \cite{}, 4 TrackThis categories \cite{}, and advertising URLS detected by Adnauseum \cite{URL_ADNASUM_GITHUB}. 
%
% Finally, we collect bids by visiting a header bidding enabled website \cite{}
% 
%\cite{cook20headerbidding}. 
%CDF


%
%Client side header bidding auctions are visit 


%of 12 URL constructed from a fixed set of ten URLs selected from the Alexa top list \cite{}, a test website, selected from 1 of 22 categories) and a URL selected from a site that supports header bidding.  
%
%Each profile's base, test and header bidding site is visited in order, for each round of crawling. 

%1) price 
%To maximize the value browser, we systematic crawls by varying browsing  history across 
%2) information
%\paratitle{base profile crawling}

\subsection{RL for offensive obfuscation.} 
We conclude two significant limitations in existing offensive obfuscation approaches such as TrackThis and Adnauseam.
Firstly, they do not provide any offensiveness measurements as feedback and lack a learning process to improve their effectiveness and efficiency.
While they achieve offensiveness in an aggressive way, they cannot provide any utility and stealthiness guarantees.
Secondly, they click extension URLs in a independently and identically distributed fashion, without considering the correlation of URLs in browsing history.
To avoid these limitations, we utilize RL for offensive obfuscation in \ToolX, since RL can effectively learn policy for sequential decision making problem based on feedback.
%








\subsection{Feature Extraction/Selection}
With our data we performed feature extraction using three methods, binary features, TF-IDF and Doc2Vec. With binary features we one-hot encoded the data, if the feature was present in the event it was 1 and if it was not present it remained 0. This method was employed to give a baseline in what the initial performance could be expected in the models. Next we used TF-IDF which stands for term frequency over inverse document frequency. Unlike binary this method takes into account how often the feature is used in each document and how common it is amongst all documents. The final method we used for feature extraction is Doc2Vec. Doc2Vec is similar in some ways to word2vec. The high-level idea is that the document itself is represented as a n-dimensional vector. The Doc2Vec model attempts to group similar documents and thus give them similar vectors. We use both pre-trained doc2vec and custom made doc2vec. 

In addition to these extraction methods we also performed feature selection to remove extraneous features. For binary features and TF-IDF we chose the top k based off the variance. Features with low variance were not selected as they are likely not generalizable enough to be used in the models. With Doc2Vec we use a different method since the individual features are condensed into n-dimensional vectors. We used a parameter "vector size" to control how many vectors were used to describe a single document. To best compare the number of features from TF-IDF and Binary methods we matched the number of features to the number of vectors used for the Doc2Vec method. Due to the domain specific language in cybersecurity we wanted to measure the performance of a general use doc2vec model against our custom trained doc2vec. The pre-trained doc2vec model was trained with the entire corpus of Wikipedia, our model is trained with our own TI feed data. The pretrained doc2vec model generates 300-dimentional vectors only. Our models were made to generate 100,300,500,1000 vector outputs. The best performance is at 1000 vectors. In addition to this vector size parameter there is also the amount of steps used to infer a vector. Usually the higher the steps for inference the more likely two similar documents will converge. For our custom model we use 500 steps. 
%why did you use the sizes of vectors, 
%discuss any other parameters used


\subsection{pre-processing}
Before the features are generated we had to preprocess the data, this includes cleaning the data, creating derived features, and formatting. For binary features and TF-IDF the same method of pre-processing was used. This was performed by splitting the features on special characters, and removal of stopwords. After this was complete a derived feature was created for each event this feature was generated by a sentiment analyser.

Doc2Vec uses a stronger data cleaning method. It first removes any stop words, next it splits on all special characters. Next if there are features with a length over 30 characters or less then 2 characters the entire feature is removed. This results in more words being captured and less hashes or IP addresses being kept. The intuition behind this is to have the Doc2Vec model is not given data that is specific to one event such as a file signature. Instead we use this method of cleaning to better generalize the data the Doc2Vec model uses, and therefore generates. 
%Put this under feature selection near the end of doc2vec
%Due to the domain specific language in cybersecurity we wanted to measure the performance of a general use doc2vec model against our custom trained doc2vec. The pre-trained doc2vec model was trained with the entire corpus of Wikipedia, our model is trained with our own TI feed data. The pretrained doc2vec model generates 300-dimentional vecors only. Our models were made to generate 100,300,500,1000 vector outputs. The best performance is at 1000 vectors. In addition to this vector size parameter there is also the amount of steps used to infer a vector. Usually the higher the steps for inference the more likely two similar documents will converge. For our custom model we use 500 steps. 

\subsection{ML Models}
We use 3 machine learning models to classify our data. Naive Bayes, Decision Tree, and Ada boosted Decision trees. Naive Bays establishes a baseline for performance, as it is not a particularly effective model due to its simple design. The major limitation to the use of Naive Bayes it that it assumes total Independence between features. Decision trees do not have this limitation, as they allow for interdependence between features. Also decision tress come with a particular advantage, they are  interpretable, and their process easily explainable. For additional performance we use boosting. Boosting is the process of using many, low-fidelity learners and using them together in an iterative process. In the case of Adaboost incorrect predictions are given a higher weight, the more errors made for a specific prediction the higher the weight there is to correct that prediction. 



\vspace{.05in} \noindent \textbf{Overlap.}
Next, we analyze the overlap between IoCs across TI feeds.  
%
To this end, we restrict ourselves to IP and Hash IoCs overlapping across at least one pair of TI feeds. IP and Hash IoCs were chosen because the specific nature of these IoC types lends them to be representative of commonality between feeds. (\hl{I am unsure if this is a strong enough reason, but this is the reasoning Ashton gave me (I believe the previous paper had this restriction as well}).
%
For $n$ total feeds, the percentage of overlap between Feed $i$ (row value) and Feed $j$ (column value) in each cell in Figure~\ref{fig:feed_overlap} is calculated as follows:

\[ \text{Overlap}_{ij} = \frac{|Feed \thinspace i \cap Feed \thinspace j|}{|\bigcup_{k=1, k\neq i, k \neq j}^n (Feed \thinspace k \cap Feed \thinspace i)|} \]

Note that, in the above formula, the denominator excludes the overlap between the same feeds.


%%
\hl{font size in figure}
Figure~\ref{fig:feed_overlap} shows that among the IP and Hash IoCs that are shared with another feed by \CIRCL,  25.4\% of these shared IoCs specifically have the same value as an IoC generated by \DCSO, e.g., the same IP address or Hash value.
\hl{don't get the above sentence. please unpack}
% 
The dark vertical streak shows that many TI feeds tend to share a large fraction of their IoCs with CRICL.
%
For example, four TI feeds (\inThreat, \InnoTecSystem, \CthulhuSPRL, \INCIBE) on average share ?\% of their IoCs with \CIRCL. 
%
Two other feeds (\DCSO, \Cryptolaemus) also share a majority (\hl{?\%}) of their IoCs with CERT-Bund.
%
Such overlap is expected and has been reported in prior work on IP blocklists \cite{li19tealeaves,Ramanathan20blacklists}.
%The overlap is because different TI feeds use the same source or when a large TI feed simply aggregates multiple smaller feeds.



\begin{figure}[!t]
    \centering
    \includegraphics[width=1.1\columnwidth]{docs/ioc-overlap-raw-count.png}
       \precaption
    \caption{IoC overlap across top-10 TI feeds for IPs and Hashes. Note that some TI feeds, in particular \CIRCL, share common IoCs with several other TI feeds. (only considered hashes and ips)}
    \label{fig:feed_overlap}
    \postcaption
\end{figure}

\begin{figure}[!t]
    \centering
    \includegraphics[width=1.1\columnwidth]{docs/figures/similarity-heatmap.png}
       \precaption
    \caption{URL, Link, and Domain similarity across top-10 TI feeds}
    \label{fig:similarity_heatmap}
%    \postcaption
\end{figure}


%To further dig into differential contribution of different TI feeds, w

%%
We next analyze the flow (or temporal ordering) of common IoCs across TI feeds. 
%
Specifically, in contrast to the IoC overlap analysis above, we take into account which feed  publishes a common IoC before the other.
%
Figure~\ref{figure:sankey} plots a Sankey diagram to visualize the flow of IoCs across the top-10 TI feeds. 
%
%Similar to as was done for Figure~\ref{fig:feed_overlap}, analysis was restricted to IP and Hash IoCs. 
%
First, we note that some TI feeds are mainly the source of common IoCs. 
%
For example, CERT-Bund is the source of approximately 84.8\% of its common IoCs.
%
Second, some TI feeds are mainly the sink of common IoCs. 
%
For example, \DCSO is mainly the sink of IoCs from CERT-Bund and \CIRCL. 
%
This shows that \DCSO basically aggregates a subset of IoCs from multiple TI feeds.
%
Third, other feeds are more symmetric in being the sources/sinks of common IoCs.
%
For example, \CIRCL is the source of 68\% of its common IoCs with other feeds \hl{can we find another feed closer to 50\%}.
%
\hl{Thus, we conclude that most TI feeds complement each other in terms of timing (or information freshness). -- I don't think this is the right conclusion?}

\noindent \textbf{IoC Similarity.}
\hl{what's our motivation to go from same-to-similar?}
Next, we analyze the IoC similarity across the top 10 feeds. 
%
For this purpose, we focus on IoCs of categories url, link, or domain. We define similarity as when two IoCs share the same "base domain" value (e.g., a value of http://efax.pfdregistry.org/efax/37486.zip would have a "base domain" of efax.pfdregistry.org).


%%
Figure~\ref{fig:similarity_heatmap} shows that feeds tend to share many IoCs of the same "base domains," even if the exact values differ. Some of the most common "base domains" across the top 10 feeds include virustotal.com, 185.234.216.52, ..., b4ckdoorarchive.com, and dropbox.com. In particular, it is interesting to note that \CIRCL shares significant similarity of url, link, and domain IoCs with nearly each of the other top 10 feeds, respectively. This is in sharp contrast to the other feeds, which share a much less uniform distribution of similarity with other feeds in terms of "base domains".

\begin{figure}[!t]
    \centering
    \includegraphics[width=1.1\columnwidth]{docs/figures/similarity-heatmap.png}
       \precaption
    \caption{URL, Link, and Domain similarity across top-10 TI feeds}
    \label{fig:similarity_heatmap}
%    \postcaption
\end{figure}

\textit{Pre-processing:}
Before features are extracted, we conduct standard pre-processing such as splitting the text on all special characters such as hyphens and removal of stop words. 
%
Words with length over 30 characters, which typically correspond to file hashes, receive special treatment, as indicated below, and are then removed. 

\textit{Feature extraction:}
We consider three different approaches for  feature extraction: binary feature extraction, TF-IDF and Doc2Vec \cite{le2014distributed}. 
%
First, binary feature extraction corresponds to a one-hot encoding of words in an event. 
%
Second, TF-IDF feature extraction corresponds to a numerical statistic accounting for how often a word is used in an event and amongst all events. 
%
Third, Doc2Vec, also combines local and global information by representing each event (``doc'') as an $n$-dimensional vector (``vec'').
%
We use an off-the-shelf pre-trained Doc2Vec embedding that is trained in an unsupervised manner using the entire Wikipedia corpus of Wikipedia.
%
The vocabulary size of this pre-trained embedding is 915,715 tokens.
%
We also train a customized word embedding, called {TI2Vec}, in an unsupervised manner using the corpus of 191 TI feeds in our dataset.
%
Training is done over 15 epochs.
%
The resulting vocabulary size is 4,242 tokens.
%
The insight behind training a purpose-built word embedding is to capture the context of domain-specific vocabulary that is typically used in TI feeds. 


\textit{Out-of-band features:}
Out-of-band features are derived from data using domain knowledge. 
%
Some IoCs, such as  hashes, might refer to a malware payload, and require special treatment.  
%
As threats have polymorphic capabilities to mask file signatures, most hashes are unique to one feed.
%
This, in turn, implies that information about hashes cannot be readily generalizable across feeds.   
%
To address this issue, we derive the count of how many times different hashes appeared in an event.
%
Additional out-of-band features include a count of  distinct timestamps (similar to the count of hashes) and the count of IoCs in an event.
%
Sentiment is   another out-of-band feature.  
%
We leverage an off-the-shelf sentiment analysis tool, which  given a textual input, returns a polarity score measuring how positive or negative is a given piece of text~\cite{hutto2014vader}.  



\textit{Feature selection:}
We perform feature selection to avoid over-fitting.
%
We choose the top-$K$ features with highest  variance~\cite{cai2010unsupervised} for binary and TF-IDF feature sets. 
%
For Doc2Vec, recall that each document is characterized by an $n$-dimensional vector.
%
Feature selection consists of parsimoniously  choosing   $n$. 
%
The pre-trained Doc2Vec embedding uses $n$=300.
%
For {TI2Vec}, we select $n$ to be 100, 300, 500, and 1000. 



\noindent \textbf{Supervised classification.}
Given the features and labeled dataset, we train different supervised machine learning algorithms to classify TI feed events.  
%
We begin by considering naive Bayes and decision tree classifiers, as both serve to classify  non-linearly separable classes, with naive Bayes relying on conditional independence among features for that purpose.  
%
Following the discussion in Section~\ref{sec: data}, there are significant inter-dependencies across features within each class, suggesting that decision trees are better suited than naive Bayes. 
%
As a natural extension to  decision trees, 
we also consider the AdaBoost ensemble classifier.  
%
Boosting in that context consists of using many  low-fidelity decision trees, which together are supposed to outperform a single tree. 
%
While the decision tree is amenable to interpretability, ensemble classifiers tend to provide better classification performance.

\noindent \textbf{Impact of feature sets.}
Our customized word embedding (TI2Vec) turns out to be a much better feature extraction approach than binary, TF-IDF, or pre-trained Doc2Vec. 
%
In contrast to binary and TF-IDF, TI2Vec is unique in that it avoids the limitations of handcrafted simple word features. 
%
In contrast to pre-trained Doc2Vec, TI2Vec embedding is learnt in an unsupervised manner from a large corpus of IoC data from many different TI feeds.  
%
By doing so, \textsc{TI2Vec}  captures the context of  security events in TI feeds, being able to  better characterize its similarity to other security events when compared against other feature extraction approaches. 
%
% Specifically, TF-IDF is not contextually aware of similar or dissimilar events,  as it is based on  individual words in the whole data set. 
%
Specifically, TF-IDF is not contextually aware of similar or  dissimilar events, as it is computed based on individual words without considering cross-word relations within documents.
%
Binary feature set is even simpler as it does not capture relative term-document frequency information. 
%
The pre-trained Doc2Vec is contextual by design but is trained on generic document corpus \cite{dai2015document, lau2016empirical, niu2015topic2vec} that is not specific to the vocabulary in TI feeds. 
%
Thus, we expect our domain-specific TI2Vec to be advantageous to a domain-agnostic pre-trained Doc2Vec model. 






\noindent \textbf{Impact of feature selection.}
We use unsupervised approaches to limit the number of selected features.
%
Using the top-$K$ in terms of variance, we selected $K$= 100, 300, 500, and 1000 features to train our models. 
%
We note that the accuracy of the binary feature set improves with more features. 
%
In TF-IDF, there is a plateauing effect that occurs as more features are added. 
%
There is no general trend in TI2Vec---the accuracy can slightly increase or decrease with more features.  
%
Overall, the most accurate AdaBoost model does indeed perform better with more features, while simpler models such as decision trees suffer from the curse of dimensionality, performing worse with more features. 


\noindent \textbf{Impact of classifiers.}
Comparing machine learning classifiers, we note that AdaBoost outperforms naive Bayes and decision tree. 
%
Different classifiers appear to handle the precision-recall tradeoff differently. 
%
For instance, the decision tree classifier is inclined to optimize for precision while the naive Bayes classifier is inclined to optimize for recall.
%
These trends are the most apparent for the TF-IDF feature set, where the decision tree classifier gets 83\% precision and 37\% recall while the naive Bayes classifier gets 50\% precision and 98\% recall.
%
AdaBoost achieves a good balance between precision and recall. 
%
For the TF-IDF feature set, the average difference between precision and recall for AdaBoost is only 1\%.



\noindent \textbf{Interpretability of decision tree model.}
Figure \ref{fig:tree} shows a pruned decision tree model for the TF-IDF feature set.
%
The decision tree model is interpretable and can provide useful insights about IoCs that are more likely to indicate exploitation events.  
%
The features at the higher levels of the  tree have more distinguishing power than lower level features.
%
The root node at the top of the tree is ``njrat'', which is a remote access trojan   used in multiple attack campaigns.
%
The presence of this word indicates exploitation for more than one-fifth of relevant TI feed events with perfect accuracy. 
%
In the absence of ``njrat'' the presence of ``darkcomet'', a remote access trojan like njrat, indicates exploitation for 9\% of TI feed events in our data with perfect accuracy.
%
Other similar words such as ``ransomware'' also indicate exploitation.  
%
Although not shown here due to space constraints, out-of-band features such as sentiment also show up in a less pruned version of the decision tree.  


\begin{figure}[!t]
\precaption
    \centering
    \includegraphics[width=0.5\columnwidth]{docs/figures/decision_trees/tree_tifeeds(3)(7).png}
    \caption{Pruned decision tree for the TF-IDF feature set. Leaf nodes show (\textcolor{red}{error\%}, \textcolor{blue}{population size\%}). Note that certain words that appear in the tree are strongly indicative of exploitation events.
    }
    \label{fig:tree}
   \postcaption
\end{figure}

\noindent \textbf{Takeaway.}
The results show that a supervised machine learning classifier using our customized TI2Vec embedding is able to more accurately detect exploitation events in TI feeds than the one using a pre-trained Doc2Vec embedding. 
%
This shows that our purpose-built embedding is able to suitably capture the semantics from loosely structured information in TI feeds.

\begin{figure}[H]
    \centering
  %  \vspace{-0.5in}
    \includegraphics[width=1\columnwidth]{docs/figures/decision_trees/partial_dtc_binary.png}
       \precaption
    \caption{Pruned decision tree for binary feature extraction and specific split method}
    \label{fig: binary decision tree}
    \postcaption
\end{figure}

\begin{figure}[H]
    \centering
  %  \vspace{-0.5in}
    \includegraphics[width=1\columnwidth]{docs/figures/decision_trees/partial_dtc_tfidf.png}
       \precaption
    \caption{Pruned decision tree for TF-IDF feature extraction and specific split method}
    \label{fig: tfidf decision tree}
    \postcaption
\end{figure}

\begin{table}[H]
\centering
\caption{Temporal and Spatial train test split meta information. All other temporal and spatial tables’ evaluation id column corresponds to the train test splits shown here}
{\fontsize{4}{4}\selectfont
\arrayrulecolor{black}
\begin{tabular}{!{\color{black}\vrule}l!{\color{black}\vrule}l!{\color{black}\vrule}r!{\color{black}\vrule}r!{\color{black}\vrule}l!{\color{black}\vrule}l!{\color{black}\vrule}r!{\color{black}\vrule}} 
\arrayrulecolor{black}\cline{1-1}\arrayrulecolor{black}\cline{2-7}
Train and Split Test Type          & Feed Omitted   & \multicolumn{1}{l!{\color{black}\vrule}}{Train Length} & \multicolumn{1}{l!{\color{black}\vrule}}{Test Length} & Train Date Range         & Test Date Range          & \multicolumn{1}{l!{\color{black}\vrule}}{Evaluation Id}  \\ 
\arrayrulecolor{black}\cline{1-1}\arrayrulecolor{black}\cline{2-7}
\multirow{7}{*}{Specific Time}     & \CERTBund      & 9732                                                   & 576                                                   & 2009-03-29 to 2017-10-13 & 2017-10-13 to 2019-05-12 & 1                                                        \\ 
\cline{2-7}
                                   & \CIRCL          & 8877                                                   & 311                                                   & 2011-06-22 to 2017-10-13 & 2017-10-16 to 2019-05-09 & 1                                                        \\ 
\cline{2-7}
                                   & \Crimeware      & 9663                                                   & 1                                                     & 2009-03-29 to 2017-10-13 & 2017-12-29 to 2017-12-29 & 1                                                        \\ 
\cline{2-7}
                                   & \CthulhuSPRL  & 9686                                                   & 6                                                     & 2009-03-29 to 2017-10-13 & 2017-10-16 to 2019-03-28 & 1                                                        \\ 
\cline{2-7}
                                   & \DCSO           & 9747                                                   & 177                                                   & 2009-03-29 to 2017-10-13 & 2017-10-16 to 2019-02-14 & 1                                                        \\ 
\cline{2-7}
                                   & \INCIBE         & 9746                                                   & 1                                                     & 2009-03-29 to 2017-10-13 & 2018-11-16 to 2018-11-16 & 1                                                        \\ 
\cline{2-7}
                                   & \inThreat   & 9767                                                   & 97                                                    & 2009-03-29 to 2017-10-13 & 2017-10-27 to 2019-05-07 & 1                                                        \\ 
\hline
\multirow{41}{*}{Window Equal}     & \CIRCL          & 1211                                                   & 3                                                     & 2011-06-22 to 2015-02-28 & 2015-03-06 to 2015-03-31 & 1                                                        \\ 
\cline{2-7}
                                   & \CthulhuSPRL  & 1271                                                   & 2                                                     & 2009-03-29 to 2015-02-28 & 2015-03-30 to 2015-04-03 & 1                                                        \\ 
\cline{2-7}
                                   & \CIRCL          & 1269                                                   & 21                                                    & 2015-02-28 to 2015-04-07 & 2015-04-16 to 2015-06-26 & 2                                                        \\ 
\cline{2-7}
                                   & \CthulhuSPRL  & 1270                                                   & 12                                                    & 2015-02-28 to 2015-04-07 & 2015-04-12 to 2015-06-24 & 2                                                        \\ 
\cline{2-7}
                                   & \CIRCL          & 1251                                                   & 35                                                    & 2015-04-07 to 2015-06-28 & 2015-07-08 to 2015-12-04 & 3                                                        \\ 
\cline{2-7}
                                   & \CthulhuSPRL  & 1260                                                   & 29                                                    & 2015-04-07 to 2015-06-28 & 2015-06-29 to 2015-11-18 & 3                                                        \\ 
\cline{2-7}
                                   & \CIRCL          & 1237                                                   & 135                                                   & 2015-06-28 to 2015-12-07 & 2015-12-09 to 2016-03-09 & 4                                                        \\ 
\cline{2-7}
                                   & \CthulhuSPRL  & 1243                                                   & 22                                                    & 2015-06-28 to 2015-12-07 & 2015-12-11 to 2016-02-23 & 4                                                        \\ 
\cline{2-7}
                                   & \INCIBE         & 1272                                                   & 18                                                    & 2015-06-28 to 2015-12-07 & 2016-01-20 to 2016-03-10 & 4                                                        \\ 
\cline{2-7}
                                   & \CIRCL          & 1137                                                   & 98                                                    & 2015-12-07 to 2016-03-10 & 2016-03-10 to 2016-05-19 & 5                                                        \\ 
\cline{2-7}
                                   & \CthulhuSPRL  & 1250                                                   & 3                                                     & 2015-12-07 to 2016-03-10 & 2016-04-22 to 2016-05-13 & 5                                                        \\ 
\cline{2-7}
                                   & \INCIBE         & 1254                                                   & 9                                                     & 2015-12-07 to 2016-03-10 & 2016-03-10 to 2016-04-29 & 5                                                        \\ 
\cline{2-7}
                                   & \CERTBund      & 1270                                                   & 20                                                    & 2016-03-10 to 2016-05-20 & 2016-08-26 to 2017-03-28 & 6                                                        \\ 
\cline{2-7}
                                   & \CIRCL          & 1174                                                   & 328                                                   & 2016-03-10 to 2016-05-20 & 2016-05-20 to 2017-03-31 & 6                                                        \\ 
\cline{2-7}
                                   & \Crimeware      & 1272                                                   & 131                                                   & 2016-03-10 to 2016-05-20 & 2016-07-05 to 2017-03-22 & 6                                                        \\ 
\cline{2-7}
                                   & \CthulhuSPRL  & 1269                                                   & 30                                                    & 2016-03-10 to 2016-05-20 & 2016-06-07 to 2017-02-22 & 6                                                        \\ 
\cline{2-7}
                                   & \DCSO           & 1272                                                   & 11                                                    & 2016-03-10 to 2016-05-20 & 2016-08-12 to 2017-02-28 & 6                                                        \\ 
\cline{2-7}
                                   & \INCIBE         & 1263                                                   & 11                                                    & 2016-03-10 to 2016-05-20 & 2016-05-27 to 2017-02-17 & 6                                                        \\ 
\cline{2-7}
                                   & \inThreat   & 1272                                                   & 18                                                    & 2016-03-10 to 2016-05-20 & 2016-06-23 to 2017-03-02 & 6                                                        \\ 
\cline{2-7}
                                   & \CERTBund      & 1252                                                   & 77                                                    & 2016-05-20 to 2017-03-31 & 2017-04-04 to 2017-12-18 & 7                                                        \\ 
\cline{2-7}
                                   & \CIRCL          & 944                                                    & 306                                                   & 2016-05-20 to 2017-03-31 & 2017-04-04 to 2017-12-18 & 7                                                        \\ 
\cline{2-7}
                                   & \Crimeware      & 1141                                                   & 6                                                     & 2016-05-20 to 2017-03-31 & 2017-04-07 to 2017-04-14 & 7                                                        \\ 
\cline{2-7}
                                   & \CthulhuSPRL  & 1242                                                   & 9                                                     & 2016-05-20 to 2017-03-31 & 2017-06-14 to 2017-11-02 & 7                                                        \\ 
\cline{2-7}
                                   & \DCSO           & 1261                                                   & 52                                                    & 2016-05-20 to 2017-03-31 & 2017-04-28 to 2017-12-12 & 7                                                        \\ 
\cline{2-7}
                                   & \INCIBE         & 1261                                                   & 16                                                    & 2016-05-20 to 2017-03-31 & 2017-04-03 to 2017-09-20 & 7                                                        \\ 
\cline{2-7}
                                   & \inThreat   & 1254                                                   & 20                                                    & 2016-05-20 to 2017-03-31 & 2017-04-10 to 2017-12-19 & 7                                                        \\ 
\cline{2-7}
                                   & \CERTBund      & 1195                                                   & 61                                                    & 2017-04-03 to 2017-12-19 & 2017-12-19 to 2018-06-26 & 8                                                        \\ 
\cline{2-7}
                                   & \CIRCL          & 966                                                    & 111                                                   & 2017-04-03 to 2017-12-19 & 2017-12-19 to 2018-06-26 & 8                                                        \\ 
\cline{2-7}
                                   & \Crimeware      & 1266                                                   & 1                                                     & 2017-04-03 to 2017-12-19 & 2017-12-29 to 2017-12-29 & 8                                                        \\ 
\cline{2-7}
                                   & \CthulhuSPRL  & 1263                                                   & 3                                                     & 2017-04-03 to 2017-12-19 & 2018-01-11 to 2018-02-21 & 8                                                        \\ 
\cline{2-7}
                                   & \DCSO           & 1220                                                   & 63                                                    & 2017-04-03 to 2017-12-19 & 2017-12-22 to 2018-06-14 & 8                                                        \\ 
\cline{2-7}
                                   & \inThreat   & 1252                                                   & 24                                                    & 2017-04-03 to 2017-12-19 & 2017-12-19 to 2018-05-30 & 8                                                        \\ 
\cline{2-7}
                                   & \CERTBund      & 1211                                                   & 94                                                    & 2017-12-19 to 2018-06-26 & 2018-06-26 to 2018-11-27 & 9                                                        \\ 
\cline{2-7}
                                   & \CIRCL          & 1161                                                   & 61                                                    & 2017-12-19 to 2018-06-26 & 2018-06-26 to 2018-11-27 & 9                                                        \\ 
\cline{2-7}
                                   & \DCSO           & 1209                                                   & 70                                                    & 2017-12-19 to 2018-06-26 & 2018-06-26 to 2018-11-28 & 9                                                        \\ 
\cline{2-7}
                                   & \INCIBE         & 1272                                                   & 1                                                     & 2017-12-19 to 2018-06-26 & 2018-11-16 to 2018-11-16 & 9                                                        \\ 
\cline{2-7}
                                   & \inThreat   & 1248                                                   & 21                                                    & 2017-12-19 to 2018-06-26 & 2018-07-26 to 2018-10-08 & 9                                                        \\ 
\cline{2-7}
                                   & \CERTBund      & 1178                                                   & 389                                                   & 2018-06-26 to 2018-11-28 & 2018-11-29 to 2019-05-12 & 10                                                       \\ 
\cline{2-7}
                                   & \CIRCL          & 1211                                                   & 67                                                    & 2018-06-26 to 2018-11-28 & 2018-11-29 to 2019-05-09 & 10                                                       \\ 
\cline{2-7}
                                   & \DCSO           & 1202                                                   & 34                                                    & 2018-06-26 to 2018-11-28 & 2018-12-01 to 2019-02-14 & 10                                                       \\ 
\cline{2-7}
                                   & \inThreat   & 1251                                                   & 47                                                    & 2018-06-26 to 2018-11-28 & 2019-03-07 to 2019-05-07 & 10                                                       \\ 
\hline
\multirow{41}{*}{Window Aggregate} & \CIRCL          & 1211                                                   & 3                                                     & 2011-06-22 to 2015-02-28 & 2015-03-06 to 2015-03-31 & 1                                                        \\ 
\cline{2-7}
                                   & \CthulhuSPRL  & 1271                                                   & 2                                                     & 2009-03-29 to 2015-02-28 & 2015-03-30 to 2015-04-03 & 1                                                        \\ 
\cline{2-7}
                                   & \CIRCL          & 2480                                                   & 21                                                    & 2011-06-22 to 2015-04-07 & 2015-04-16 to 2015-06-26 & 2                                                        \\ 
\cline{2-7}
                                   & \CthulhuSPRL  & 2541                                                   & 12                                                    & 2009-03-29 to 2015-04-07 & 2015-04-12 to 2015-06-24 & 2                                                        \\ 
\cline{2-7}
                                   & \CIRCL          & 3731                                                   & 35                                                    & 2011-06-22 to 2015-06-28 & 2015-07-08 to 2015-12-04 & 3                                                        \\ 
\cline{2-7}
                                   & \CthulhuSPRL  & 3801                                                   & 29                                                    & 2009-03-29 to 2015-06-28 & 2015-06-29 to 2015-11-18 & 3                                                        \\ 
\cline{2-7}
                                   & \CIRCL          & 4968                                                   & 135                                                   & 2011-06-22 to 2015-12-07 & 2015-12-09 to 2016-03-09 & 4                                                        \\ 
\cline{2-7}
                                   & \CthulhuSPRL  & 5044                                                   & 22                                                    & 2009-03-29 to 2015-12-07 & 2015-12-11 to 2016-02-23 & 4                                                        \\ 
\cline{2-7}
                                   & \INCIBE         & 5096                                                   & 18                                                    & 2009-03-29 to 2015-12-07 & 2016-01-20 to 2016-03-10 & 4                                                        \\ 
\cline{2-7}
                                   & \CIRCL          & 6105                                                   & 98                                                    & 2011-06-22 to 2016-03-10 & 2016-03-10 to 2016-05-19 & 5                                                        \\ 
\cline{2-7}
                                   & \CthulhuSPRL  & 6294                                                   & 3                                                     & 2009-03-29 to 2016-03-10 & 2016-04-22 to 2016-05-13 & 5                                                        \\ 
\cline{2-7}
                                   & \INCIBE         & 6350                                                   & 9                                                     & 2009-03-29 to 2016-03-10 & 2016-03-10 to 2016-04-29 & 5                                                        \\ 
\cline{2-7}
                                   & \CERTBund      & 7637                                                   & 20                                                    & 2009-03-29 to 2016-05-20 & 2016-08-26 to 2017-03-28 & 6                                                        \\ 
\cline{2-7}
                                   & \CIRCL          & 7279                                                   & 328                                                   & 2011-06-22 to 2016-05-20 & 2016-05-20 to 2017-03-31 & 6                                                        \\ 
\cline{2-7}
                                   & \Crimeware      & 7640                                                   & 131                                                   & 2009-03-29 to 2016-05-20 & 2016-07-05 to 2017-03-22 & 6                                                        \\ 
\cline{2-7}
                                   & \CthulhuSPRL  & 7563                                                   & 30                                                    & 2009-03-29 to 2016-05-20 & 2016-06-07 to 2017-02-22 & 6                                                        \\ 
\cline{2-7}
                                   & \DCSO           & 7640                                                   & 11                                                    & 2009-03-29 to 2016-05-20 & 2016-08-12 to 2017-02-28 & 6                                                        \\ 
\cline{2-7}
                                   & \INCIBE         & 7613                                                   & 11                                                    & 2009-03-29 to 2016-05-20 & 2016-05-27 to 2017-02-17 & 6                                                        \\ 
\cline{2-7}
                                   & \inThreat   & 7640                                                   & 18                                                    & 2009-03-29 to 2016-05-20 & 2016-06-23 to 2017-03-02 & 6                                                        \\ 
\cline{2-7}
                                   & \CERTBund      & 8889                                                   & 77                                                    & 2009-03-29 to 2017-03-31 & 2017-04-04 to 2017-12-18 & 7                                                        \\ 
\cline{2-7}
                                   & \CIRCL          & 8223                                                   & 306                                                   & 2011-06-22 to 2017-03-31 & 2017-04-04 to 2017-12-18 & 7                                                        \\ 
\cline{2-7}
                                   & \Crimeware      & 8781                                                   & 6                                                     & 2009-03-29 to 2017-03-31 & 2017-04-07 to 2017-04-14 & 7                                                        \\ 
\cline{2-7}
                                   & \CthulhuSPRL  & 8805                                                   & 9                                                     & 2009-03-29 to 2017-03-31 & 2017-06-14 to 2017-11-02 & 7                                                        \\ 
\cline{2-7}
                                   & \DCSO           & 8901                                                   & 52                                                    & 2009-03-29 to 2017-03-31 & 2017-04-28 to 2017-12-12 & 7                                                        \\ 
\cline{2-7}
                                   & \INCIBE         & 8874                                                   & 16                                                    & 2009-03-29 to 2017-03-31 & 2017-04-03 to 2017-09-20 & 7                                                        \\ 
\cline{2-7}
                                   & \inThreat   & 8894                                                   & 20                                                    & 2009-03-29 to 2017-03-31 & 2017-04-10 to 2017-12-19 & 7                                                        \\ 
\cline{2-7}
                                   & \CERTBund      & 10084                                                  & 61                                                    & 2009-03-29 to 2017-12-19 & 2017-12-19 to 2018-06-26 & 8                                                        \\ 
\cline{2-7}
                                   & \CIRCL          & 9189                                                   & 111                                                   & 2011-06-22 to 2017-12-19 & 2017-12-19 to 2018-06-26 & 8                                                        \\ 
\cline{2-7}
                                   & \Crimeware      & 10047                                                  & 1                                                     & 2009-03-29 to 2017-12-19 & 2017-12-29 to 2017-12-29 & 8                                                        \\ 
\cline{2-7}
                                   & \CthulhuSPRL  & 10068                                                  & 3                                                     & 2009-03-29 to 2017-12-19 & 2018-01-11 to 2018-02-21 & 8                                                        \\ 
\cline{2-7}
                                   & \DCSO           & 10121                                                  & 63                                                    & 2009-03-29 to 2017-12-19 & 2017-12-22 to 2018-06-14 & 8                                                        \\ 
\cline{2-7}
                                   & \inThreat   & 10146                                                  & 24                                                    & 2009-03-29 to 2017-12-19 & 2017-12-19 to 2018-05-30 & 8                                                        \\ 
\cline{2-7}
                                   & \CERTBund      & 11295                                                  & 94                                                    & 2009-03-29 to 2018-06-26 & 2018-06-26 to 2018-11-27 & 9                                                        \\ 
\cline{2-7}
                                   & \CIRCL          & 10350                                                  & 61                                                    & 2011-06-22 to 2018-06-26 & 2018-06-26 to 2018-11-27 & 9                                                        \\ 
\cline{2-7}
                                   & \DCSO           & 11330                                                  & 70                                                    & 2009-03-29 to 2018-06-26 & 2018-06-26 to 2018-11-28 & 9                                                        \\ 
\cline{2-7}
                                   & \INCIBE         & 11402                                                  & 1                                                     & 2009-03-29 to 2018-06-26 & 2018-11-16 to 2018-11-16 & 9                                                        \\ 
\cline{2-7}
                                   & \inThreat   & 11394                                                  & 21                                                    & 2009-03-29 to 2018-06-26 & 2018-07-26 to 2018-10-08 & 9                                                        \\ 
\cline{2-7}
                                   & \CERTBund      & 12473                                                  & 389                                                   & 2009-03-29 to 2018-11-28 & 2018-11-29 to 2019-05-12 & 10                                                       \\ 
\cline{2-7}
                                   & \CIRCL          & 11561                                                  & 67                                                    & 2011-06-22 to 2018-11-28 & 2018-11-29 to 2019-05-09 & 10                                                       \\ 
\cline{2-7}
                                   & \DCSO           & 12532                                                  & 34                                                    & 2009-03-29 to 2018-11-28 & 2018-12-01 to 2019-02-14 & 10                                                       \\ 
\cline{2-7}
                                   & \inThreat   & 12645                                                  & 47                                                    & 2009-03-29 to 2018-11-28 & 2019-03-07 to 2019-05-07 & 10                                                       \\
\hline
\end{tabular}
}
\arrayrulecolor{black}
\end{table}

% \usepackage{multirow}
% \usepackage{colortbl}


\begin{table}[H]
\centering
\caption{Binary Temporal and Spatial Results. This uses 1000 features and a tree depth of 10 for Decision Tree and AdaBoost. The results are (precision, recall, F1). Note that the results for the Specific Time Split are omitted from this table as Specific Time Split only has one split and, thus, the results are identical to that in the table showing the weighted averages.}
{\fontsize{4}{4}\selectfont
\arrayrulecolor{black}
\begin{tabular}{!{\color{black}\vrule}l!{\color{black}\vrule}l!{\color{black}\vrule}r!{\color{black}\vrule}l!{\color{black}\vrule}l!{\color{black}\vrule}l!{\color{black}\vrule}} 
\arrayrulecolor{black}\cline{1-1}\arrayrulecolor{black}\cline{2-6}
Train and Split Test Type          & Feed Omitted  & \multicolumn{1}{l!{\color{black}\vrule}}{Evaluation Id} & NB                 & DTree              & Ada                 \\ 
\arrayrulecolor{black}\cline{1-1}\arrayrulecolor{black}\cline{2-6}
\multirow{41}{*}{Window Equal}     & \CIRCL          & 1                                                       & Ignore             & Ignore             & Ignore              \\ 
\cline{2-6}
                                   & \CthulhuSPRL  & 1                                                       & Ignore             & Ignore             & Ignore              \\ 
\cline{2-6}
                                   & \CIRCL          & 2                                                       & Ignore             & Ignore             & Ignore              \\ 
\cline{2-6}
                                   & \CthulhuSPRL  & 2                                                       & Ignore             & Ignore             & Ignore              \\ 
\cline{2-6}
                                   & \CIRCL          & 3                                                       & Ignore             & Ignore             & Ignore              \\ 
\cline{2-6}
                                   & \CthulhuSPRL  & 3                                                       & Ignore             & Ignore             & Ignore              \\ 
\cline{2-6}
                                   & \CIRCL          & 4                                                       & Ignore             & Ignore             & Ignore              \\ 
\cline{2-6}
                                   & \CthulhuSPRL  & 4                                                       & Ignore             & Ignore             & Ignore              \\ 
\cline{2-6}
                                   & \INCIBE         & 4                                                       & (1.0, 0.06, 0.11)  & Ignore             & (1.0, 0.12, 0.21)   \\ 
\cline{2-6}
                                   & \CIRCL          & 5                                                       & (0.5, 0.01, 0.03)  & (0.86, 0.08, 0.14) & Ignore              \\ 
\cline{2-6}
                                   & \CthulhuSPRL  & 5                                                       & Ignore             & Ignore             & Ignore              \\ 
\cline{2-6}
                                   & \INCIBE         & 5                                                       & Ignore             & Ignore             & Ignore              \\ 
\cline{2-6}
                                   & \CERTBund      & 6                                                       & (0.44, 0.78, 0.56) & (0.0, 0.0, 0.0)    & (0.0, 0.0, 0.0)     \\ 
\cline{2-6}
                                   & \CIRCL          & 6                                                       & (0.33, 0.01, 0.01) & (0.44, 0.09, 0.14) & (0.0, 0.0, 0.0)     \\ 
\cline{2-6}
                                   & \Crimeware      & 6                                                       & (0.02, 0.67, 0.04) & (0.0, 0.0, 0.0)    & (0.0, 0.0, 0.0)     \\ 
\cline{2-6}
                                   & \CthulhuSPRL  & 6                                                       & (0.0, 0.0, 0.0)    & (0.33, 0.14, 0.2)  & (0.0, 0.0, 0.0)     \\ 
\cline{2-6}
                                   & \DCSO           & 6                                                       & (0.0, 0.0, 0.0)    & (1.0, 0.33, 0.5)   & Ignore              \\ 
\cline{2-6}
                                   & \INCIBE         & 6                                                       & (0.67, 0.22, 0.33) & Ignore             & (0.0, 0.0, 0.0)     \\ 
\cline{2-6}
                                   & \inThreat   & 6                                                       & (0.0, 0.0, 0.0)    & (0.5, 0.11, 0.18)  & Ignore              \\ 
\cline{2-6}
                                   & \CERTBund      & 7                                                       & (0.19, 0.93, 0.32) & (0.25, 0.07, 0.11) & (0.0, 0.0, 0.0)     \\ 
\cline{2-6}
                                   & \CIRCL          & 7                                                       & (0.39, 0.23, 0.29) & (0.62, 0.14, 0.23) & (0.5, 0.05, 0.09)   \\ 
\cline{2-6}
                                   & \Crimeware      & 7                                                       & (0.17, 1.0, 0.29)  & Ignore             & Ignore              \\ 
\cline{2-6}
                                   & \CthulhuSPRL  & 7                                                       & (0.83, 0.62, 0.71) & Ignore             & Ignore              \\ 
\cline{2-6}
                                   & \DCSO           & 7                                                       & (0.88, 0.65, 0.75) & (0.75, 0.07, 0.13) & (1.0, 0.05, 0.09)   \\ 
\cline{2-6}
                                   & \INCIBE         & 7                                                       & (0.75, 0.75, 0.75) & Ignore             & Ignore              \\ 
\cline{2-6}
                                   & \inThreat   & 7                                                       & (0.82, 0.82, 0.82) & (1.0, 0.12, 0.21)  & (0.75, 0.18, 0.29)  \\ 
\cline{2-6}
                                   & \CERTBund      & 8                                                       & (0.35, 0.44, 0.39) & (0.0, 0.0, 0.0)    & (0.31, 0.22, 0.26)  \\ 
\cline{2-6}
                                   & \CIRCL          & 8                                                       & (0.55, 0.62, 0.58) & (0.56, 0.22, 0.31) & (0.65, 0.23, 0.34)  \\ 
\cline{2-6}
                                   & \Crimeware      & 8                                                       & (1.0, 1.0, 1.0)    & Ignore             & Ignore              \\ 
\cline{2-6}
                                   & \CthulhuSPRL  & 8                                                       & (1.0, 1.0, 1.0)    & (1.0, 0.33, 0.5)   & (1.0, 0.67, 0.8)    \\ 
\cline{2-6}
                                   & \DCSO           & 8                                                       & (0.58, 0.39, 0.47) & (0.6, 0.25, 0.35)  & (0.56, 0.14, 0.22)  \\ 
\cline{2-6}
                                   & \inThreat   & 8                                                       & (1.0, 0.83, 0.91)  & (1.0, 0.04, 0.08)  & (1.0, 0.42, 0.59)   \\ 
\cline{2-6}
                                   & \CERTBund      & 9                                                       & (0.46, 0.88, 0.61) & (0.0, 0.0, 0.0)    & (0.4, 0.05, 0.09)   \\ 
\cline{2-6}
                                   & \CIRCL          & 9                                                       & (0.71, 0.41, 0.52) & (0.78, 0.17, 0.28) & Ignore              \\ 
\cline{2-6}
                                   & \DCSO           & 9                                                       & (0.94, 0.52, 0.67) & (0.86, 0.09, 0.16) & (0.71, 0.08, 0.14)  \\ 
\cline{2-6}
                                   & \INCIBE         & 9                                                       & (1.0, 1.0, 1.0)    & Ignore             & Ignore              \\ 
\cline{2-6}
                                   & \inThreat   & 9                                                       & (1.0, 0.62, 0.76)  & (1.0, 0.05, 0.09)  & (1.0, 0.05, 0.09)   \\ 
\cline{2-6}
                                   & \CERTBund      & 10                                                      & (0.07, 0.67, 0.12) & (0.07, 0.21, 0.1)  & (0.06, 0.21, 0.09)  \\ 
\cline{2-6}
                                   & \CIRCL          & 10                                                      & (0.85, 0.51, 0.64) & (0.81, 0.31, 0.45) & (1.0, 0.4, 0.57)    \\ 
\cline{2-6}
                                   & \DCSO           & 10                                                      & (1.0, 0.76, 0.87)  & (1.0, 0.38, 0.55)  & (1.0, 0.53, 0.69)   \\ 
\cline{2-6}
                                   & \inThreat   & 10                                                      & (0.95, 0.91, 0.93) & (1.0, 0.04, 0.09)  & (0.94, 0.76, 0.84)  \\ 
\hline
\multirow{41}{*}{Window Aggregate} & \CIRCL          & 1                                                       & Ignore             & Ignore             & Ignore              \\ 
\cline{2-6}
                                   & \CthulhuSPRL  & 1                                                       & Ignore             & Ignore             & Ignore              \\ 
\cline{2-6}
                                   & \CIRCL          & 2                                                       & Ignore             & (1.0, 0.05, 0.1)   & Ignore              \\ 
\cline{2-6}
                                   & \CthulhuSPRL  & 2                                                       & Ignore             & Ignore             & Ignore              \\ 
\cline{2-6}
                                   & \CIRCL          & 3                                                       & Ignore             & Ignore             & Ignore              \\ 
\cline{2-6}
                                   & \CthulhuSPRL  & 3                                                       & Ignore             & Ignore             & Ignore              \\ 
\cline{2-6}
                                   & \CIRCL          & 4                                                       & Ignore             & Ignore             & Ignore              \\ 
\cline{2-6}
                                   & \CthulhuSPRL  & 4                                                       & Ignore             & Ignore             & Ignore              \\ 
\cline{2-6}
                                   & \INCIBE         & 4                                                       & (0.5, 0.06, 0.11)  & (1.0, 0.06, 0.11)  & (1.0, 0.06, 0.11)   \\ 
\cline{2-6}
                                   & \CIRCL          & 5                                                       & (0.67, 0.03, 0.05) & (1.0, 0.01, 0.03)  & Ignore              \\ 
\cline{2-6}
                                   & \CthulhuSPRL  & 5                                                       & (1.0, 0.5, 0.67)   & Ignore             & Ignore              \\ 
\cline{2-6}
                                   & \INCIBE         & 5                                                       & (1.0, 0.22, 0.36)  & Ignore             & Ignore              \\ 
\cline{2-6}
                                   & \CERTBund      & 6                                                       & (0.47, 1.0, 0.64)  & Ignore             & Ignore              \\ 
\cline{2-6}
                                   & \CIRCL          & 6                                                       & (0.53, 0.29, 0.37) & (0.5, 0.03, 0.06)  & (0.33, 0.01, 0.02)  \\ 
\cline{2-6}
                                   & \Crimeware      & 6                                                       & (0.02, 0.67, 0.03) & (0.0, 0.0, 0.0)    & (0.0, 0.0, 0.0)     \\ 
\cline{2-6}
                                   & \CthulhuSPRL  & 6                                                       & (0.3, 0.86, 0.44)  & Ignore             & Ignore              \\ 
\cline{2-6}
                                   & \DCSO           & 6                                                       & (0.12, 0.33, 0.18) & (0.0, 0.0, 0.0)    & (0.0, 0.0, 0.0)     \\ 
\cline{2-6}
                                   & \INCIBE         & 6                                                       & (0.8, 0.89, 0.84)  & Ignore             & Ignore              \\ 
\cline{2-6}
                                   & \inThreat   & 6                                                       & (0.5, 1.0, 0.67)   & (0.0, 0.0, 0.0)    & (0.0, 0.0, 0.0)     \\ 
\cline{2-6}
                                   & \CERTBund      & 7                                                       & (0.15, 0.6, 0.24)  & Ignore             & Ignore              \\ 
\cline{2-6}
                                   & \CIRCL          & 7                                                       & (1.0, 0.01, 0.01)  & (0.71, 0.03, 0.07) & (0.71, 0.03, 0.07)  \\ 
\cline{2-6}
                                   & \Crimeware      & 7                                                       & (0.0, 0.0, 0.0)    & Ignore             & (0.0, 0.0, 0.0)     \\ 
\cline{2-6}
                                   & \CthulhuSPRL  & 7                                                       & (0.75, 0.38, 0.5)  & Ignore             & Ignore              \\ 
\cline{2-6}
                                   & \DCSO           & 7                                                       & (0.9, 0.21, 0.34)  & Ignore             & Ignore              \\ 
\cline{2-6}
                                   & \INCIBE         & 7                                                       & (0.75, 0.25, 0.38) & (1.0, 0.08, 0.15)  & Ignore              \\ 
\cline{2-6}
                                   & \inThreat   & 7                                                       & (0.86, 0.71, 0.77) & Ignore             & Ignore              \\ 
\cline{2-6}
                                   & \CERTBund      & 8                                                       & (0.24, 0.67, 0.35) & Ignore             & Ignore              \\ 
\cline{2-6}
                                   & \CIRCL          & 8                                                       & (0.61, 0.27, 0.37) & (0.67, 0.03, 0.06) & (0.5, 0.02, 0.03)   \\ 
\cline{2-6}
                                   & \Crimeware      & 8                                                       & Ignore             & Ignore             & Ignore              \\ 
\cline{2-6}
                                   & \CthulhuSPRL  & 8                                                       & (1.0, 0.67, 0.8)   & Ignore             & Ignore              \\ 
\cline{2-6}
                                   & \DCSO           & 8                                                       & (0.62, 0.36, 0.46) & (0.67, 0.06, 0.1)  & (1.0, 0.03, 0.05)   \\ 
\cline{2-6}
                                   & \inThreat   & 8                                                       & (1.0, 0.08, 0.15)  & Ignore             & Ignore              \\ 
\cline{2-6}
                                   & \CERTBund      & 9                                                       & (0.48, 0.88, 0.62) & (0.0, 0.0, 0.0)    & (0.5, 0.02, 0.05)   \\ 
\cline{2-6}
                                   & \CIRCL          & 9                                                       & (0.53, 0.2, 0.29)  & (0.5, 0.02, 0.05)  & Ignore              \\ 
\cline{2-6}
                                   & \DCSO           & 9                                                       & (0.88, 0.21, 0.34) & (1.0, 0.02, 0.03)  & Ignore              \\ 
\cline{2-6}
                                   & \INCIBE         & 9                                                       & (1.0, 1.0, 1.0)    & Ignore             & Ignore              \\ 
\cline{2-6}
                                   & \inThreat   & 9                                                       & (1.0, 0.05, 0.09)  & Ignore             & Ignore              \\ 
\cline{2-6}
                                   & \CERTBund      & 10                                                      & (0.06, 0.96, 0.12) & (0.0, 0.0, 0.0)    & Ignore              \\ 
\cline{2-6}
                                   & \CIRCL          & 10                                                      & (0.85, 0.91, 0.88) & Ignore             & Ignore              \\ 
\cline{2-6}
                                   & \DCSO           & 10                                                      & (1.0, 0.97, 0.99)  & Ignore             & Ignore              \\ 
\cline{2-6}
                                   & \inThreat   & 10                                                      & (0.92, 0.24, 0.39) & (1.0, 0.04, 0.09)  & Ignore              \\
\hline
\end{tabular}
}
\arrayrulecolor{black}
\end{table}

% \usepackage{multirow}
% \usepackage{colortbl}



\begin{table}[H]
\centering
\caption{TF-IDF Temporal and Spatial Results. This uses 1000 features and a tree depth of 10 for Decision Tree and AdaBoost. The results are (precision, recall, F1). Note that the results for the Specific Time Split are omitted from this table as Specific Time Split only has one split and, thus, the results are identical to that in the table showing the weighted averages.}
{\fontsize{4}{4}\selectfont
\arrayrulecolor{black}
\begin{tabular}{!{\color{black}\vrule}l!{\color{black}\vrule}l!{\color{black}\vrule}r!{\color{black}\vrule}l!{\color{black}\vrule}l!{\color{black}\vrule}l!{\color{black}\vrule}} 
\arrayrulecolor{black}\cline{1-1}\arrayrulecolor{black}\cline{2-6}
Train and Split Test Type          & Feed Omitted  & \multicolumn{1}{l!{\color{black}\vrule}}{Evaluation Id} & NB                 & DTree              & Ada                 \\ 
\arrayrulecolor{black}\cline{1-1}\arrayrulecolor{black}\cline{2-6}
\multirow{41}{*}{Window Equal}     & \CIRCL          & 1                                                       & Ignore             & Ignore             & Ignore              \\ 
\cline{2-6}
                                   & \CthulhuSPRL  & 1                                                       & Ignore             & Ignore             & Ignore              \\ 
\cline{2-6}
                                   & \CIRCL          & 2                                                       & Ignore             & Ignore             & Ignore              \\ 
\cline{2-6}
                                   & \CthulhuSPRL  & 2                                                       & Ignore             & Ignore             & Ignore              \\ 
\cline{2-6}
                                   & \CIRCL          & 3                                                       & Ignore             & Ignore             & Ignore              \\ 
\cline{2-6}
                                   & \CthulhuSPRL  & 3                                                       & Ignore             & Ignore             & Ignore              \\ 
\cline{2-6}
                                   & \CIRCL          & 4                                                       & Ignore             & Ignore             & Ignore              \\ 
\cline{2-6}
                                   & \CthulhuSPRL  & 4                                                       & Ignore             & Ignore             & Ignore              \\ 
\cline{2-6}
                                   & \INCIBE         & 4                                                       & (1.0, 0.06, 0.11)  & (1.0, 0.06, 0.11)  & Ignore              \\ 
\cline{2-6}
                                   & \CIRCL          & 5                                                       & Ignore             & Ignore             & Ignore              \\ 
\cline{2-6}
                                   & \CthulhuSPRL  & 5                                                       & Ignore             & Ignore             & Ignore              \\ 
\cline{2-6}
                                   & \INCIBE         & 5                                                       & Ignore             & Ignore             & Ignore              \\ 
\cline{2-6}
                                   & \CERTBund      & 6                                                       & (0.44, 0.44, 0.44) & (0.5, 0.11, 0.18)  & (0.5, 0.11, 0.18)   \\ 
\cline{2-6}
                                   & \CIRCL          & 6                                                       & (0.5, 0.02, 0.04)  & (0.43, 0.09, 0.15) & (0.67, 0.02, 0.05)  \\ 
\cline{2-6}
                                   & \Crimeware      & 6                                                       & (0.0, 0.0, 0.0)    & (0.05, 0.33, 0.09) & (0.0, 0.0, 0.0)     \\ 
\cline{2-6}
                                   & \CthulhuSPRL  & 6                                                       & (0.0, 0.0, 0.0)    & (0.17, 0.14, 0.15) & (0.0, 0.0, 0.0)     \\ 
\cline{2-6}
                                   & \DCSO           & 6                                                       & (1.0, 0.33, 0.5)   & Ignore             & Ignore              \\ 
\cline{2-6}
                                   & \INCIBE         & 6                                                       & (0.8, 0.44, 0.57)  & (1.0, 0.11, 0.2)   & Ignore              \\ 
\cline{2-6}
                                   & \inThreat   & 6                                                       & (0.0, 0.0, 0.0)    & (0.5, 0.22, 0.31)  & (1.0, 0.11, 0.2)    \\ 
\cline{2-6}
                                   & \CERTBund      & 7                                                       & (0.21, 0.87, 0.34) & (0.25, 0.07, 0.11) & (0.0, 0.0, 0.0)     \\ 
\cline{2-6}
                                   & \CIRCL          & 7                                                       & (0.37, 0.19, 0.25) & (0.45, 0.06, 0.11) & (0.17, 0.01, 0.01)  \\ 
\cline{2-6}
                                   & \Crimeware      & 7                                                       & (1.0, 1.0, 1.0)    & Ignore             & (0.0, 0.0, 0.0)     \\ 
\cline{2-6}
                                   & \CthulhuSPRL  & 7                                                       & (0.86, 0.75, 0.8)  & (1.0, 0.12, 0.22)  & Ignore              \\ 
\cline{2-6}
                                   & \DCSO           & 7                                                       & (0.92, 0.26, 0.4)  & (0.6, 0.07, 0.12)  & Ignore              \\ 
\cline{2-6}
                                   & \INCIBE         & 7                                                       & (0.86, 0.5, 0.63)  & (1.0, 0.08, 0.15)  & (1.0, 0.08, 0.15)   \\ 
\cline{2-6}
                                   & \inThreat   & 7                                                       & (1.0, 0.53, 0.69)  & (0.67, 0.24, 0.35) & (0.75, 0.18, 0.29)  \\ 
\cline{2-6}
                                   & \CERTBund      & 8                                                       & (0.31, 0.5, 0.38)  & (0.19, 0.28, 0.23) & (0.18, 0.11, 0.14)  \\ 
\cline{2-6}
                                   & \CIRCL          & 8                                                       & (0.5, 0.42, 0.46)  & (0.6, 0.19, 0.29)  & (0.46, 0.19, 0.27)  \\ 
\cline{2-6}
                                   & \Crimeware      & 8                                                       & Ignore             & Ignore             & Ignore              \\ 
\cline{2-6}
                                   & \CthulhuSPRL  & 8                                                       & (1.0, 1.0, 1.0)    & (1.0, 0.33, 0.5)   & Ignore              \\ 
\cline{2-6}
                                   & \DCSO           & 8                                                       & (0.57, 0.36, 0.44) & (0.5, 0.14, 0.22)  & (0.56, 0.14, 0.22)  \\ 
\cline{2-6}
                                   & \inThreat   & 8                                                       & (1.0, 0.88, 0.93)  & (1.0, 0.08, 0.15)  & (1.0, 0.04, 0.08)   \\ 
\cline{2-6}
                                   & \CERTBund      & 9                                                       & (0.42, 0.74, 0.53) & (1.0, 0.02, 0.05)  & (0.78, 0.17, 0.27)  \\ 
\cline{2-6}
                                   & \CIRCL          & 9                                                       & (0.9, 0.22, 0.35)  & (0.67, 0.05, 0.09) & Ignore              \\ 
\cline{2-6}
                                   & \DCSO           & 9                                                       & (0.91, 0.15, 0.26) & (1.0, 0.05, 0.09)  & Ignore              \\ 
\cline{2-6}
                                   & \INCIBE         & 9                                                       & (1.0, 1.0, 1.0)    & Ignore             & Ignore              \\ 
\cline{2-6}
                                   & \inThreat   & 9                                                       & (1.0, 0.62, 0.76)  & Ignore             & Ignore              \\ 
\cline{2-6}
                                   & \CERTBund      & 10                                                      & (0.06, 0.54, 0.11) & (0.01, 0.04, 0.02) & (0.03, 0.04, 0.04)  \\ 
\cline{2-6}
                                   & \CIRCL          & 10                                                      & (0.82, 0.33, 0.47) & (0.84, 0.38, 0.53) & (0.83, 0.45, 0.59)  \\ 
\cline{2-6}
                                   & \DCSO           & 10                                                      & (1.0, 0.56, 0.72)  & (1.0, 0.76, 0.87)  & (1.0, 0.62, 0.76)   \\ 
\cline{2-6}
                                   & \inThreat   & 10                                                      & (0.97, 0.62, 0.76) & (1.0, 0.09, 0.16)  & (0.88, 0.31, 0.46)  \\ 
\hline
\multirow{41}{*}{Window Aggregate} & \CIRCL          & 1                                                       & Ignore             & Ignore             & Ignore              \\ 
\cline{2-6}
                                   & \CthulhuSPRL  & 1                                                       & Ignore             & Ignore             & Ignore              \\ 
\cline{2-6}
                                   & \CIRCL          & 2                                                       & Ignore             & Ignore             & Ignore              \\ 
\cline{2-6}
                                   & \CthulhuSPRL  & 2                                                       & Ignore             & (1.0, 0.08, 0.15)  & Ignore              \\ 
\cline{2-6}
                                   & \CIRCL          & 3                                                       & Ignore             & Ignore             & Ignore              \\ 
\cline{2-6}
                                   & \CthulhuSPRL  & 3                                                       & Ignore             & (1.0, 0.03, 0.07)  & Ignore              \\ 
\cline{2-6}
                                   & \CIRCL          & 4                                                       & Ignore             & Ignore             & Ignore              \\ 
\cline{2-6}
                                   & \CthulhuSPRL  & 4                                                       & (1.0, 0.05, 0.09)  & Ignore             & Ignore              \\ 
\cline{2-6}
                                   & \INCIBE         & 4                                                       & (0.5, 0.06, 0.11)  & Ignore             & Ignore              \\ 
\cline{2-6}
                                   & \CIRCL          & 5                                                       & (0.6, 0.04, 0.07)  & (1.0, 0.01, 0.03)  & Ignore              \\ 
\cline{2-6}
                                   & \CthulhuSPRL  & 5                                                       & Ignore             & Ignore             & Ignore              \\ 
\cline{2-6}
                                   & \INCIBE         & 5                                                       & (1.0, 0.22, 0.36)  & Ignore             & Ignore              \\ 
\cline{2-6}
                                   & \CERTBund      & 6                                                       & (0.5, 0.67, 0.57)  & Ignore             & Ignore              \\ 
\cline{2-6}
                                   & \CIRCL          & 6                                                       & (0.52, 0.3, 0.38)  & (0.13, 0.01, 0.02) & (0.17, 0.01, 0.01)  \\ 
\cline{2-6}
                                   & \Crimeware      & 6                                                       & (0.0, 0.0, 0.0)    & Ignore             & Ignore              \\ 
\cline{2-6}
                                   & \CthulhuSPRL  & 6                                                       & (0.38, 0.71, 0.5)  & Ignore             & Ignore              \\ 
\cline{2-6}
                                   & \DCSO           & 6                                                       & (0.33, 1.0, 0.5)   & (1.0, 0.33, 0.5)   & Ignore              \\ 
\cline{2-6}
                                   & \INCIBE         & 6                                                       & (0.75, 0.67, 0.71) & Ignore             & Ignore              \\ 
\cline{2-6}
                                   & \inThreat   & 6                                                       & (0.5, 0.56, 0.53)  & (0.5, 0.22, 0.31)  & (0.67, 0.22, 0.33)  \\ 
\cline{2-6}
                                   & \CERTBund      & 7                                                       & (0.36, 0.33, 0.34) & Ignore             & Ignore              \\ 
\cline{2-6}
                                   & \CIRCL          & 7                                                       & (0.75, 0.04, 0.08) & (0.0, 0.0, 0.0)    & Ignore              \\ 
\cline{2-6}
                                   & \Crimeware      & 7                                                       & Ignore             & Ignore             & Ignore              \\ 
\cline{2-6}
                                   & \CthulhuSPRL  & 7                                                       & (0.8, 0.5, 0.62)   & Ignore             & Ignore              \\ 
\cline{2-6}
                                   & \DCSO           & 7                                                       & (1.0, 0.19, 0.31)  & (1.0, 0.02, 0.05)  & (1.0, 0.02, 0.05)   \\ 
\cline{2-6}
                                   & \INCIBE         & 7                                                       & (1.0, 0.08, 0.15)  & Ignore             & Ignore              \\ 
\cline{2-6}
                                   & \inThreat   & 7                                                       & (0.75, 0.18, 0.29) & Ignore             & Ignore              \\ 
\cline{2-6}
                                   & \CERTBund      & 8                                                       & (0.26, 0.67, 0.38) & Ignore             & Ignore              \\ 
\cline{2-6}
                                   & \CIRCL          & 8                                                       & (0.46, 0.17, 0.25) & (0.75, 0.05, 0.09) & Ignore              \\ 
\cline{2-6}
                                   & \Crimeware      & 8                                                       & (1.0, 1.0, 1.0)    & Ignore             & Ignore              \\ 
\cline{2-6}
                                   & \CthulhuSPRL  & 8                                                       & (1.0, 0.67, 0.8)   & Ignore             & Ignore              \\ 
\cline{2-6}
                                   & \DCSO           & 8                                                       & (0.62, 0.44, 0.52) & Ignore             & Ignore              \\ 
\cline{2-6}
                                   & \inThreat   & 8                                                       & (1.0, 0.29, 0.45)  & Ignore             & Ignore              \\ 
\cline{2-6}
                                   & \CERTBund      & 9                                                       & (0.46, 0.79, 0.58) & (0.5, 0.02, 0.05)  & Ignore              \\ 
\cline{2-6}
                                   & \CIRCL          & 9                                                       & (0.44, 0.1, 0.16)  & (1.0, 0.02, 0.05)  & Ignore              \\ 
\cline{2-6}
                                   & \DCSO           & 9                                                       & (0.88, 0.35, 0.5)  & (1.0, 0.02, 0.03)  & Ignore              \\ 
\cline{2-6}
                                   & \INCIBE         & 9                                                       & (1.0, 1.0, 1.0)    & Ignore             & Ignore              \\ 
\cline{2-6}
                                   & \inThreat   & 9                                                       & (1.0, 0.62, 0.76)  & Ignore             & Ignore              \\ 
\cline{2-6}
                                   & \CERTBund      & 10                                                      & (0.07, 0.58, 0.12) & Ignore             & (0.0, 0.0, 0.0)     \\ 
\cline{2-6}
                                   & \CIRCL          & 10                                                      & (0.8, 0.44, 0.56)  & Ignore             & (1.0, 0.02, 0.04)   \\ 
\cline{2-6}
                                   & \DCSO           & 10                                                      & (1.0, 0.79, 0.89)  & Ignore             & Ignore              \\ 
\cline{2-6}
                                   & \inThreat   & 10                                                      & (0.95, 0.91, 0.93) & (0.5, 0.02, 0.04)  & (0.5, 0.02, 0.04)   \\
\hline
\end{tabular}
\arrayrulecolor{black}
}
\end{table}

% \usepackage{multirow}
% \usepackage{colortbl}

\begin{table}[H]
\centering
\caption{TI2Vec Temporal and Spatial Results. This uses 1000 features and a tree depth of 4 for Decision Tree and AdaBoost. The results are (precision, recall, F1). Note that the results for the Specific Time Split are omitted from this table as Specific Time Split only has one split and, thus, the results are identical to that in the table showing the weighted averages.}
{\fontsize{4}{4}\selectfont
\arrayrulecolor{black}
\begin{tabular}{!{\color{black}\vrule}l!{\color{black}\vrule}l!{\color{black}\vrule}r!{\color{black}\vrule}l!{\color{black}\vrule}l!{\color{black}\vrule}l!{\color{black}\vrule}} 
\arrayrulecolor{black}\cline{1-1}\arrayrulecolor{black}\cline{2-6}
Train and Split Test Type          & Feed Omitted  & \multicolumn{1}{l!{\color{black}\vrule}}{Evaluation Id} & NB                 & DTree              & Ada                 \\ 
\arrayrulecolor{black}\cline{1-1}\arrayrulecolor{black}\cline{2-6}
\multirow{41}{*}{Window Equal}     & \CIRCL          & 1                                                       & (1.0, 1.0, 1.0)    & (1.0, 0.67, 0.8)   & (1.0, 0.33, 0.5)    \\ 
\cline{2-6}
                                   & \CthulhuSPRL  & 1                                                       & (1.0, 1.0, 1.0)    & (1.0, 1.0, 1.0)    & (1.0, 1.0, 1.0)     \\ 
\cline{2-6}
                                   & \CIRCL          & 2                                                       & Ignore             & (1.0, 0.65, 0.79)  & (0.83, 0.25, 0.38)  \\ 
\cline{2-6}
                                   & \CthulhuSPRL  & 2                                                       & (1.0, 1.0, 1.0)    & (1.0, 0.33, 0.5)   & (1.0, 0.42, 0.59)   \\ 
\cline{2-6}
                                   & \CIRCL          & 3                                                       & (0.89, 1.0, 0.94)  & (0.9, 0.84, 0.87)  & (0.9, 0.84, 0.87)   \\ 
\cline{2-6}
                                   & \CthulhuSPRL  & 3                                                       & (1.0, 1.0, 1.0)    & (1.0, 0.76, 0.86)  & (1.0, 0.76, 0.86)   \\ 
\cline{2-6}
                                   & \CIRCL          & 4                                                       & (0.74, 1.0, 0.85)  & (0.68, 0.52, 0.59) & (0.75, 0.74, 0.74)  \\ 
\cline{2-6}
                                   & \CthulhuSPRL  & 4                                                       & (1.0, 1.0, 1.0)    & (1.0, 0.68, 0.81)  & (1.0, 0.82, 0.9)    \\ 
\cline{2-6}
                                   & \INCIBE         & 4                                                       & (0.94, 0.94, 0.94) & (1.0, 0.65, 0.79)  & (1.0, 0.59, 0.74)   \\ 
\cline{2-6}
                                   & \CIRCL          & 5                                                       & (0.87, 0.92, 0.89) & (0.83, 0.83, 0.83) & (0.82, 0.83, 0.83)  \\ 
\cline{2-6}
                                   & \CthulhuSPRL  & 5                                                       & (0.0, 0.0, 0.0)    & (1.0, 1.0, 1.0)    & (0.67, 1.0, 0.8)    \\ 
\cline{2-6}
                                   & \INCIBE         & 5                                                       & (1.0, 0.44, 0.62)  & (1.0, 0.67, 0.8)   & (1.0, 1.0, 1.0)     \\ 
\cline{2-6}
                                   & \CERTBund      & 6                                                       & (0.5, 0.89, 0.64)  & (0.44, 0.44, 0.44) & (0.5, 0.56, 0.53)   \\ 
\cline{2-6}
                                   & \CIRCL          & 6                                                       & (0.5, 1.0, 0.66)   & (0.49, 0.45, 0.47) & (0.64, 0.56, 0.59)  \\ 
\cline{2-6}
                                   & \Crimeware      & 6                                                       & (0.03, 1.0, 0.06)  & (0.29, 0.67, 0.4)  & (0.14, 0.33, 0.2)   \\ 
\cline{2-6}
                                   & \CthulhuSPRL  & 6                                                       & (0.23, 1.0, 0.38)  & (0.24, 0.71, 0.36) & (0.24, 0.86, 0.38)  \\ 
\cline{2-6}
                                   & \DCSO           & 6                                                       & (0.3, 1.0, 0.46)   & (0.2, 0.33, 0.25)  & (0.22, 0.67, 0.33)  \\ 
\cline{2-6}
                                   & \INCIBE         & 6                                                       & (0.89, 0.89, 0.89) & (0.86, 0.67, 0.75) & (0.88, 0.78, 0.82)  \\ 
\cline{2-6}
                                   & \inThreat   & 6                                                       & (0.56, 1.0, 0.72)  & (0.43, 0.33, 0.38) & (0.57, 0.44, 0.5)   \\ 
\cline{2-6}
                                   & \CERTBund      & 7                                                       & (0.29, 0.13, 0.18) & (0.2, 0.2, 0.2)    & (0.18, 0.13, 0.15)  \\ 
\cline{2-6}
                                   & \CIRCL          & 7                                                       & (0.68, 0.91, 0.78) & (0.62, 0.6, 0.61)  & (0.72, 0.66, 0.69)  \\ 
\cline{2-6}
                                   & \Crimeware      & 7                                                       & Ignore             & Ignore             & (1.0, 1.0, 1.0)     \\ 
\cline{2-6}
                                   & \CthulhuSPRL  & 7                                                       & (0.8, 0.5, 0.62)   & (0.88, 0.88, 0.88) & (0.86, 0.75, 0.8)   \\ 
\cline{2-6}
                                   & \DCSO           & 7                                                       & (0.85, 0.79, 0.82) & (0.85, 0.65, 0.74) & (0.83, 0.79, 0.81)  \\ 
\cline{2-6}
                                   & \INCIBE         & 7                                                       & (0.78, 0.58, 0.67) & (0.5, 0.17, 0.25)  & (0.5, 0.25, 0.33)   \\ 
\cline{2-6}
                                   & \inThreat   & 7                                                       & (1.0, 0.12, 0.21)  & (0.77, 0.59, 0.67) & (1.0, 0.29, 0.45)   \\ 
\cline{2-6}
                                   & \CERTBund      & 8                                                       & (0.25, 0.06, 0.09) & (0.62, 0.72, 0.67) & (0.59, 0.72, 0.65)  \\ 
\cline{2-6}
                                   & \CIRCL          & 8                                                       & (0.72, 0.83, 0.77) & (0.63, 0.83, 0.72) & (0.66, 0.94, 0.77)  \\ 
\cline{2-6}
                                   & \Crimeware      & 8                                                       & (1.0, 1.0, 1.0)    & (1.0, 1.0, 1.0)    & (1.0, 1.0, 1.0)     \\ 
\cline{2-6}
                                   & \CthulhuSPRL  & 8                                                       & (1.0, 0.33, 0.5)   & (1.0, 0.67, 0.8)   & (1.0, 0.67, 0.8)    \\ 
\cline{2-6}
                                   & \DCSO           & 8                                                       & (0.68, 0.89, 0.77) & (0.64, 0.78, 0.7)  & (0.67, 0.92, 0.78)  \\ 
\cline{2-6}
                                   & \inThreat   & 8                                                       & (1.0, 0.04, 0.08)  & (1.0, 0.5, 0.67)   & (1.0, 0.46, 0.63)   \\ 
\cline{2-6}
                                   & \CERTBund      & 9                                                       & (0.5, 0.1, 0.16)   & (0.75, 0.36, 0.48) & (0.53, 0.74, 0.61)  \\ 
\cline{2-6}
                                   & \CIRCL          & 9                                                       & (0.83, 0.73, 0.78) & (0.74, 0.76, 0.75) & (0.79, 0.9, 0.84)   \\ 
\cline{2-6}
                                   & \DCSO           & 9                                                       & (0.97, 0.85, 0.9)  & (0.95, 0.94, 0.95) & (0.93, 0.83, 0.88)  \\ 
\cline{2-6}
                                   & \INCIBE         & 9                                                       & Ignore             & Ignore             & (1.0, 1.0, 1.0)     \\ 
\cline{2-6}
                                   & \inThreat   & 9                                                       & (1.0, 0.57, 0.73)  & (1.0, 0.24, 0.38)  & (1.0, 0.1, 0.17)    \\ 
\cline{2-6}
                                   & \CERTBund      & 10                                                      & (0.06, 0.96, 0.11) & (0.04, 0.38, 0.07) & (0.07, 0.75, 0.12)  \\ 
\cline{2-6}
                                   & \CIRCL          & 10                                                      & (0.8, 0.64, 0.71)  & (0.84, 0.47, 0.6)  & (0.84, 0.67, 0.75)  \\ 
\cline{2-6}
                                   & \DCSO           & 10                                                      & (1.0, 0.71, 0.83)  & (1.0, 0.79, 0.89)  & (1.0, 0.59, 0.74)   \\ 
\cline{2-6}
                                   & \inThreat   & 10                                                      & (0.94, 0.67, 0.78) & (0.87, 0.29, 0.43) & (0.9, 0.42, 0.58)   \\ 
\hline
\multirow{41}{*}{Window Aggregate} & \CIRCL          & 1                                                       & (1.0, 1.0, 1.0)    & (1.0, 0.67, 0.8)   & (1.0, 0.67, 0.8)    \\ 
\cline{2-6}
                                   & \CthulhuSPRL  & 1                                                       & (1.0, 1.0, 1.0)    & (1.0, 1.0, 1.0)    & (1.0, 1.0, 1.0)     \\ 
\cline{2-6}
                                   & \CIRCL          & 2                                                       & (0.95, 1.0, 0.98)  & (1.0, 0.7, 0.82)   & (0.93, 0.65, 0.76)  \\ 
\cline{2-6}
                                   & \CthulhuSPRL  & 2                                                       & (1.0, 1.0, 1.0)    & (1.0, 1.0, 1.0)    & (1.0, 0.92, 0.96)   \\ 
\cline{2-6}
                                   & \CIRCL          & 3                                                       & (0.89, 1.0, 0.94)  & (0.89, 0.81, 0.85) & (0.89, 0.81, 0.85)  \\ 
\cline{2-6}
                                   & \CthulhuSPRL  & 3                                                       & (1.0, 1.0, 1.0)    & (1.0, 0.93, 0.96)  & (1.0, 0.93, 0.96)   \\ 
\cline{2-6}
                                   & \CIRCL          & 4                                                       & (0.74, 1.0, 0.85)  & (0.86, 0.66, 0.75) & (0.79, 0.65, 0.71)  \\ 
\cline{2-6}
                                   & \CthulhuSPRL  & 4                                                       & (1.0, 1.0, 1.0)    & (1.0, 0.95, 0.98)  & (1.0, 1.0, 1.0)     \\ 
\cline{2-6}
                                   & \INCIBE         & 4                                                       & (0.94, 1.0, 0.97)  & (0.93, 0.82, 0.87) & (0.94, 0.88, 0.91)  \\ 
\cline{2-6}
                                   & \CIRCL          & 5                                                       & (0.83, 0.97, 0.9)  & (0.85, 0.6, 0.7)   & (0.83, 0.97, 0.9)   \\ 
\cline{2-6}
                                   & \CthulhuSPRL  & 5                                                       & (0.5, 0.5, 0.5)    & (0.5, 0.5, 0.5)    & (0.67, 1.0, 0.8)    \\ 
\cline{2-6}
                                   & \INCIBE         & 5                                                       & (1.0, 0.89, 0.94)  & (1.0, 0.78, 0.88)  & (1.0, 1.0, 1.0)     \\ 
\cline{2-6}
                                   & \CERTBund      & 6                                                       & (0.57, 0.44, 0.5)  & (0.42, 0.56, 0.48) & (0.5, 0.78, 0.61)   \\ 
\cline{2-6}
                                   & \CIRCL          & 6                                                       & (0.61, 0.93, 0.74) & (0.66, 0.74, 0.7)  & (0.69, 0.94, 0.8)   \\ 
\cline{2-6}
                                   & \Crimeware      & 6                                                       & (0.02, 0.67, 0.04) & (0.02, 0.33, 0.03) & (0.04, 0.33, 0.07)  \\ 
\cline{2-6}
                                   & \CthulhuSPRL  & 6                                                       & (0.2, 0.71, 0.31)  & (0.2, 0.71, 0.31)  & (0.23, 1.0, 0.38)   \\ 
\cline{2-6}
                                   & \DCSO           & 6                                                       & (0.22, 0.67, 0.33) & (0.11, 0.33, 0.17) & (0.22, 0.67, 0.33)  \\ 
\cline{2-6}
                                   & \INCIBE         & 6                                                       & (0.86, 0.67, 0.75) & (0.88, 0.78, 0.82) & (0.89, 0.89, 0.89)  \\ 
\cline{2-6}
                                   & \inThreat   & 6                                                       & (0.54, 0.78, 0.64) & (0.6, 0.67, 0.63)  & (0.5, 0.67, 0.57)   \\ 
\cline{2-6}
                                   & \CERTBund      & 7                                                       & (0.4, 0.27, 0.32)  & (0.43, 0.2, 0.27)  & (0.4, 0.53, 0.46)   \\ 
\cline{2-6}
                                   & \CIRCL          & 7                                                       & (0.52, 0.94, 0.67) & (0.6, 0.61, 0.61)  & (0.7, 0.9, 0.79)    \\ 
\cline{2-6}
                                   & \Crimeware      & 7                                                       & Ignore             & Ignore             & (0.33, 1.0, 0.5)    \\ 
\cline{2-6}
                                   & \CthulhuSPRL  & 7                                                       & (0.88, 0.88, 0.88) & (0.83, 0.62, 0.71) & (0.88, 0.88, 0.88)  \\ 
\cline{2-6}
                                   & \DCSO           & 7                                                       & (0.85, 0.95, 0.9)  & (0.88, 0.86, 0.87) & (0.86, 0.98, 0.91)  \\ 
\cline{2-6}
                                   & \INCIBE         & 7                                                       & (0.82, 0.75, 0.78) & (0.75, 0.5, 0.6)   & (0.67, 0.33, 0.44)  \\ 
\cline{2-6}
                                   & \inThreat   & 7                                                       & (0.93, 0.76, 0.84) & (0.81, 0.76, 0.79) & (0.81, 0.76, 0.79)  \\ 
\cline{2-6}
                                   & \CERTBund      & 8                                                       & (0.33, 0.17, 0.22) & (0.57, 0.72, 0.63) & (0.53, 0.56, 0.54)  \\ 
\cline{2-6}
                                   & \CIRCL          & 8                                                       & (0.68, 0.89, 0.77) & (0.7, 0.7, 0.7)    & (0.67, 0.95, 0.79)  \\ 
\cline{2-6}
                                   & \Crimeware      & 8                                                       & (1.0, 1.0, 1.0)    & (1.0, 1.0, 1.0)    & (1.0, 1.0, 1.0)     \\ 
\cline{2-6}
                                   & \CthulhuSPRL  & 8                                                       & (1.0, 0.33, 0.5)   & (1.0, 0.67, 0.8)   & (1.0, 1.0, 1.0)     \\ 
\cline{2-6}
                                   & \DCSO           & 8                                                       & (0.61, 0.97, 0.75) & (0.57, 0.72, 0.63) & (0.58, 0.83, 0.68)  \\ 
\cline{2-6}
                                   & \inThreat   & 8                                                       & (1.0, 0.29, 0.45)  & (1.0, 0.5, 0.67)   & (1.0, 0.42, 0.59)   \\ 
\cline{2-6}
                                   & \CERTBund      & 9                                                       & (0.67, 0.33, 0.44) & (0.76, 0.81, 0.78) & (0.55, 0.67, 0.6)   \\ 
\cline{2-6}
                                   & \CIRCL          & 9                                                       & (0.82, 0.78, 0.8)  & (0.71, 0.78, 0.74) & (0.73, 0.8, 0.77)   \\ 
\cline{2-6}
                                   & \DCSO           & 9                                                       & (0.97, 0.86, 0.91) & (0.97, 0.94, 0.95) & (0.95, 0.89, 0.92)  \\ 
\cline{2-6}
                                   & \INCIBE         & 9                                                       & Ignore             & Ignore             & Ignore              \\ 
\cline{2-6}
                                   & \inThreat   & 9                                                       & (1.0, 0.81, 0.89)  & (1.0, 0.57, 0.73)  & (1.0, 0.29, 0.44)   \\ 
\cline{2-6}
                                   & \CERTBund      & 10                                                      & (0.07, 0.42, 0.12) & (0.27, 0.92, 0.42) & (0.14, 0.67, 0.24)  \\ 
\cline{2-6}
                                   & \CIRCL          & 10                                                      & (0.89, 0.6, 0.72)  & (0.92, 0.82, 0.87) & (0.85, 0.71, 0.77)  \\ 
\cline{2-6}
                                   & \DCSO           & 10                                                      & (1.0, 0.88, 0.94)  & (1.0, 0.97, 0.99)  & (1.0, 0.79, 0.89)   \\ 
\cline{2-6}
                                   & \inThreat   & 10                                                      & (1.0, 0.4, 0.57)   & (0.85, 0.24, 0.38) & (0.88, 0.33, 0.48)  \\
\hline
\end{tabular}
}
\arrayrulecolor{black}
\end{table}

% \usepackage{multirow}
% \usepackage{colortbl}

\begin{table}[H]
\centering
\caption{BERT Temporal and Spatial Results. This uses a tree depth of 4 for Decision Tree and AdaBoost. The results are (precision, recall, F1). Note that the results for the Specific Time Split are omitted from this table as Specific Time Split only has one split and, thus, the results are identical to that in the table showing the weighted averages.}
{\fontsize{4}{4}\selectfont
\arrayrulecolor{black}
\begin{tabular}{!{\color{black}\vrule}l!{\color{black}\vrule}l!{\color{black}\vrule}r!{\color{black}\vrule}l!{\color{black}\vrule}l!{\color{black}\vrule}l!{\color{black}\vrule}} 
\arrayrulecolor{black}\cline{1-1}\arrayrulecolor{black}\cline{2-6}
Train and Split Test Type          & Feed Omitted  & \multicolumn{1}{l!{\color{black}\vrule}}{Evaluation Id} & NB                 & DTree              & Ada                 \\ 
\arrayrulecolor{black}\cline{1-1}\arrayrulecolor{black}\cline{2-6}
\multirow{41}{*}{Window Equal}     & \CIRCL          & 1                                                       & (1.0, 1.0, 1.0)    & (1.0, 1.0, 1.0)    & (1.0, 1.0, 1.0)     \\ 
\cline{2-6}
                                   & \CthulhuSPRL  & 1                                                       & (1.0, 1.0, 1.0)    & (1.0, 1.0, 1.0)    & (1.0, 1.0, 1.0)     \\ 
\cline{2-6}
                                   & \CIRCL          & 2                                                       & Ignore             & Ignore             & (1.0, 0.5, 0.67)    \\ 
\cline{2-6}
                                   & \CthulhuSPRL  & 2                                                       & (1.0, 0.25, 0.4)   & (1.0, 0.67, 0.8)   & (1.0, 0.58, 0.74)   \\ 
\cline{2-6}
                                   & \CIRCL          & 3                                                       & (0.89, 1.0, 0.94)  & (0.87, 0.87, 0.87) & (0.89, 0.77, 0.83)  \\ 
\cline{2-6}
                                   & \CthulhuSPRL  & 3                                                       & (1.0, 1.0, 1.0)    & (1.0, 0.83, 0.91)  & (1.0, 0.72, 0.84)   \\ 
\cline{2-6}
                                   & \CIRCL          & 4                                                       & (0.74, 0.99, 0.85) & (0.72, 0.61, 0.66) & (0.7, 0.66, 0.68)   \\ 
\cline{2-6}
                                   & \CthulhuSPRL  & 4                                                       & (1.0, 0.91, 0.95)  & (1.0, 0.68, 0.81)  & (1.0, 0.64, 0.78)   \\ 
\cline{2-6}
                                   & \INCIBE         & 4                                                       & (0.92, 0.65, 0.76) & (0.92, 0.65, 0.76) & (0.9, 0.53, 0.67)   \\ 
\cline{2-6}
                                   & \CIRCL          & 5                                                       & (0.79, 1.0, 0.88)  & (0.77, 0.61, 0.68) & (0.81, 0.95, 0.87)  \\ 
\cline{2-6}
                                   & \CthulhuSPRL  & 5                                                       & (0.5, 0.5, 0.5)    & (0.5, 0.5, 0.5)    & (0.5, 0.5, 0.5)     \\ 
\cline{2-6}
                                   & \INCIBE         & 5                                                       & (1.0, 0.89, 0.94)  & (1.0, 0.44, 0.62)  & (1.0, 1.0, 1.0)     \\ 
\cline{2-6}
                                   & \CERTBund      & 6                                                       & (0.45, 1.0, 0.62)  & (0.5, 0.33, 0.4)   & (0.75, 0.33, 0.46)  \\ 
\cline{2-6}
                                   & \CIRCL          & 6                                                       & (0.5, 0.99, 0.66)  & (0.51, 0.53, 0.52) & (0.5, 0.43, 0.46)   \\ 
\cline{2-6}
                                   & \Crimeware      & 6                                                       & (0.02, 1.0, 0.04)  & (0.05, 0.67, 0.09) & (0.03, 1.0, 0.06)   \\ 
\cline{2-6}
                                   & \CthulhuSPRL  & 6                                                       & (0.23, 1.0, 0.38)  & (0.24, 0.57, 0.33) & (0.2, 0.43, 0.27)   \\ 
\cline{2-6}
                                   & \DCSO           & 6                                                       & (0.27, 1.0, 0.43)  & (0.33, 0.33, 0.33) & (0.17, 0.33, 0.22)  \\ 
\cline{2-6}
                                   & \INCIBE         & 6                                                       & (0.82, 1.0, 0.9)   & (1.0, 0.11, 0.2)   & (0.0, 0.0, 0.0)     \\ 
\cline{2-6}
                                   & \inThreat   & 6                                                       & (0.5, 1.0, 0.67)   & (0.64, 0.78, 0.7)  & (0.5, 0.78, 0.61)   \\ 
\cline{2-6}
                                   & \CERTBund      & 7                                                       & (0.42, 0.33, 0.37) & (0.2, 0.4, 0.27)   & (0.38, 0.33, 0.36)  \\ 
\cline{2-6}
                                   & \CIRCL          & 7                                                       & (0.61, 0.87, 0.72) & (0.6, 0.64, 0.62)  & (0.76, 0.69, 0.72)  \\ 
\cline{2-6}
                                   & \Crimeware      & 7                                                       & (0.0, 0.0, 0.0)    & (1.0, 1.0, 1.0)    & (1.0, 1.0, 1.0)     \\ 
\cline{2-6}
                                   & \CthulhuSPRL  & 7                                                       & (1.0, 0.25, 0.4)   & (1.0, 0.12, 0.22)  & (1.0, 0.25, 0.4)    \\ 
\cline{2-6}
                                   & \DCSO           & 7                                                       & (0.84, 0.84, 0.84) & (1.0, 0.12, 0.21)  & (0.78, 0.42, 0.55)  \\ 
\cline{2-6}
                                   & \INCIBE         & 7                                                       & (0.86, 0.5, 0.63)  & (0.57, 0.33, 0.42) & (0.6, 0.25, 0.35)   \\ 
\cline{2-6}
                                   & \inThreat   & 7                                                       & (0.81, 0.76, 0.79) & (1.0, 0.29, 0.45)  & (0.92, 0.65, 0.76)  \\ 
\cline{2-6}
                                   & \CERTBund      & 8                                                       & (0.57, 0.44, 0.5)  & (0.17, 0.33, 0.23) & (0.46, 0.33, 0.39)  \\ 
\cline{2-6}
                                   & \CIRCL          & 8                                                       & (0.66, 0.77, 0.71) & (0.59, 0.61, 0.6)  & (0.71, 0.7, 0.71)   \\ 
\cline{2-6}
                                   & \Crimeware      & 8                                                       & (1.0, 1.0, 1.0)    & Ignore             & (1.0, 1.0, 1.0)     \\ 
\cline{2-6}
                                   & \CthulhuSPRL  & 8                                                       & (1.0, 0.33, 0.5)   & Ignore             & (1.0, 0.67, 0.8)    \\ 
\cline{2-6}
                                   & \DCSO           & 8                                                       & (0.69, 0.86, 0.77) & (0.74, 0.72, 0.73) & (0.73, 0.89, 0.8)   \\ 
\cline{2-6}
                                   & \inThreat   & 8                                                       & (1.0, 0.46, 0.63)  & (1.0, 0.5, 0.67)   & (1.0, 0.54, 0.7)    \\ 
\cline{2-6}
                                   & \CERTBund      & 9                                                       & (0.49, 0.67, 0.57) & (0.56, 0.71, 0.63) & (0.73, 0.64, 0.68)  \\ 
\cline{2-6}
                                   & \CIRCL          & 9                                                       & (0.72, 0.93, 0.81) & (0.77, 0.88, 0.82) & (0.78, 0.93, 0.84)  \\ 
\cline{2-6}
                                   & \DCSO           & 9                                                       & (0.96, 0.97, 0.96) & (0.95, 0.79, 0.86) & (0.94, 0.97, 0.96)  \\ 
\cline{2-6}
                                   & \INCIBE         & 9                                                       & (1.0, 1.0, 1.0)    & Ignore             & Ignore              \\ 
\cline{2-6}
                                   & \inThreat   & 9                                                       & (1.0, 0.43, 0.6)   & (1.0, 0.52, 0.69)  & (1.0, 0.29, 0.44)   \\ 
\cline{2-6}
                                   & \CERTBund      & 10                                                      & (0.09, 0.67, 0.15) & (0.06, 0.71, 0.11) & (0.07, 0.5, 0.13)   \\ 
\cline{2-6}
                                   & \CIRCL          & 10                                                      & (0.84, 0.67, 0.75) & (0.82, 0.67, 0.74) & (0.85, 0.62, 0.72)  \\ 
\cline{2-6}
                                   & \DCSO           & 10                                                      & (1.0, 0.76, 0.87)  & (1.0, 0.59, 0.74)  & (1.0, 0.74, 0.85)   \\ 
\cline{2-6}
                                   & \inThreat   & 10                                                      & (0.92, 0.27, 0.41) & (0.93, 0.62, 0.75) & (0.94, 0.69, 0.79)  \\ 
\hline
\multirow{41}{*}{Window Aggregate} & \CIRCL          & 1                                                       & (1.0, 1.0, 1.0)    & (1.0, 1.0, 1.0)    & (1.0, 1.0, 1.0)     \\ 
\cline{2-6}
                                   & \CthulhuSPRL  & 1                                                       & (1.0, 1.0, 1.0)    & (1.0, 1.0, 1.0)    & (1.0, 1.0, 1.0)     \\ 
\cline{2-6}
                                   & \CIRCL          & 2                                                       & (0.95, 1.0, 0.98)  & (0.93, 0.65, 0.76) & (0.93, 0.65, 0.76)  \\ 
\cline{2-6}
                                   & \CthulhuSPRL  & 2                                                       & (1.0, 1.0, 1.0)    & (1.0, 1.0, 1.0)    & (1.0, 0.92, 0.96)   \\ 
\cline{2-6}
                                   & \CIRCL          & 3                                                       & (0.88, 0.97, 0.92) & (0.9, 0.87, 0.89)  & (0.94, 0.94, 0.94)  \\ 
\cline{2-6}
                                   & \CthulhuSPRL  & 3                                                       & (1.0, 1.0, 1.0)    & (1.0, 0.93, 0.96)  & (1.0, 0.97, 0.98)   \\ 
\cline{2-6}
                                   & \CIRCL          & 4                                                       & (0.74, 0.99, 0.85) & (0.71, 0.84, 0.77) & (0.76, 0.91, 0.83)  \\ 
\cline{2-6}
                                   & \CthulhuSPRL  & 4                                                       & (1.0, 0.95, 0.98)  & (1.0, 0.77, 0.87)  & (1.0, 0.95, 0.98)   \\ 
\cline{2-6}
                                   & \INCIBE         & 4                                                       & (0.94, 0.88, 0.91) & (0.91, 0.59, 0.71) & (0.93, 0.76, 0.84)  \\ 
\cline{2-6}
                                   & \CIRCL          & 5                                                       & (0.78, 0.99, 0.87) & (0.81, 0.6, 0.69)  & (0.81, 0.97, 0.88)  \\ 
\cline{2-6}
                                   & \CthulhuSPRL  & 5                                                       & (0.5, 0.5, 0.5)    & (0.5, 0.5, 0.5)    & (0.67, 1.0, 0.8)    \\ 
\cline{2-6}
                                   & \INCIBE         & 5                                                       & (1.0, 1.0, 1.0)    & (1.0, 0.33, 0.5)   & (1.0, 1.0, 1.0)     \\ 
\cline{2-6}
                                   & \CERTBund      & 6                                                       & (0.47, 0.89, 0.62) & (0.42, 0.56, 0.48) & (0.46, 0.67, 0.55)  \\ 
\cline{2-6}
                                   & \CIRCL          & 6                                                       & (0.5, 0.94, 0.66)  & (0.5, 0.53, 0.51)  & (0.53, 0.9, 0.67)   \\ 
\cline{2-6}
                                   & \Crimeware      & 6                                                       & (0.02, 1.0, 0.05)  & (0.01, 0.33, 0.02) & (0.02, 0.67, 0.03)  \\ 
\cline{2-6}
                                   & \CthulhuSPRL  & 6                                                       & (0.24, 0.86, 0.38) & (0.2, 0.43, 0.27)  & (0.17, 0.57, 0.26)  \\ 
\cline{2-6}
                                   & \DCSO           & 6                                                       & (0.3, 1.0, 0.46)   & (0.17, 0.33, 0.22) & (0.33, 1.0, 0.5)    \\ 
\cline{2-6}
                                   & \INCIBE         & 6                                                       & (0.78, 0.78, 0.78) & (0.8, 0.44, 0.57)  & (0.78, 0.78, 0.78)  \\ 
\cline{2-6}
                                   & \inThreat   & 6                                                       & (0.47, 0.78, 0.58) & (0.25, 0.22, 0.24) & (0.53, 0.89, 0.67)  \\ 
\cline{2-6}
                                   & \CERTBund      & 7                                                       & (0.21, 0.8, 0.33)  & (0.47, 0.53, 0.5)  & (0.44, 0.53, 0.48)  \\ 
\cline{2-6}
                                   & \CIRCL          & 7                                                       & (0.54, 0.94, 0.69) & (0.63, 0.74, 0.68) & (0.72, 0.88, 0.79)  \\ 
\cline{2-6}
                                   & \Crimeware      & 7                                                       & (0.0, 0.0, 0.0)    & (0.0, 0.0, 0.0)    & (1.0, 1.0, 1.0)     \\ 
\cline{2-6}
                                   & \CthulhuSPRL  & 7                                                       & (0.86, 0.75, 0.8)  & (0.67, 0.25, 0.36) & (0.86, 0.75, 0.8)   \\ 
\cline{2-6}
                                   & \DCSO           & 7                                                       & (0.82, 0.93, 0.87) & (0.82, 0.53, 0.65) & (0.83, 0.79, 0.81)  \\ 
\cline{2-6}
                                   & \INCIBE         & 7                                                       & (0.69, 0.75, 0.72) & (0.75, 0.5, 0.6)   & (0.67, 0.5, 0.57)   \\ 
\cline{2-6}
                                   & \inThreat   & 7                                                       & (0.84, 0.94, 0.89) & (0.82, 0.53, 0.64) & (0.92, 0.71, 0.8)   \\ 
\cline{2-6}
                                   & \CERTBund      & 8                                                       & (0.23, 0.5, 0.32)  & (0.21, 0.28, 0.24) & (0.58, 0.61, 0.59)  \\ 
\cline{2-6}
                                   & \CIRCL          & 8                                                       & (0.6, 0.92, 0.72)  & (0.57, 0.7, 0.63)  & (0.7, 0.88, 0.78)   \\ 
\cline{2-6}
                                   & \Crimeware      & 8                                                       & (1.0, 1.0, 1.0)    & (1.0, 1.0, 1.0)    & (1.0, 1.0, 1.0)     \\ 
\cline{2-6}
                                   & \CthulhuSPRL  & 8                                                       & (1.0, 0.67, 0.8)   & (1.0, 0.33, 0.5)   & (1.0, 0.67, 0.8)    \\ 
\cline{2-6}
                                   & \DCSO           & 8                                                       & (0.54, 0.86, 0.67) & (0.64, 0.58, 0.61) & (0.7, 0.97, 0.81)   \\ 
\cline{2-6}
                                   & \inThreat   & 8                                                       & (1.0, 0.88, 0.93)  & (1.0, 0.33, 0.5)   & (1.0, 0.83, 0.91)   \\ 
\cline{2-6}
                                   & \CERTBund      & 9                                                       & (0.45, 0.69, 0.54) & (0.44, 0.55, 0.49) & (0.51, 0.69, 0.59)  \\ 
\cline{2-6}
                                   & \CIRCL          & 9                                                       & (0.75, 0.95, 0.84) & (0.76, 0.85, 0.8)  & (0.78, 0.85, 0.81)  \\ 
\cline{2-6}
                                   & \DCSO           & 9                                                       & (0.94, 0.89, 0.91) & (0.95, 0.83, 0.89) & (0.94, 0.97, 0.96)  \\ 
\cline{2-6}
                                   & \INCIBE         & 9                                                       & (1.0, 1.0, 1.0)    & (1.0, 1.0, 1.0)    & Ignore              \\ 
\cline{2-6}
                                   & \inThreat   & 9                                                       & (1.0, 0.76, 0.86)  & (1.0, 0.24, 0.38)  & (1.0, 0.43, 0.6)    \\ 
\cline{2-6}
                                   & \CERTBund      & 10                                                      & (0.09, 0.62, 0.15) & (0.11, 0.75, 0.2)  & (0.13, 0.67, 0.22)  \\ 
\cline{2-6}
                                   & \CIRCL          & 10                                                      & (0.84, 0.85, 0.85) & (0.85, 0.84, 0.84) & (0.87, 0.71, 0.78)  \\ 
\cline{2-6}
                                   & \DCSO           & 10                                                      & (1.0, 0.79, 0.89)  & (1.0, 0.82, 0.9)   & (1.0, 0.85, 0.92)   \\ 
\cline{2-6}
                                   & \inThreat   & 10                                                      & (1.0, 0.4, 0.57)   & (1.0, 0.36, 0.52)  & (1.0, 0.64, 0.78)   \\
\hline
\end{tabular}
}
\arrayrulecolor{black}
\end{table}

==> docs/introduction.tex <==


\section{Introduction}\label{sec:introduction} 


Thtreat 
 Intelligence (TI) has become a cornerstone of collaborative data-driven security \cite{grandview}.
%
Many organizations rely on TI feeds to assess the risk associated with security vulnerabilities and deploy countermeasures in a timely manner. 
%
The interest in TI feeds has grown over the last few years, with an increasing amount and variety of TI feeds \cite{chismon2015threat}.
%
TI feeds are now available in many different flavors---from free to commercial, from many different providers ranging from third-party firms or public groups, and targeting various kinds of threats from phishing to botnets.


%%
A key challenge in effectively leveraging TI feeds is coping with the volume of data. 
%
Large amounts of new threat information is regularly published, sometimes in excess of millions per day.
%
As the volume of threat information has increased, it has become infeasible to manually sift through them \cite{suciu2021expected}.
%
Thus, automated methods to systematically sift through TI feeds are needed. 
%
Another key challenge is that TI feeds are loosely structured due to heterogeneous data sources, software ecosystems, internal processes, maturity of the TI program, and staff expertise.
%
There has been progress over the last decade to standardize information sharing in TI feeds \cite{misp}.\footnote{The Malware Information Sharing Platform (MISP) \cite{misp} and the Structured Threat Information (STIX)   are two important initiatives in this direction. Both MISP and STIX establish formats that allow different organizations to share data in a uniform manner.}
%
While such standardization mitigates this challenge, a significant fraction of the information in TI feeds is made available within free-form text fields that are manually filled by security experts with differing styles.
%
These challenges make it non-trivial to automatically process the information in TI feeds to extract actionable information.


%%
In this paper, we consider the problem of detecting whether information about the exploitation of vulnerabilities in the wild is present in a given TI feed event. 
%
Detection of vulnerability exploitation in the wild is crucial for risk assessment and incident response purposes. 
%
Consider, for instance, the Common Vulnerability Scoring System (CVSS) \cite{cvss}, one of the current de facto solutions to parametrize vulnerability risk. 
%
While CVSS does provide a subscore to track existence of exploits for vulnerabilities, it does not provide a subscore to track exploitation incidents \emph{in the wild}.  
%
The recently proposed Exploit Prediction Scoring System (EPSS) \cite{jacobs2021exploit} aims to bridge this gap by forecasting whether a vulnerability will be exploited following its public disclosure.
%
Thus, information about vulnerability exploitation in the wild can complement CVSS and EPSS based risk assessment strategies. 
%
To the best of our knowledge, there are currently no large-scale measurements leveraging TI feeds to assess exploitation in the wild, or tools to leverage those measurements   for risk assessment purposes.  


%The documentation of this information is done in different ways, through labels, comments and textual descriptions, sometimes because the TI feed format does not have a unique predefined way to do it (e.g., at MISP \cite{misp}) and sometimes because authors simply do not use the available formats (e.g., at STIX \cite{STIX}). 
%The final result is that this information is sometimes present across feeds in unstructured textual form and therefore calls for machine learning tools for automated parsing and detection. 


The Known Exploited Vulnerabilities (KEV) catalog, maintained by CISA~\cite{CISAKEV},  is another important source for information on vulnerabilities that have been actively exploited in the wild, yet it faces significant limitations. Its static nature means it cannot adapt to the changing threat landscape, and its focus is  tailored to vulnerabilities that government agencies must address within certain deadlines, potentially missing broader threats.  
  Google Project Zero catalog also contains a list of vulnerabilities   exploited    in the wild, but faces similar limitations, e.g.,  the list currently contains only 310 vulnerabilities~\cite{GoogleProjectZero}. Meanwhile, EPSS provides a dynamic prediction of exploit likelihood but lacks insight into the reasons behind its scores,  and is limited by its reliance on private data, which may not reflect wider environmental and organizational contexts~\cite{massacci2024holy}. 






%%
To address the aforementioned challenges, we propose a machine learning approach to automatically ingest TI feeds for detecting vulnerability exploitation in the wild and that can be tailored to specific organizational needs.
%
Our machine learning pipeline leverages natural language processing (NLP) based embedding techniques to parse and encode loosely structured information in TI feeds. 
%
To this end, we consider both static and dynamic embeddings techniques. 
%
Static embeddings generate the same embedding for the same vocabulary in different TI feed events: vector matrices which encode vocabulary into vectors are shared across events.  
%
Dynamic embeddings,  in contrast, aim at capturing vocabulary semantics in different contexts to address the issue of  context-dependent nature of information in TI feed events.
%
Specifically, we train a static embedding (Doc2Vec \cite{le2014distributed}) and dynamic embedding (BERT \cite{devlin2019bert}) in an unsupervised manner to capture the semantics of loosely structured information in different TI feeds. 
%
Moreover, we also train purpose-built embeddings that are further trained (or fine-tuned) on data from TI feeds. 
%
TI2Vec and TIBERT represent specialized embeddings corresponding to Doc2Vec and BERT, respectively. 
%(corresponding to BERT) 
%
%specialize vanilla pre-trained embeddings using TI feed
%\hl{and refer to the fine-tuned embeddings produced using our TI feeds as TI2Vec and TIBERT, respectively. }
%
We then leverage these embeddings along with labeled data to train a supervised classifier for detecting exploitation of security vulnerabilities from TI feeds.

%%
Our dataset comprises events from  191 TI feeds, including data from the default feeds of MISP~\cite{misp}.\footnote{MISP is an Open Source Threat Information Sharing Platform, which comes pre-configured with some public data feeds.  In this work, we restrict our analysis to tlp:white (=public) events and anonymize the name of the source organizations. %, and   the association between the provider organization and the community we received it from may still be confidential. 
By focusing on anonymized tlp:white events we avoid restrictive non-disclosure agreements and biases and we allow for our results to be reproduced and extended by the scientific community.}
%
To assess the effectiveness of different classifiers in detecting exploitation events in the TI feeds, we perform temporal and spatial splits of our dataset.
%
In temporal setting, the training and test sets contain past and future data, respectively. 
%
In temporal+spatial setting, the training and test sets are setup such that the TI feed used for testing is set aside during training.  
%
While F1 scores vary over different time horizons, they average around 56--78\% on average. 
%
Overall, we find that dynamic BERT embeddings outperform static Doc2Vec embedding and purpose-built specialized embeddings (i.e., TIBERT, TI2Vec) outperform their pre-trained counterparts. 
%
%When conforming to spatial constraints, we observe that the flow of information across TI feeds determine the feasibility of knowledge transfer. 

%%
Our machine learning approach to detect exploitation events from TI feeds is useful for a variety of downstream security tasks. 
%
For example, it can help organizations implement risk-aware patch management strategies. 
%
In particular, the exploitation events detected by our approach from TI feeds can be used to determine exploit code maturity level {impacting CVSS/EPSS scores.} %,  whenever CVE information is available or can be readily inferred}. 
%
Overall, our work suggests the feasibility of using TI feeds to automatically detect vulnerability exploitation in the wild, paving the way towards data-driven enrichment of vulnerability risk assessment. 


%%
Our key contributions and findings are summarized below:

 \textbf{Longitudinal analysis.} We conduct a longitudinal analysis of TI feeds, identifying the prevalence of different categories of events, such as network activity and payload delivery, across multiple organizations.  We also analyze the flow of information across TI feeds, identifying that some feeds play the role of sources whereas others behave as aggregators (Section~\ref{sec: data}).
    
\textbf{Exploitation identification. } We curate and label the events in TI feeds, e.g., indicating which of those correspond to exploitation as opposed to patch disclosures or security advisories.   To that aim, we mine for association  rules between event tags and exploitation.  Whereas tags are instrumental for curating the dataset, they require manual intervention, motivating fully automated  word embeddings (Section~\ref{sec:methods}).
    
\textbf{TI2Vec and TIBERT. } We capture semantics from loosely structured information in TI feeds using static and dynamic embeddings {(Doc2Vec and BERT, respectively and their specialized counterparts TI2Vec and TIBERT)} that are then used to train  classifiers to automatically detect exploitation of   vulnerabilities.  The training of the classifiers conforms to temporal   constraints, allowing us to assess the relevance of history on the accuracy of future predictions.   We also evaluate knowledge transfer across feeds, noting that such transfer is feasible  from TI feeds that   behave as sources to  aggregators, particularly when  the envisioned flow of knowledge is aligned with the  flow of information across TI feeds (Section~\ref{sec:results}). 
    
%    \item \hl{Mention finetuning and how it helps us learn the vocabulary}
 

\noindent \textbf{Paper organization:}
%
Section~\ref{sec: data} describes our dataset of 191 TI feeds and their key characteristics.
%
Section~\ref{sec:methods} presents our proposed machine learning pipeline to detect vulnerability exploitation in the wild.
%
Section~\ref{sec:results} reports the evaluation results,  and 
Section \ref{sec: background} summarizes related work on measurement and modeling of information in TI feeds  
before concluding.
%



% while the description of the solution is there and extensive, the description of the problem is barely there and it's rather imprecise. without that, it's hard for a reader to understand and justify why you did all this work.  
%
%you wrote something on the line of "ti feeds are high volume and unstructured so we need ML to extract relevant actionable info".
%that is imprecise if not utterly wrong.
%ti feeds are eterogeneous in nature and yes, may come in different structures. however, there are standardized established formats like stix or misp that allows different organizations to share data and to automatically process it.
% eg if i share a blacklist of ips via misp its very easy to automate blocking them at the proxy level.
% Also, data in TI feeds Is structured, often rather well.
% the probelm this work is trying to address is different:
%you/we are after some specific type of information (exploitation  of vulns) that is usually not documented and when it is, it is done in different ways (labels, comments, textual descr, etc), sometimes because the format does/did not have a unique predefined way to do it (eg misp)but usually becuase authors simply dont use it (eg in stix).
% the final result is that this info is sometimes present across feeds in unstructured textual form and therefore we need ml for parsing. 
% but thats VERY different from claiming that TI feeds are unstructured and not automatically parseable, which is a problem that instead has been addressed (with different flavors of granularity and degrees of success) throughout the past decade.



%%% generally call embeddings -- we tried Doc2Vec variations -- semantic embedings vs dynamic embedings -- BERT is the most effective


%In particular, we show that an SVM classifier using a static embedding (Doc2Vec)   is already able to detect exploitation events with a 93\% F1-score and 93\% accuracy, whereas the use of a dynamic embedding (BERT) increases F1-score to 98\% and accuracy to up to 97\% in a batch setting where all data is used for the training of the classifier. 

%
%%%%%%%%%%%%%%%%%
%
%BERT is dynamic; Doc2vec is static
%
%%%%%%%%%%%%%%%%%
%
% in related work we need to talk about threat embeddings -- training language models need to be covered
%
% generally, there is interest in adapting embedings -- repurpose, adapt to application domains
%
%  attack attribution -- https://ieeexplore.ieee.org/stamp/stamp.jsp?arnumber=8823152
% 
% Tudor Dumitra paper -- which techniques do they use?
% 
% 
% 

%https://towardsdatascience.com/from-pre-trained-word-embeddings-to-pre-trained-language-models-focus-on-bert-343815627598

% Zubair Shafiq to Everyone (21:22)

% https://dev.maxmind.com/geoip/geolite2-free-geolocation-data?lang=en
% https://web.cs.ucdavis.edu/~zubair/files/adnan-peering-icnp2017.pdf
%https://web.cs.ucdavis.edu/~zubair/files/faraz-routing-ton-2018.pdf
%Zubair Shafiq to Everyone (21:27)
% https://melaniesoek0120.medium.com/data-visualization-how-to-plot-a-map-with-geopandas-in-python-73b10dcd4b4b
%Zubair Shafiq to Everyone (22:01)
%https://towardsdatascience.com/from-pre-trained-word-embeddings-to-pre-trained-language-models-focus-on-bert-343815627598

%https://towardsdatascience.com/from-pre-trained-word-embeddings-to-pre-trained-language-models-focus-on-bert-343815627598




%and trains a supervised machine learning classifier to detect exploitation of security vulnerabilities.


%to extract contextual information in TI feeds using


%design and implementation of a system to automatically detect incidents of vulnerability exploitation from TI feeds.
%Our system extracts context information in TI feeds using a purpose-built TI word embedding (\texttt{TI2vec}) and trains a supervised machine learning classifier to detect exploitation of security vulnerabilities.
%



%CVSS does not provide a subscore to track exploitation of vulnerabilities \emph{in the wild}, and to the best of our knowledge there would currently be no tools to parametrize such a subscore from  data.  

%Risk scores such as CVSS  typically account for the aforementioned controlled events in the vulnerability lifecycle, such as patching and weaponization.   



% \vfill\eject




% but such as exploitation of vulnerabilities in the wild, are much    One of the goals of TI feeds is to 

% as the victims will typically protect themselves after publishing the feeds and 


% as the target organization will typically protect itself after reporting the events.






%Is this your own distinction or did you take it from the literature? In the second case, you should consider referencing the source

%We broadly distinguish TI feeds into two categories, depending on the sort of information shared in the feeds.  The first category encompasses information about controlled events, such as patch disclosure, security advisories and weaponization events, where the latter refers to the disclosure of proof-of-concept (PoC) or fully functional exploits without accounting for their actual use to exploit real systems.  The second category of feeds  encompasses the so called \emph{exploitation events},  which constitute our main object of study.


%Exploitation events contain information about the occurrence of events in real systems.  %We refer to this second class of events as \emph{exploitation events}, which constitute our main object of study in this work. One needs to resort either on the good faith  of the organization reporting such an  event or on public evidence supporting it to confirm its occurrence.    While controlled events can be checked and reproduced in a lab, their uncontrolled counterparts are typically non-reproducible, given the enormous amount of state variables involved in real systems and their dynamics. 

%There is a vast  set of public platforms, including the National Vulnerability Database (NVD) and  vendor websites, that reports timely, accurate and structured information about controlled events related to vulnerabilities. Exploitation events, in contrast, are arguably more valuable for risk assessment and prediction, as they indicate real as opposed to potential threats. 







%To facilitate and regulate the sharing of information within and outside such groups, communities agreed on standard protocols to ensure that sensitive information is shared with the appropriate audience~\cite{TRAFFIC_LIGHT_PROTOCOL,IEP}.

%consists mostly of unstructured information that currently requires human intervention to be parsed.

%It is also common for each participant to use its own structure and taxonomies to store and label the intel it shares. 


%patch disclosure, security advisories, proof-of-concept (PoC) or fully functional exploits, exploitation events

%Tracking exploitation events  poses its own challenges. 
%
%Firstly, many corporations are reluctant to share information concerning successful exploitation events they have been victim to due to the potential negative impact this may have on their brand or reputation.\footnote{To fight this trend many countries started to approve laws that, under certain circumstances (e.g. involvement of personal identifiable information, or for specific fields, like critical infrastructures) mandate the victims to promptly report cyber attacks to central entities, often in a matter of hours.}

%Secondly, when such information is shared, it usually happens within  trusted groups, consortia or sharing communities that, in order to preserve trust among participants, are closed in nature, often invite-only.

%To facilitate and regulate the sharing of information within and outside such groups, communities agreed on standard protocols to ensure that sensitive information is shared with the appropriate audience~\cite{TRAFFIC_LIGHT_PROTOCOL,IEP}.

%As much as standardization is desired, and sometimes partially imposed within the individual communities, different groups may have different goals and thus different requirements about the intelligence to be shared among participants. 

%It is also common for each participant to use its own structure and taxonomies to store and label the intel it shares. 

%This is mostly dictated by the fact that the primary goal of authoring Threat Intelligence information is usually the internal usage, whose requirements depend on a plethora of different factors, including software ecosystem internal processes, data sources, maturity of the TI program and staff expertise.

%\emph{The result is that, nowadays, most of the threat feeds contain information that is inconsistently structured and organized in fields that may differ significantly across different organizations.   A significant portion of the information in TI feeds is made available within free-text fields, making it extremely difficult to process it automatically.}


%
% slicing of data temporally and spatially -- random cross validation, we miss those more realistic temporal and spatial 
%
% window equal -- 2009-2015; window aggregate outperforms -- training on longer temporal dataset increases
%
% in window aggregate there is more training data -- even if more is older 
%
% difference in vocabulary -- correlates with drop in accuracy
%
% temporal + spatial: correlating sankey diagrams with results -- values with lower sinks 
%
% concept drift
%


==> docs/introduction2.tex <==
\section{Introduction} \label{sec:introduction}
Threat Intelligence (TI) has become a cornerstone of collaborative data-driven security \cite{grandview}.
%
Many organizations rely on TI feeds to assess the risk associated with security vulnerabilities and deploy countermeasures in a timely manner. 
%
The interest in TI feeds has grown over the last few years, with an increasing amount and variety of TI feeds \cite{chismon2015threat}.
%
TI feeds are now available in many different flavors---from free to commercial, from many different providers ranging from third-party firms or public groups, and targeting various kinds of threats from phishing to botnets.


%%
A key challenge in effectively leveraging TI feeds is coping with the volume of data. 
%
Large amounts of new threat information is regularly published, sometimes in excess of millions per day.
%
As the volume of threat information has increased, it has become infeasible to manually sift through them \cite{trost2014threat}.
%
Thus, automated methods to systematically sift through TI feeds are needed. 
%
Another key challenge is that TI feeds are loosely structured due to heterogeneous data sources, software ecosystems, internal processes, maturity of the TI program, and staff expertise.
%
There has been progress over the last decade to standardize information sharing in TI feeds \cite{misp,STIX}.\footnote{The Malware Information Sharing Platform (MISP) \cite{misp} and the Structured Threat Information (STIX) \cite{STIX} are two important initiatives in this direction. Both MISP and STIX establish formats that allow different organizations to share data in a uniform manner.}
%
While such standardization mitigates this challenge, a significant fraction of the information in TI feeds is made available within free-form text fields that are manually filled by security experts with differing styles.
%
These challenges make it non-trivial to automatically process the information in TI feeds to extract actionable information.


%%
In this paper, we consider the problem of detecting whether information about the exploitation of vulnerabilities in the wild is present in a given TI feed event. 
%
Detection of vulnerability exploitation in the wild is crucial for risk assessment and incident response purposes. 
%
Consider, for instance, the Common Vulnerability Scoring System (CVSS) \cite{cvss}, one of the current de facto solutions to parametrize vulnerability risk. 
%
While CVSS does provide a subscore track existence of exploits for vulnerabilities, it does not provide a subscore to track exploitation incidents \emph{in the wild}.  
%
The recently proposed Exploit Prediction Scoring System (EPSS) \cite{epss} aims to bridge this gap by forecasting whether a vulnerability will be exploited following its public disclosure.
%
Thus, information about vulnerability exploitation in the wild can complement CVSS and EPSS based risk assessment strategies. 
%
To the best of our knowledge, there are currently no large-scale measurements leveraging TI feeds to assess exploitation in the wild, or tools to leverage those measurements directly for risk assessment purposes.  


%The documentation of this information is done in different ways, through labels, comments and textual descriptions, sometimes because the TI feed format does not have a unique predefined way to do it (e.g., at MISP \cite{misp}) and sometimes because authors simply do not use the available formats (e.g., at STIX \cite{STIX}). 
%The final result is that this information is sometimes present across feeds in unstructured textual form and therefore calls for machine learning tools for automated parsing and detection. 


%%
To address the aforementioned challenges, we propose a machine learning approach to automatically ingest TI feeds for detecting vulnerability exploitation in the wild.
%
Our machine learning pipeline leverages natural language processing (NLP) based embedding techniques to parse and encode loosely structured information in TI feeds. 
%
To this end, we consider both static and dynamic embeddings techniques. 
%
Static embeddings generate the same embedding for the same vocabulary in different TI feed events: vector matrices which encode vocabulary into vectors are shared across events.  
%
Dynamic embeddings,  in contrast, aim at capturing vocabulary semantics in different contexts to address the issue of  context-dependent nature of information in TI feed events.
%
Specifically, we train a static embedding (Doc2Vec \cite{le2014distributed}) and dynamic embedding (BERT \cite{devlin2019bert}) in an unsupervised manner to capture the semantics of loosely structured information in different TI feeds. 
%
Moreover, we also train purpose-built embeddings that are further trained (or fine-tuned) on data from TI feeds. 
%
TI2Vec and TIBERT represent specialized embeddings corresponding to Doc2Vec and BERT, respectively. 
%(corresponding to BERT) 
%
%specialize vanilla pre-trained embeddings using TI feed
%\hl{and refer to the fine-tuned embeddings produced using our TI feeds as TI2Vec and TIBERT, respectively. }
%
We then leverage these embeddings along with labeled data to train a supervised classifier for detecting exploitation of security vulnerabilities from TI feeds.



%%
Our dataset comprises events from  191 TI feeds, including data from the Open Source Threat Intelligence Platform, i.e., MISP default feeds~\cite{mispdefaultfeeds}.  MISP is a threat information sharing platform, which relies on  the traffic light protocol (tlp) to determine the extent at which its events can be shared with the general public. By focusing on   the so-called tlp:white events  we  avoid restrictive non-disclosure agreements and  envision that our results can be reproduced and extended by the scientific community, which is a fundamental step towards a better understanding of the  TI feed ecosystem.\footnote{We restrict ourselves to tlp:white events, but anonymize sources as a number of them  are not part of the MISP default feeds, and   the association between the provider organization and the community we received it from may still be confidential. 
}

%
To assess the effectiveness of different classifiers in detecting exploitation events in the TI feeds, we perform temporal and spatial splits of our dataset.
%
In temporal setting, the training and test sets contain past and future data, respectively. 
%
In temporal+spatial setting, the training and test sets are setup such that the TI feed used for testing is set aside during training.  
%
While F1 scores vary over different time horizons, they average around 56--78\% on average. 
%
Overall, we find that dynamic BERT embeddings outperform static Doc2Vec embedding and purpose-built specialized embeddings (i.e., TIBERT, TI2Vec) outperform their pre-trained counterparts. 
%
%When conforming to spatial constraints, we observe that the flow of information across TI feeds determine the feasibility of knowledge transfer. 

%%
Our machine learning approach to detect exploitation events from TI feeds is useful for a variety of downstream security tasks. 
%
For example, it can help organizations implement risk-aware patch management strategies. 
%
In particular, the exploitation events detected by our approach from TI feeds can be used to determine exploit code maturity level, which can in turn be used to update CVSS/EPSS scores. 
%
Overall, our work suggests the feasibility of using TI feeds to automatically detect vulnerability exploitation in the wild, paving the way towards data-driven enrichment of vulnerability risk assessment. 


%%
Our key contributions and findings are summarized below:

\begin{enumerate}
    \item We conduct a longitudinal analysis of TI feeds, identifying the prevalence of different categories of events, such as network activity and payload delivery, across multiple organizations.  We also analyze the flow of information across TI feeds, identifying that some feeds play the role of sources whereas others behave as aggregators (Section~\ref{sec: data}).
    
    \item We curate and label the events in TI feeds, e.g., indicating which of those correspond to exploitation as opposed to patch disclosures or security advisories.  To that aim, we mine for association  rules between event tags and exploitation.  Whereas tags are instrumental for curating the dataset, they require manual intervention, motivating fully automated  word embeddings (Section~\ref{sec:methods}).
    
    \item We capture semantics from loosely structured information in TI feeds using static and dynamic embeddings {(Doc2Vec and BERT, respectively and their specialized counterparts TI2Vec and TIBERT)} that are then used to train  classifiers to automatically detect exploitation of   vulnerabilities.  The training of the classifiers conforms to temporal   constraints, allowing us to assess the relevance of history on the accuracy of future predictions.   We also evaluate knowledge transfer across feeds, noting that such transfer is feasible  from TI feeds that   behave as sources to  aggregators, particularly when  the envisioned flow of knowledge is aligned with the  flow of information across TI feeds (Section~\ref{sec:results}). 
    
%    \item \hl{Mention finetuning and how it helps us learn the vocabulary}
\end{enumerate}


\noindent \textbf{Paper organization:}
%
Section~\ref{sec: data} describes our dataset of 191 TI feeds and their key characteristics.
%
Section~\ref{sec:methods} presents our proposed machine learning pipeline to detect vulnerability exploitation in the wild.
%
Section~\ref{sec:results} reports the evaluation results,  and 
Section \ref{sec: background} summarizes related work on measurement and modeling of information in TI feeds  
before concluding.




% while the description of the solution is there and extensive, the description of the problem is barely there and it's rather imprecise. without that, it's hard for a reader to understand and justify why you did all this work.  
%
%you wrote something on the line of "ti feeds are high volume and unstructured so we need ML to extract relevant actionable info".
%that is imprecise if not utterly wrong.
%ti feeds are eterogeneous in nature and yes, may come in different structures. however, there are standardized established formats like stix or misp that allows different organizations to share data and to automatically process it.
% eg if i share a blacklist of ips via misp its very easy to automate blocking them at the proxy level.
% Also, data in TI feeds Is structured, often rather well.
% the probelm this work is trying to address is different:
%you/we are after some specific type of information (exploitation  of vulns) that is usually not documented and when it is, it is done in different ways (labels, comments, textual descr, etc), sometimes because the format does/did not have a unique predefined way to do it (eg misp)but usually becuase authors simply dont use it (eg in stix).
% the final result is that this info is sometimes present across feeds in unstructured textual form and therefore we need ml for parsing. 
% but thats VERY different from claiming that TI feeds are unstructured and not automatically parseable, which is a problem that instead has been addressed (with different flavors of granularity and degrees of success) throughout the past decade.



%%% generally call embeddings -- we tried Doc2Vec variations -- semantic embedings vs dynamic embedings -- BERT is the most effective


%In particular, we show that an SVM classifier using a static embedding (Doc2Vec)   is already able to detect exploitation events with a 93\% F1-score and 93\% accuracy, whereas the use of a dynamic embedding (BERT) increases F1-score to 98\% and accuracy to up to 97\% in a batch setting where all data is used for the training of the classifier. 

%
%%%%%%%%%%%%%%%%%
%
%BERT is dynamic; Doc2vec is static
%
%%%%%%%%%%%%%%%%%
%
% in related work we need to talk about threat embeddings -- training language models need to be covered
%
% generally, there is interest in adapting embedings -- repurpose, adapt to application domains
%
%  attack attribution -- https://ieeexplore.ieee.org/stamp/stamp.jsp?arnumber=8823152
% 
% Tudor Dumitra paper -- which techniques do they use?
% 
% 
% 

%https://towardsdatascience.com/from-pre-trained-word-embeddings-to-pre-trained-language-models-focus-on-bert-343815627598

% Zubair Shafiq to Everyone (21:22)

% https://dev.maxmind.com/geoip/geolite2-free-geolocation-data?lang=en
% https://web.cs.ucdavis.edu/~zubair/files/adnan-peering-icnp2017.pdf
%https://web.cs.ucdavis.edu/~zubair/files/faraz-routing-ton-2018.pdf
%Zubair Shafiq to Everyone (21:27)
% https://melaniesoek0120.medium.com/data-visualization-how-to-plot-a-map-with-geopandas-in-python-73b10dcd4b4b
%Zubair Shafiq to Everyone (22:01)
%https://towardsdatascience.com/from-pre-trained-word-embeddings-to-pre-trained-language-models-focus-on-bert-343815627598

%https://towardsdatascience.com/from-pre-trained-word-embeddings-to-pre-trained-language-models-focus-on-bert-343815627598




%and trains a supervised machine learning classifier to detect exploitation of security vulnerabilities.


%to extract contextual information in TI feeds using


%design and implementation of a system to automatically detect incidents of vulnerability exploitation from TI feeds.
%Our system extracts context information in TI feeds using a purpose-built TI word embedding (\texttt{TI2vec}) and trains a supervised machine learning classifier to detect exploitation of security vulnerabilities.
%



%CVSS does not provide a subscore to track exploitation of vulnerabilities \emph{in the wild}, and to the best of our knowledge there would currently be no tools to parametrize such a subscore from  data.  

%Risk scores such as CVSS  typically account for the aforementioned controlled events in the vulnerability lifecycle, such as patching and weaponization.   



% \vfill\eject




% but such as exploitation of vulnerabilities in the wild, are much    One of the goals of TI feeds is to 

% as the victims will typically protect themselves after publishing the feeds and 


% as the target organization will typically protect itself after reporting the events.






%Is this your own distinction or did you take it from the literature? In the second case, you should consider referencing the source

%We broadly distinguish TI feeds into two categories, depending on the sort of information shared in the feeds.  The first category encompasses information about controlled events, such as patch disclosure, security advisories and weaponization events, where the latter refers to the disclosure of proof-of-concept (PoC) or fully functional exploits without accounting for their actual use to exploit real systems.  The second category of feeds  encompasses the so called \emph{exploitation events},  which constitute our main object of study.


%Exploitation events contain information about the occurrence of events in real systems.  %We refer to this second class of events as \emph{exploitation events}, which constitute our main object of study in this work. One needs to resort either on the good faith  of the organization reporting such an  event or on public evidence supporting it to confirm its occurrence.    While controlled events can be checked and reproduced in a lab, their uncontrolled counterparts are typically non-reproducible, given the enormous amount of state variables involved in real systems and their dynamics. 

%There is a vast  set of public platforms, including the National Vulnerability Database (NVD) and  vendor websites, that reports timely, accurate and structured information about controlled events related to vulnerabilities. Exploitation events, in contrast, are arguably more valuable for risk assessment and prediction, as they indicate real as opposed to potential threats. 







%To facilitate and regulate the sharing of information within and outside such groups, communities agreed on standard protocols to ensure that sensitive information is shared with the appropriate audience~\cite{TRAFFIC_LIGHT_PROTOCOL,IEP}.

%consists mostly of unstructured information that currently requires human intervention to be parsed.

%It is also common for each participant to use its own structure and taxonomies to store and label the intel it shares. 


%patch disclosure, security advisories, proof-of-concept (PoC) or fully functional exploits, exploitation events

%Tracking exploitation events  poses its own challenges. 
%
%Firstly, many corporations are reluctant to share information concerning successful exploitation events they have been victim to due to the potential negative impact this may have on their brand or reputation.\footnote{To fight this trend many countries started to approve laws that, under certain circumstances (e.g. involvement of personal identifiable information, or for specific fields, like critical infrastructures) mandate the victims to promptly report cyber attacks to central entities, often in a matter of hours.}

%Secondly, when such information is shared, it usually happens within  trusted groups, consortia or sharing communities that, in order to preserve trust among participants, are closed in nature, often invite-only.

%To facilitate and regulate the sharing of information within and outside such groups, communities agreed on standard protocols to ensure that sensitive information is shared with the appropriate audience~\cite{TRAFFIC_LIGHT_PROTOCOL,IEP}.

%As much as standardization is desired, and sometimes partially imposed within the individual communities, different groups may have different goals and thus different requirements about the intelligence to be shared among participants. 

%It is also common for each participant to use its own structure and taxonomies to store and label the intel it shares. 

%This is mostly dictated by the fact that the primary goal of authoring Threat Intelligence information is usually the internal usage, whose requirements depend on a plethora of different factors, including software ecosystem internal processes, data sources, maturity of the TI program and staff expertise.

%\emph{The result is that, nowadays, most of the threat feeds contain information that is inconsistently structured and organized in fields that may differ significantly across different organizations.   A significant portion of the information in TI feeds is made available within free-text fields, making it extremely difficult to process it automatically.}


%
% slicing of data temporally and spatially -- random cross validation, we miss those more realistic temporal and spatial 
%
% window equal -- 2009-2015; window aggregate outperforms -- training on longer temporal dataset increases
%
% in window aggregate there is more training data -- even if more is older 
%
% difference in vocabulary -- correlates with drop in accuracy
%
% temporal + spatial: correlating sankey diagrams with results -- values with lower sinks 
%
% concept drift
%


==> docs/introduction_backup.tex <==
\section{introduction} \label{sec:introduction}

Threat Intelligence (TI) has become a cornerstone of collaborative data-driven security \cite{grandview}.
%
\textbf{Cite TI feed market spending numbers.}
%
Many organizations rely on TI feeds to assess risk associated with security vulnerabilities and deploy suitable countermeasures in a timely manner. 
%
There has been a steady increase in the amount and variety of TI feeds over the last few years. 
%
TI feeds are now available in many different flavors---from free to commercial, from many different providers ranging from private companies to governments, and targeting various kinds of threats from phishing to botnets.


%%
%While quality is also an issue, the 
A key challenge in effectively leveraging information from TI feeds is coping with the \textit{volume} of data. 
%
More and more threat information is being collected from a variety of sources.
%
Large amounts of new threat information is regularly published, sometimes in excess of millions per day.
%
As the volume of threat information has increased, it has become infeasible to manually sift through and figure out actionable information \cite{trost2014threat}.
%
Thus, it is imperative to develop automated methods to systematically sift through TI feeds to identify actionable information about real-world  threats. 




We broadly distinguish TI feeds into two categories, depending on the sort of information shared in the feeds.  The first category encompasses information about controlled events, such as patch disclosure, security advisories and weaponization events, where the latter refers to the disclosure of proof-of-concept (PoC) or fully functional exploits without accounting for their actual use to exploit real systems.  The second category of feeds  encompasses the so called \emph{exploitation events},  which constitute our main object of study.


Exploitation events contain information about the occurrence of events in real systems.  %We refer to this second class of events as \emph{exploitation events}, which constitute our main object of study in this work. 
One needs to resort either on the good faith  of the organization reporting such an  event or on public evidence supporting it to confirm its occurrence.    While controlled events can be checked and reproduced in a lab, their uncontrolled counterparts are typically non-reproducible, given the enormous amount of state variables involved in real systems and their dynamics. 

There is a vast  set of public platforms, including the National Vulnerability Database (NVD) and  vendor websites, that reports timely, accurate and structured information about controlled events related to vulnerabilities. Exploitation events, in contrast, are arguably more valuable for risk assessment and prediction, as they indicate real as opposed to potential threats. 
Nonetheless, the huge volume of TI feeds consists mostly of unstructured  information that currently requires human intervention to be parsed.

% actionable .

%Although the volume of % Nonetheless, the amount of
%information available about the latter is much scarcer.  

Tracking exploitation events  poses its own challenges. Firstly, many corporations are reluctant to share information concerning successful exploitation events they have been victim to due to the potential negative impact this may have on their brand or reputation.\footnote{To fight this trend many countries started to approve laws that, under certain circumstances (e.g. involvement of personal identifiable information, or for specific fields, like critical infrastructures) mandate the victims to promptly report cyber attacks to central entities, often in a matter of hours.}

Secondly, when such information is shared, it usually happens within  trusted groups, consortia or sharing communities that, in order to preserve trust among participants, are closed in nature, often invite-only.
To facilitate and regulate the sharing of information within and outside such groups, communities agreed on standard protocols to ensure that sensitive information is shared with the appropriate audience~\cite{TRAFFIC_LIGHT_PROTOCOL,IEP}.

As much as standardization is desired, and sometimes partially imposed within the individual communities, different groups may have different goals and thus different requirements about the intelligence to be shared among participants. It is also common for each participant to use its own structure and taxonomies to store and label the intel it shares. This is mostly dictated by the fact that the primary goal of authoring Threat Intelligence information is usually the internal usage, whose requirements depend on a plethora of different factors, including software ecosystem internal processes, data sources, maturity of the TI program and staff expertise.

\emph{The result is that, nowadays, most of the threat feeds contain information that is inconsistently structured and organized in fields that may differ significantly across different organizations.   A significant portion of the information in TI feeds is made available within free-text fields, making it extremely difficult to process it automatically.}

%%
In this work, we address the above challenge through the design and implementation of a system to automatically detect incidents of vulnerability exploitation from TI feeds. 
%
Our system extracts context information in TI feeds using a purpose-built TI word embedding (\texttt{TI2vec}) and trains a supervised machine learning classifier to detect exploitation of security vulnerabilities.
%
We train the machine learning classifier using expert-labeled exploitation events.
%
We then use the classifier to identify exploitation events in 191 different TI feeds. 




% but such as exploitation of vulnerabilities in the wild, are much    One of the goals of TI feeds is to 

% as the victims will typically protect themselves after publishing the feeds and 


% as the target organization will typically protect itself after reporting the events.




%%
Our system is useful for a variety of downstream security tasks. 
%
For example, it can help organizations implement risk-aware patch management strategies. 
%
Specifically, the exploitation events detected by our system from TI feeds can be used to determine exploit code maturity level. 
%
This determination can in turn be used to update Common Vulnerability Scoring System (CVSS) risk scores. 


Risk scores such as CVSS  typically account for the aforementioned controlled events in the vulnerability lifecycle, such as patching and weaponization.   CVSS does not provide a subscore to track exploitation of vulnerabilities \emph{in the wild}, and to the best of our knowledge there would currently be no tools to parametrize such a subscore from  data.  Our system suggests the  feasibility of using   TI feeds to  automatically tag  vulnerabilities that have been exploited in the wild, paving the way towards enriching CVSS and alternative risk scores with this additional  dimension.





%%
In summary, this paper makes the following contributions:

\begin{enumerate}
    \item we  conduct a longitudinal analysis of 
    TI feeds, identifying the prevalence of different categories of events, such as network activity and payload delivery, across multiple organizations
    \item we curate and label the collected TI feeds, e.g., indicating which of those correspond to exploitation as opposed to controlled events such as weaponization and patching
    \item we extract contextual information from TI feeds using a purpose-built TI word embedding (\texttt{TI2vec}) that is then used to train a supervised machine learning classifier to detect exploitation of security vulnerabilities 
    \item we train classifiers to automatically filter exploitation events from the collection of TI feeds, contrasting different alternatives and deriving insights that shed light into the TI feeds. For instance,  leveraging \texttt{TI2vec}  to produce features that are used  to   train a decision tree,  we discover that the NjRat malware is responsible for 21\% of the exploitation events in our dataset.
\end{enumerate}

The remainder of this paper is structured as follows. In the upcoming section we present related work. Then, Section~\ref{sec: data} describes our dataset and Section~\ref{sec:methods}  presents the methodology to  label TI feeds and to produce \texttt{TI2vec} and  train TI feed classifiers. Section~\ref{sec:results} reports our results, and Section~\ref{sec:conclusion} concludes. 


% \vfill\eject



==> docs/methods.tex <==
\section{TI Feed Classification}
\label{sec:methods} 
The increasing volume of loosely-structured information in TI feeds renders them unwieldy for manual sifting, calling for methods to extract actionable information in an automated manner.    
%
In this section, we present a machine learning pipeline to automatically analyze and classify TI feed events.
%
Our proposed machine learning pipeline first leverages state-of-the-art natural language processing (NLP) techniques to extract semantic information from TI feeds and then trains supervised machine learning models for classification.  


\subsection{Problem statement}
We focus on the problem of detecting exploitation of security vulnerabilities from TI feeds, {classifying  TI feed events for that matter}.\footnote{Note that this problem is related but different compared to vulnerability weaponization (i.e., whether an exploit for a particular vulnerability exists) \cite{Frei06vulnerabilityanalysis,Bozorgi10exploitprediction,Shahzad12vulnerabilitylife}. In particular, weaponization can be determined in a controlled environment, whereas exploitation requires measurements in the wild.} 
%
This is a useful undertaking because exploitation information is crucial for threat response and vulnerability management. 
%
The most concrete application is the recently proposed Exploit Prediction Scoring System (EPSS) \cite{jacobs2021exploit}, which specifically aims to predict the likelihood of vulnerability exploitation after disclosure. 
%
EPSS scores (i.e., likelihood that a vulnerability will be exploited within the 12 months following its public disclosure) are calculated based on a regression model that takes into account features such as the vendor's name and whether a proof-of-concept exploit has been developed~\cite{jacobs2021exploit}.  
%
Measurement and detection of exploitation events in the wild essentially provides the ground truth for EPSS scores. 
{  Indeed, after an  event is  classified as an exploitation, the set of vulnerabilities in the attack surface of the environment where the exploitation occurred are natural candidates to have their CVSS/EPSS scores updated.}
%
% Since EPSS is parametrized from data, e.g.,  IoC sightings,  shared by multiple organizations,
% and each organzination 
% it is instrumet
%
% TI Feed text
% ===> CVE id
% ===> EPSS
%
% TI Feeds 
% ===> organization ===> CVE ids that affect the organization
% ===> EPSS
%
%
%
%
%and the knowledge of the CVEs, 
%
%our TI Feed data can be used to infer information about (1) CVE information or (2) their organization.  % 
%
Thus, we aim to build models to automatically classify TI feed events into two classes: \textit{exploitation} and \textit{non-exploitation}. 


\subsection{Ground truth}
We need labeled ground truth to train and test our machine learning classification pipeline.
%
Thus, we discuss our approach to bootstrap ground truth using a small set of TI feed events that are painstakingly labeled by experts manually. 


\textbf{Manual labeling by experts. }
We begin by filtering TI feed events that mention specific vulnerabilities (i.e., CVE–ID) in their textual descriptions, comment, or IoC attributes. 
%
The filtered TI feed events are then manually labeled by two independent experts, with 10\% concurrently labeled events achieving the inter-rater agreement score of 89\%.
%
The experts used the following code book to manually label exploitation events.
%
Events that are labeled exploitation:   
%
(1) have a definite malicious components such as APTs, DDoS, and trojan attacks; 
%
(2) are part of a well-known malicious campaign; 
%
(3) mention a well-known hacker group/organization; or 
%
(4) contain keywords such as espionage or campaign (given suitable surrounding context).  %The event illustrated in the  Supplementary Material~\cite{supplementarymaterial}, for instance, was labeled as an exploitation event since it fits criteria (2), (3), and (4).
%
In contrast, events that are labeled non-exploitation:   
%
(1) are updates to existing software without a malicious component for that update;
% 
(2) contain keywords such as patch, update, reset (given suitable surrounding context); 
%
(3) have no clear-cut indication of malicious action; or
%
(4) contain insufficient data or ambiguous terminology to be classified as exploitation. 
%
This manual procedure was used to label four thousand events.


\textbf{Event tags. }
\label{subsec: tags}
Each event in TI feeds may contain one or more tags.\footnote{Tags are referred to as `machine tags' in MISP.} 
%
Composed of a namespace, predicate, and optional value, a  tag of the form namespace:predicate=value can be utilized to further classify an event. "misp-galaxy:threat-actor=Sofacy" and "tlp:white" are examples of tags in an exploitative event. % (see   Supplementary Material~\cite{supplementarymaterial}).
%
These tags are part of the MISP taxonomies \cite{misp}, which allow various organizations to adopt standard classification vocabulary. 
%
The tags are manually assigned to each event and are designed for automated consumption by downstream tasks (e.g., intrusion detection systems).
%
There are drawbacks to this approach as bias from a security expert could sway which tags are being added and tagging each event is time intensive. 
%
On the other hand, it can be easier to control quality with manual tagging. 
%
Since every event in our dataset is annotated with at least one tag, tags could be utilized as a baseline for classification analysis. 


%%
We analyze the distribution of tags in the top-10 feeds in our dataset. 
%
Figure \ref{fig:FrequencyTagBreakdown} plots the percentage of each tag type in terms of all tags found per feed. 
%
% A frequent tag was ``tlp:white'' (>20{\%} per feed) indicating that the information included could be shared publicly and had no risk of misuse. 
%
In most feeds, the events typically contain 2-3 tags. 
%
Common tags across feeds include circl:incident-classification=``malware'', malware:emotet, type:\-osint, and malware{\_} classification:malware-category=  ``ransomware''. %
The specific nature of each tag helps to verify the focus of an event. 
%
Since tags are manually added and hold pertinent information about an event, they may be useful in determining exploitation incidents. 


\begin{figure}[!t]
    \centering
     \includegraphics[width=\columnwidth]{docs/figures/tag-percent-breakdown-anon.pdf}
       \precaption
          \vspace{-.2in}
    \caption{Breakdown of   common tags throughout top 10 feeds}
    \label{fig:FrequencyTagBreakdown}
    \postcaption
    \vspace{-.25in}
\end{figure}


\textbf{Automated labeling based on event tags. }
To expand ground truth beyond the four thousand manually labeled events, the rest of the labeling process was automated using these event tags. 
%
%Each event can contain multiple tags from this taxonomy and these tags help provide information about the event. 
%For information regarding the structure of a tag and the full list of the different tags, see https://www.misp-project.org/taxonomies.html.
%%
Specifically, we extracted association rules between event tags and exploitation on manually labeled events. 
%
We used the {apriori} algorithm with support $\geq$ 0.001, confidence $\geq$ 0.5, and lift $\geq$ 1 to shortlist approximately 735 rules. 
%
Note that we filtered some unrelated tags (e.g., \texttt{tlp}) before extracting association rules. 
%
Once the rules which mapped combinations of tags to exploitation were generated, these rules were used to determine the ground truth for the remaining ten thousand unlabeled events. 
%
More specifically, an event was labeled as an \textit{exploitation} if and only if all of the tags in at least one of the shortlisted rules matched the tags of the event. 
%
If not, the event was marked as \textit{non-exploitation}. 
%
For example, the apriori algorithm determined a rule \texttt{sectorfinancial} \& \texttt{kill-chain:delivery} \& \texttt{kill-chain:command and control} $\rightarrow$ \textbf{Exploitation}, meaning that if each of “sectorfinancial”, “kill-chain:delivery”, and “kill-chain:command and control” tags are present then it  would be labeled as an exploitation event. %



\textbf{Label distribution. }
%
We note that 11\% of  events in the top 10 feeds were labeled as exploitation and 
%
%Further, we note that a the majority of events within a feed tended to have one label.
%
  the distribution of threat events varies across different feeds. 
%
For example, {\inThreat} and {\INCIBE}  had approximately 89\% and 87\% of their events labeled as exploitation, respectively.
%
This is in stark contrast to the ground truth labeling results of feeds such as {\InnoTecSystem}, {\Barncat}, and {\Cryptolaemus}, all of which had no exploitation events.
%
Across all TI feeds in our dataset, 82\% of the events were labeled as non-exploitation and the remaining 18\% were labeled as exploitation. 



\textbf{Summary. }
The rule-mining mechanism   effectively automates the labeling procedure, but leverages  manually curated event tags for its purpose.  The classifiers  considered in the remainder of this paper, in contrast, are useful even when  event tags are not  present, e.g.,  for feeds with no tags, or as soon as IOCs are  produced.   To evaluate the accuracy of those classifiers, in turn,  it is key to conform to temporal and spatial constraints, as described next.


 

\begin{comment}

\begin{table}[!t]
\centering
%\scriptsize
% \footnotesize
\precaption \caption{Results from ground truth labeling for top-10 TI feeds.}
\arrayrulecolor{black}\resizebox{\columnwidth}{!}{
\begin{tabular}{!{\color{black}\vrule}l!{\color{black}\vrule}r!{\color{black}\vrule}r!{\color{black}\vrule}r!{\color{black}\vrule}r!{\color{black}\vrule}r!{\color{black}\vrule}r!{\color{black}\vrule}r!{\color{black}\vrule}r!{\color{black}\vrule}r!{\color{black}\vrule}r!{\color{black}\vrule}r!{\color{black}\vrule}} 
\hline
%~                & \multicolumn{1}{l!{\color{black}\vrule}}{\CERTBund} & \multicolumn{1}{l!{\color{black}\vrule}}{\CIRCL} & \multicolumn{1}{l!{\color{black}\vrule}}{\inThreat} & \multicolumn{1}{l!{\color{black}\vrule}}{\InnoTecSystem} & \multicolumn{1}{l!{\color{black}\vrule}}{\CthulhuSPRL} & \multicolumn{1}{l!{\color{black}\vrule}}{\DCSO} & \multicolumn{1}{l!{\color{black}\vrule}}{\Barncat} & \multicolumn{1}{l!{\color{black}\vrule}}{\Cryptolaemus} & \multicolumn{1}{l!{\color{black}\vrule}}{\Crimeware} & \multicolumn{1}{l!{\color{black}\vrule}}{\INCIBE} & \multicolumn{1}{l!{\color{black}\vrule}}{Total}  \\ 
%~ & Feed & Feed & Feed & Feed & Feed & Feed & Feed & Feed & Feed & Feed  & Total \\
Feed ID &  1 &  2 &  3 &  4 &  5 &  6 &  7 &  8 &  9 &  10 &  Total\\
\hline \hline
Exploitation     & 108                                                 & 766                                             & 116                                                    & 0                                                        & 92                                                       & 182                                            & 0                                                 & 0                                                      & 5                                                   & 48                                               & 1317                                             \\ 
\hline
Non-exploitation & 536                                                 & 468                                             & 14                                                     & 6955                                                     & 28                                                       & 48                                             & 1623                                              & 613                                                    & 133                                                 & 7                                                & 10425                                            \\
\hline
\end{tabular}}
\arrayrulecolor{black}
\label{table: ground truth}
\end{table}

\end{comment}

%are typically  restarted by operating systems 
%During normal operation, the computer regularly restarts the watchdog timer to prevent it from elapsing, or "timing out". 
%
% `Cryptolaemus', for instance, is a white hat group that reports vulnerabilities and appears in the word cloud of non-exploitation events.  
%
%One of the major targets of the group is the `emotet' malware, suggesting that the presence of such term in an event signals that the target host is vulnerable to the malware.  
%
%It is also noteworthy the presence of the term `update' in the non-exploitation even cloud, indicating that vulnerabilities require systems or IoC updates, as opposed to exploitation events that report that the system was `updated', in retrospect. % Note also that the presence of words in an event does not necessarily determine its class. % The word `abuse', for instance, typically appears in non-exploitation events, in the context of potential but non-realized abuses, e.g., as reported at  \url{https://urlhaus.abuse.ch/}.



\subsection{Longitudinal evaluation}
A key challenge in detecting incidents such as vulnerability exploitation is their constantly evolving arms race nature. 
%
Thus, it is important to evaluate the accuracy of detection models in a longitudinal manner as classifiers need to evolve over time in response to the dynamic threats. 
%
To this end, we use two methods to split the dataset for training and testing: \emph{temporal} and \emph{temporal+spatial}.


\textbf{Temporal splits. }
To evaluate the accuracy of our classification models in a longitudinal setup, we split our entire dataset into distinct time windows such that the earlier windows are used for training and the later windows are used for testing. 
%
Thus, we make sure that the events in the train set occur prior to those in the test set.
%
We consider two different approaches to longitudinally split our dataset: aggregate window and equal window. 
%
%The fixed split method uses the first 70\% events for training and the remaining 30\% events for testing. 
%
Both aggregate window and equal window splits divide data into 11 time windows such that each window contains an equal number of events. 
%
In aggregate window split, the model uses the events in the next time window for testing and the events in all previous time windows for training. 
%
Thus, the amount of training data increases over time as more time windows are accumulated.
%%%%%% in equal window splits.
%
In equal window split, the model uses the events in the next time window for testing and the events in the immediately preceding time window for training. 
%
Thus, the amount of training data remains the same over time in equal window splits. 
%
Such temporal splits would help us evaluate whether the accuracy of our machine learning pipeline is sensitive to the amount and recency bias of training data.



\textbf{Temporal+spatial splits. }
We further build upon the aforementioned temporal splits by additionally splitting events across different TI feeds. 
%
Specifically, we consider the scenario where a feed is not available during the training but its events need to be classified at the test time. 
%
Thus, the test set is restricted to contain events only from one feed and the associated train set contains no events from that feed while respecting the aforementioned temporal splits. 
%
For example, consider  {\CIRCL}. 
%
If we split spatially, the train set of each window will not contain any events from {\CIRCL}, while the test set will only contain events from {\CIRCL}.
%
Such temporal+spatial splits would help us evaluate whether the accuracy of our machine learning pipeline generalizes to other previously unseen feeds. 
 

\subsection{Features}
%%
Next, we explain our feature extraction pipeline. 



\textbf{Pre-processing. }
Before features are extracted, we conduct standard pre-processing, including splitting the text on all special characters, such as hyphens, and removal of stop words.
%
Some IoCs, such as hashes, might refer to a malware payload, and receive special treatment. 
%
As threats have polymorphic capabilities to mask file signatures, most hashes are unique to one feed.
%
This, in turn, implies that information about hashes cannot be readily generalizable across feeds.   
%
To address this issue, we replace all instances of hashes with an abstract representation noting the existence of a hash value.


\textbf{Feature extraction. }
We consider two different embedding-based feature extraction techniques. 
%
First, we use a context-independent static embedding technique, called Doc2Vec \cite{le2014distributed}.
%
Doc2Vec maps all words in an event to a feature vector such that it captures the relationship between a word given its neighboring words. 
%
Second, we use a content-dependent dynamic embedding technique, called Bidirectional Encoder Representations from Transformers, BERT~\cite{devlin2019bert}. 
%
BERT maps all words in an event to a feature vector using an attention-based model that learns contextual relations between words in a text. 
%
We use BERT base uncased  in~\cite{xiao2018bertservice} to encode our input data into fixed-length vector representations. 
%
As compared to Doc2Vec, which generates the same embedding for the same word in different contexts, BERT is better able to capture the semantics by modeling the surrounding context of an input word. 
%
For both Doc2Vec and BERT, we not only consider pre-trained models but also train purpose-built models that are further trained on data from TI feeds. 
%
For Doc2Vec, we train TI2Vec in an unsupervised manner using the corpus of 191 TI Feeds in our dataset. Training is done over 15 epochs. This customized embedding aims to capture the context of domain specific vocabulary that is typically found in TI feeds. With BERT for sequence classification, we train TIBERT in a supervised manner from the standard BERT-base-uncased model with our TI dataset. We utilize a classification layer to fine-tune it over 10 epochs.
%First, binary feature extraction (or simply bag-of-words) corresponds to a one-hot encoding of words in an event. 
%
%Second, TF-IDF feature extraction corresponds to a numerical statistic accounting for how often a word is used in an event and amongst all events. 
%

%
%A discussion of additional details on the BERT attention model is deferred to Section~\ref{sec:visual}.


\textbf{Feature selection. }
We perform feature selection to avoid over-fitting.
%
%We choose the top 1000 features with highest term frequency for Binary and TF-IDF feature sets. 
%
For {Doc2Vec}, we select $n$ to be 1000. 
%
For BERT, input is transformed into 768-dimensional vectors.


\textbf{Supervised classification. }
Given the features and labeled dataset, we train different supervised machine learning algorithms to classify TI feed events.  
%
We begin by considering Naive Bayes and Decision Tree classifiers, as both serve to classify  non-linearly separable classes, with Naive Bayes relying on conditional independence among features for that purpose.  
%
Following the discussion in Section~\ref{sec: data}, there are significant inter-dependencies across features within each class, suggesting that Decision Trees are better suited than Naive Bayes. 
%
As a natural extension to  Decision Trees, we also consider the AdaBoost ensemble classifier.  
%
Boosting in that context consists of using many  low-fidelity Decision Trees, which together are supposed to outperform a single tree. 
%
While the Decision Tree is amenable to interpretability, ensemble classifiers tend to provide better classification performance.
%
Finally, TIBERT has a built-in head that classifies the transformer's vector representation of the input based on what was learned during training, i.e., different from the other considered approaches, TIBERT learns to produce its embeddings and to classify events through a unified framework. 





\begin{comment}

% in a  watune the number   % we use a different method since the individual features are condensed into $n$-dimensional vectors. 
% we tune the number of vectors were used to describe a single document. 

% To fairly  compare the number of features from TF-IDF and Binary methods against Doc2Vec, we typically  match the number of features used by the former two methods against the dimension of the vectors used by Doc2Vec.  Note that the pre-trained doc2vec model  
% generates 300-dimensional vectors.
%For the \textsc{TI2vec} models trained with our dataset, in contrast,  we consider $n$ ranging between 100, 300, 500 and 1000. % vector outputs. 



% It is also worth noting that while deriving the features one needs to determine the amount of steps used to infer the  vector corresponding to a given document. Usually the higher the steps for inference the more likely two similar documents will converge. For our custom model we use 500 steps. 

% is trained with our own TI feed data. The pretrained doc2vec model generates 300-dimentional vectors only.


%The cybersecurity domain specific language in  we wanted to measure the performance of a general use doc2vec model against our custom trained doc2vec. The pre-trained doc2vec model was trained with the entire corpus of Wikipedia, our model is trained with our own TI feed data. The pretrained doc2vec model generates 300-dimentional vectors only. Our models were made to generate 100,300,500,1000 vector outputs. The best performance is at 1000 vectors.


%why did you use the sizes of vectors, 
%discuss any other parameters used



%Put this under feature selection near the end of doc2vec
%Due to the domain specific language in cybersecurity we wanted to measure the performance of a general use doc2vec model against our custom trained doc2vec. The pre-trained doc2vec model was trained with the entire corpus of Wikipedia, our model is trained with our own TI feed data. The pretrained doc2vec model generates 300-dimentional vecors only. Our models were made to generate 100,300,500,1000 vector outputs. The best performance is at 1000 vectors. In addition to this vector size parameter there is also the amount of steps used to infer a vector. Usually the higher the steps for inference the more likely two similar documents will converge. For our custom model we use 500 steps. 




%The polarity score is a value ranging between -1 and 1. 



%As discussed in Section~\ref{sec: data},  a number of IoCs are shared across TI feeds.  
%
%Other IoCs, however, require special treatment. 
%
 %After this was complete a derived feature was created for each event this feature was generated by a sentiment analyser. % here
%

%creating derived features, and formatting. For Binary features and TF-IDF the same method of pre-processing was used. This was performed by splitting the features on special characters, and 
% here
% Doc2Vec  goes through an 
%Additional steps include  % uses a stronger
%data cleaning step, wherein %. It first removes any stop words, next 
%splitting the text   on all special characters, such as hyphens. Any of the pieces %. Next if there are features 
%with a length over 30 characters, which typically correspond to file hashes, receive special treatment, as indicated below, and are then removed. 

%or less then 2 characters %the entire feature 
%are removed. This results in more words being captured as individual features  and less hashes or IP addresses. The rationale is to increase the number of generalizable features, rather than keeping  data that is specific to one event such as a file signature. 

% The intuition behind this is to have the Doc2Vec model is not given data that is specific to one event such as a file signature. Instead we use this method of cleaning to better generalize the data the Doc2Vec model uses, and therefore generates. 

%We empirically discover that Sentiment is widely generalizable, serving well for the purposes of . 

%and sentiment \cite{wikiDoc2vec}. 
%added this to describe sentiment
%In particular, the advantage of sentiment analysis is the ability to assign a positive or negative value to the sentiment of the statement. Sentiment is widely generalizable, and as a metric can be used to compare threat events against each other. 


\subsection{Ground Truth  and Classification}

% Question: Are the classes exploitation and weponization?


\textbf{Manual Ground Truth Labeling. }
We resort on supervised training of machine learning models to filter  exploitation events from the collection of TI feeds. To that aim, we manually labeled the TI feeds  with our two target categories:  exploitation and non exploitation. 

% Crime BB related. Paragraph removed.
% For the CrimeBB dataset we followed the same methodology, but allowing one additional class: exploitation, weaponization and other. The latter class encompasses proof-of-concept (PoC) and other events.

% Crime BB related. Paragraph removed.
% To analyse the discussions of vulnerabilities in Hackforums, we filter from the dataset what we call special threads. These threads contain 1 or more posts citing vulnerabilities. By reading the discussions of each of these threads, we classify them according to their danger level. We define the following 3 classes in ascending order of threat level:

%To analyze events in TI Feeds, 

We begin by filtering from the dataset events that mention at least one vulnerability in their textual descriptions, commentaries or attributes. %These events can contain 1 or more cited vulnerabilities. 
Then, we read each of the remaining TI feeds, and classify them with respect to whether they refer to an attempt to exploit a vulnerability in real systems. While going through the TI feeds, we learned that the following heuristics are  helpful to filter exploitation events. Events that    %read By reading these descriptions and commentaries, we classify them according to their threat level. We developed the following heuristics for consistent class categories for events that 
%
% Text removed
% For our two classes we used data from the textual description of the event to inform our decision making.
%
% Text removed
% If one of the following heuristics is met the classification is threat event. 
%
%\begin{enumerate}
   $(1)$ have  a definite malicious components such as APTs, DDoS, and Trojan attacks; 
    $(2)$ contain keywords such as ransomware, espionage, targeted, and campaign; 
    $(3)$ are  part of an existing malicious campaign; or
    $(4)$ mention a known malicious group/organization are typically exploitation events. 
%\end{enumerate}

The following characteristics, in contrast, were typically used to label non exploitation events. Events that 
%\begin{enumerate}
  %  \item
  $(1)$  were updates to existing software without a malicious component for that update;
    $(2)$ contained keywords such as patch, update, reset; 
    $(3)$   contained insufficient data to classify as threat;
    $(4)$
      had no clear malicious action;
 $(5)$ had ambiguous terminology that could not be determined as malicious are typically non exploitation events.  
    
% \end{enumerate}


% Crime BB related. Section removed.    
% These keywords are from crimeBB.
    %   keywords: 
    %   - fud*
    %   - money, price, bitcoin
    %   - sell, trade
    %   - buy
    %   - packs
    %   - metasploit
    %   - code**
      
    %   * Fud kits or exploits are considered to be weaponization?
      
    %   ** in case someone is sharing a code because is trying to hack



% Crime BB related. Section removed.
% 3) Exploitation: 
%       While in weaponization threads there is no conclusion of exploits being used, exploitation threads are assertive regarding 
%       an exploitation being available in the wild. In these threads, we see confirmed trades and exploitations
%       by Hackforums' members. We envision that our model will have a higher precision for classification of threads of this class.



The whole dataset was labeled by two of the co-authors, with 10\% of the events being labeled concurrently by the two, with disagreement score~\cite{soberon2013measuring} of 11.162\%.





% \subsection{Supervised classifier}

\textbf{Supervised Classifier.}
Given the labeled and  curated dataset, we  leverage machine learning tools to classify the TI feeds.  We  begin by considering  Naive Bayes (NB) and  decision tree classifiers, as both serve   to classify  non-linearly separable classes, with NB relying on conditional independence among features for that purpose.  % classification, but relies on independence among features  
Following the discussion in Section~\ref{sec: data}, there are significant  interdependencies across features within each class, suggesting that decision trees perform better than NB. % classifiers as the latter is oblivious to such dependencies.  
As a natural extension to  decision trees, 
we also consider  an AdaBoost
Random Forest (RF) classifier.  
Boosting in that context consists of using many  low-fidelity  decision trees, which together yield better accuracy than a single  tree. 
 % as well as deep learning techniques such as Convolutional Neural Network (CNN)
While  the decision tree is  amenable to interpretability, allowing us to illustrate its pruned version in Section~\ref{sec:results},    ensemble classifiers such as RF % is an ensemble classifier known 
provide better prediction accuracy.


\end{comment}

%, but are not as trivially interpretable as  simple decision trees.  

%{\bf explain why boosting is expected to help? noisy data?}


%Boosting is expected to help in problems involving noisy data, 



% naive bayes and decision tree very close
% noisy ground truth
% manually labeling experts, noisy data
% 
% copy from proposal from Zubair

%
% 
% preview
% adaboost -- meta classifier, ensemble decision tree
% why boosting is expected to help
% naive bayes and decision tree very close
% noisy ground truth
% manually labeling experts, noisy data
% 
% copy from proposal from Zubair
%
% single column figure 
%
% complicte pipeline? feeds --> features --> 
%
% TI feeds -- feature, exploit labeling, model, trained model, label, test TI feed
% 
%

% recap: setup problem
% all discussion tighetd to problem
% ground truth
% labeling
% ML classifiers
%

%\emph{in the introduction: emphasize that innovation of the paper is on measurements rather than on methods -- }

%pull up something from results to here

%provide high level descriptions of the following (from simpler)

%naive bayes - good for non-linear classification, but relies on independence among features

%decision tree - good for non-linear classification, and does not rely on assumptions

%adaboost - ensemble classifier (ensemble of trees) -- better than decision trees, but less interpretable


%We use 3 machine learning models to classify our data. Naive Bayes, Decision Tree, and Ada boosted Decision trees. Naive Bays establishes a baseline for performance. Naive Bayes does perform well with non-linear classification, however one major limitation to the use of Naive Bayes it that it assumes total Independence between features. Decision trees differ in this respect to Naive Bays as they allow for interdependence between features, but is best with binary classification. 
%better explain why the models matter



% Due to the relation of threat attributes interdependence is an important interaction to capture.  In addition, Decision trees are interpretable, and their process easily explainable. For additional performance we use boosting. Boosting is the process of using many, low-fidelity learners and using them together in an iterative process. In the case of Adaboost incorrect predictions are given a higher weight, the more errors made for a specific prediction the higher the weight there is to correct that prediction. Using these many weak learners the model is better able to capture sophisticated interactions within the data, with the cost of a less interpretable model then compared to decision trees.



\begin{comment}
\begin{table}[h]
    \centering
    \begin{tabular}{l|c|c}
         \hline
         Method & Threat feeds & Blackhat forums \\
         \hline
         Decision tree (CART algorithm) & & \\
         Decision tree (C4.5) & & \\
         Naive Bayes & & \\
         SVM & & \\
         Random forest & & \\
         ADA Boost & & \\
         \hline
    \end{tabular}
    \caption{Caption}
    \label{tab:my_label}
\end{table}

\end{comment}




% Crime BB related. Section removed.    
% These keywords are from crimeBB.
    %   keywords: 
    %   - fud*
    %   - money, price, bitcoin
    %   - sell, trade
    %   - buy
    %   - packs
    %   - metasploit
    %   - code**
      
    %   * Fud kits or exploits are considered to be weaponization?
      
    %   ** in case someone is sharing a code because is trying to hack



% Crime BB related. Section removed.
% 3) Exploitation: 
%       While in weaponization threads there is no conclusion of exploits being used, exploitation threads are assertive regarding 
%       an exploitation being available in the wild. In these threads, we see confirmed trades and exploitations
%       by Hackforums' members. We envision that our model will have a higher precision for classification of threads of this class.



%The whole dataset was labeled by two of the co-authors, with 10\% of the events being labeled concurrently by the two, with disagreement score~\cite{soberon2013measuring} of 11.162\%.




%We resort on supervised training of machine learning models to filter  exploitation events from the collection of TI feeds. To that aim, we manually labeled the TI feeds  with our two target categories: exploitation and non exploitation. 

% Crime BB related. Paragraph removed.
% For the CrimeBB dataset we followed the same methodology, but allowing one additional class: exploitation, weaponization and other. The latter class encompasses proof-of-concept (PoC) and other events.

% Crime BB related. Paragraph removed.
% To analyse the discussions of vulnerabilities in Hackforums, we filter from the dataset what we call special threads. These threads contain 1 or more posts citing vulnerabilities. By reading the discussions of each of these threads, we classify them according to their danger level. We define the following 3 classes in ascending order of threat level:

%To analyze events in TI Feeds, 





%Given our limited man-hour budget  to label the dataset, simplifying the labeling task allowed us to count with multiple manual labels for a subset of our samples, which builds robustness and confidence into the obtained labels.
%Second, having two classes  avoids ambiguity between multiple classes. 
%

%Third, having two classes  simplifies the task of manual labeling. 
%




%First, one of our main goals is to analyze exploitation in the wild, as events on weaponization were already analyzed by previous efforts, e.g., accounting for the ExploitDB dataset..  
%

%The features associated to each event are its IoCs.  

% The rationale for considering two classes stems from the fact that TI feeds are envisioned to assist in software vulnerability risk assessment. Although there is a vast amount of structured information about non exploitation  events, such  as patch disclosure, security advisories and weaponization events much less is known about exploitation events in the wild.  One needs to resort either on the good faith  of the organization reporting such an  event or on public evidence supporting it to confirm its occurrence.   Therefore, filtering  such events is instrumental to complement the structured information made available through other sources, such as vendors websites, ExploitDB and NVD, and for concreteness we consider this target application in the remainder of this paper. 


%Exploitation events contain information about the occurrence of events in real systems.  %We refer to this second class of events as \emph{exploitation events}, which constitute our main object of study in this work. One needs to resort either on the good faith  of the organization reporting such an  event or on public evidence supporting it to confirm its occurrence.    While controlled events can be checked and reproduced in a lab, their uncontrolled counterparts are typically non-reproducible, given the enormous amount of state variables involved in real systems and their dynamics. 




% Next, we describe the methods used to identify relevant information in the TI feeds, focusing on the filtering of vulnerability exploitation. 

% As in any information extraction exercise, we have to trade-off  between generality and  specifics of the domain at hand.

\begin{comment}
In what follows, we begin with a brief overview of three text mining strategies common in the literature, from the most general to the one that most explores the specifics of TI feeds.

\begin{enumerate}
\item \textbf{Off-the-shelf text mining (classic mining): } More general methods involving off-the-shelf text mining tools, e.g., text binarization and TF-IDF, already allowed us to classify threat feed events 
\item \textbf{Context dependent text mining (deep mining): } Then, specializing those methods with pre-trained word embeddings, such as Doc2Vec, allowed us to get increased accuracy~\cite{wikiDoc2vec, rehurek_lrec}.    % (\textbf{is there a special doc2vec version that takes dates/timestamps in the input and treat them differently?})
\item  \textbf{Context dependent text mining with augmented features: } 
Out-of-band features, such as the number of IP addresses contained in each event, as well as contextual information related to the TI feed domain, can be leveraged by   training a purpose-build word embedding ({TI2Vec}) 
\end{enumerate}


\end{comment}

 %none of the methods above explore the subsumed structure of the dataset.  In particular, 


% Note that all the methods considered  account for the whole dataset as a collection of textual documents.  This is due to the fact that, while the information in TI feeds is mostly represented by  IoCs, a significant fraction of the content is actually stored with free text. As the vulnerability information we are looking for in this work is often stored within the description of the events or in other free text fields, we opted for  solutions that can naturally embrace the heterogeneity of our source data. 


%providing a unified framework to handle it.  Using the structure of the dataset, the classifiers can be tuned. To that aim, one can take into account IoCs in TI feeds as  structured features, some of which containing free text in their instances as a special case. However, we leave such an analysis as subject for future work, noting that structure must be extracted as a function of the features available in the dataset.


% \textbf{Zubair: This does not fit in section 3. I think it should be explain in feature extraction. Daniel, please take a look.}



%Prior research on detection  research does not respect space and time when determining vulnerabilities. 
%We consider that having technically valid results involves splitting our data with respect to time. 
%



%- explain why modeling needs to respect space/time (streaming)

%-- particularly important because security arms race (threats evolve)

%--accordingly, ml pipelines need to be updated in a streaming fashion (concept drift)

%--thus evaluation needs to reflect spatial/temporal cross-validation


%- explain why focus on this problem of exploitation detection (borrow/expand from introduction)


% \usepackage{colortbl}




==> docs/results.tex <==
\section{Experimental Evaluation}
\label{sec:results}


%\subsection{Evaluation metrics}
To evaluate the accuracy of our classifiers, we use three well-known metrics: precision, recall, and F1 score. 
%
Precision is the fraction of presumed exploitation events that are correctly detected.
%
Recall is the fraction of exploitation events that are detected. 
%
The F1 score combines precision and recall through their harmonic mean. 
%
Our dataset has imbalanced class distribution {(82\% non-exploitation; 18\% exploitation)}; thus, we focus on F1 score here.
%
Due to space constraints, we do not include precision and recall results that show similar overall trends.

%
%The detailed precision and recall results showing similar overall trends are reported in Appendix \ref{subsec: appendix temporal tables} (Tables \ref{table: appendix-binary-temp}--\ref{table: appendix-bert-temp}). \hl{Are we reporting precision/recall in appendix otherwise we should remove this line?}

%\input{docs/TempTable}
\input{docs/results_tables/impact_of_approach}

%\subsection{Results} \label{sec:temposplit} 
%
%Split IDs with additional details about the time and size of training and testing data for each split are reported in Table \ref{table: metadata}.
%

%Results shown are limited to Doc2Vec and BERT due to their significantly better performance; however, Binary and TF-IDF results are included in Appendix \ref{subsec: appendix temporal tables} (Tables \ref{table: appendix-binary-temp}--\ref{table: appendix-tfidf-temp}) for completeness.
%
%
%Among different split types, equal outperforms aggregate window. 
%Among different feature sets, BERT outperforms Doc2Vec as well as Binary and TF-IDF feature sets. 
%
%Among different classifiers, AdaBoost outperforms Naive Bayes and Decision Tree classifiers. 
%
%Next, we discuss these dimensions in more details. 


\textbf{Impact of feature extraction. }
Table \ref{table: impact_of_approach} summarizes the classification results for different feature extraction approaches using the equal window split. 
%
We break down the results for 4 different feature extraction approaches: Doc2Vec, TI2Vec, BERT, and TIBERT. 
%
The best average classification accuracy of 78\% is achieved by TIBERT. 
%
TIBERT turns out to be a better approach than the pre-trained BERT embeddings as well as Doc2Vec and TI2Vec embeddings. 
%
TIBERT achieves 4{\%} better F1 score than TI2Vec.%; however, Ti2Vec exhibits similar trends. 
%
As compared to TI2Vec, TIBERT further produces word representations that are context-dependent. 
%
Thus, the same word would have multiple embeddings differing by the context of the words around them whereas TI2Vec is a context-independent embedding. 
%
Thus, we expect the context-dependent TIBERT to be advantageous to the TI2Vec embeddings.
%
Overall, TI2Vec and TIBERT significantly outperform their vanilla pre-trained Doc2Vec and BERT counterparts. 
%
The improvement in accuracy can be attributed to the specialization of these embeddings on a large corpus of IoC data from many different TI feeds. 
%
By doing so, TI2Vec and TIBERT capture the context of security events in TI feeds, being able to better characterize its similarity to other security events when compared to vanilla pre-trained embeddings. 



\textbf{Impact of classifier. }
Comparing different machine learning classifiers\footnote{except for TIBERT which has a built-in classifier}, we note that AdaBoost outperforms Naive Bayes and Decision Tree. 
%
Different classifiers appear to handle the precision-recall trade-off differently. 
%
For instance, not shown in Table \ref{table: impact_of_approach}, the Decision Tree classifier is inclined to optimize for precision while the Naive Bayes classifier is inclined to optimize for recall. 
%
AdaBoost achieves the best balance between precision and recall. 
%
AdaBoost outperforms Decision Tree by 12\% for Doc2Vec, 6\% for TI2Vec, and 6\% for BERT in terms of overall F1 score.



\input{docs/results_tables/TiBERT_temporal}

\textbf{Impact of temporal splits. }
Table \ref{table: temporal_bert_results} reports F1 score for TIBERT for two types of temporal splits: equal and aggregate window. 
%
As compared to equal window splits, aggregate window splits accumulates training data over time. 
%
However, we note that the classification accuracy for aggregate window splits does not monotonically increase across splits -- it increases initially and then decreases sharply for split 4 and then improves again eventually as the size of the train set increases. 
%
The equal window split type explores the impact of equal-sized train and test sets. 
%
Note that the test sets are comparable between both split types, but aggregate window uses more training data.  
%
It is interesting to note that TIBERT achieves higher F1 scores overall for equal window splits. 
%
For split  4, the sharp drop in F1 scores is explained by the large difference in the vocabulary between train and test sets.\footnote{For split 4, the difference in vocabulary between the test and train sets was about 44,000 words. The difference was determined by computing the number of words in the test set that did not appear in the train set.} 


%%
Comparing aggregate window and equal window, we note that equal window achieves better classification performance.
%
For each split, limiting our training data to only recent events instead of aggregating it generally resulted in a higher F1 score. 
%
For instance, the equal window split average (78\%) outperformed  aggregate window split average (63\%) for TIBERT. 
%
Thus, we conclude that the limiting the training data to the most recent ultimately helps the classifier to more accurately detect exploitation events than using more training data. 


%\begin{table}[!t]
 %   \centering
  %  \scriptsize
  %% \caption{Temporal+Spatial classification accuracy results for Doc2Vec and BERT. Each value is the weighted average of F1 scores when using the AdaBoost classifier and the specified feature extraction method. Note that, although the results for the omission of {\Crimeware} are available in the Appendix, we do not consider them for analysis as our dataset only contains 5 exploitation events from \Crimeware.}
    %\label{table: temp-spatial-results}
    %\subfloat[Doc2Vec]{%
     %   \begin{tabular}{|l|l|l|l|l|l|l|l|}
      %  \hline
% &             \multicolumn{6}{c|}{Feed Omitted} \\\hline
%       Split Type      & \CERTBund & \CIRCL  &  \inThreat & \CthulhuSPRL   & \DCSO & \INCIBE  \\ \hline \hline
 %           Specific Time & 0.49 & 0.82 & 0.41 & 1 & 0.89 & Ignore \\ \hline
 %            Equal Window& 0.26 & 0.7 & 0.49 & 0.7 & 0.79 & 0.68 \\ \hline
  %          Aggregate Window & 0.36 & 0.79 & 0.55 & 0.8 & 0.82 & 0.78 \\ \hline
   %     \end{tabular}%
  %  }\vspace{0.5cm}
   % \subfloat[BERT]{%
    %    \begin{tabular}{|l|l|l|l|l|l|l|l|}
    %    \hline
% &             \multicolumn{6}{c|}{Feed Omitted} \\\hline
%       Split Type      & \CERTBund & \CIRCL  & \inThreat  & \CthulhuSPRL   & \DCSO & \INCIBE \\ \hline \hline
 %           Specific Time & 0.48 & 0.8 & 0.7 & 0.8 & 0.86 & Ignore \\ \hline
%             Equal Window& 0.27 & 0.66 & 0.69 & 0.62 & 0.77 & 0.49 \\ \hline
%             Aggregate Window& 0.35 & 0.77 & 0.76  & 0.76 & 0.86 & 0.77\\ \hline
%        \end{tabular}%
%    }
%\end{table}

\input{docs/results_tables/TiBERT_spatial}

\textbf{Impact of TI feed. }
Next, we report the accuracy results for joint temporal+spatial splits. 
%
These joint splits allow us evaluate the transferability of the classification model to an unseen TI feed. 
%
Table \ref{table: spatial_results} shows the F1 scores for the various temporal+spatial splits, grouped by the feed omitted from the train set (which is the only feed present in the test set).
%
Since valid F1 scores depend on the presence of exploit events in the test set, we further restrict analysis to temporal+spatial splits for feeds that contain at least 1 exploit event in the test set.
%
We focus our analysis on the TIBERT aggregate window approach as it yielded the highest F1 scores.
%
We observe a strong correlation between the findings of Figure \ref{figure:sankey} and Table \ref{table: spatial_results}. 
%
We note that the feeds with IoCs that are mostly ``sinks" also have higher average F1 scores when that feed is omitted in the temporal+spatial splits.
%
%This tends to hold across both equal and aggregate window split types. 
%
For example, Table \ref{table: spatial_results} shows that the omission of {\DCSO} yields a high F1 score (89\%). 
%
{\DCSO} also notably has the most number of Hash and IP IoCs (2088) that are sinks of IoCs from other feeds in the dataset. 
%
Likewise, the omission of {\CIRCL}, which has the second highest number of sink Hash and IP IoCs (1095), yields F1 scores that are in the top 4 highest scores for aggregate window split.


%%
In the same vein, the omission of {\CERTBund} yields a relatively low F1 score (45\%). While   {\CERTBund} has high IoC overlap with other feeds,  % (see~\cite{supplementarymaterial}), 
Figure \ref{figure:sankey} shows that the majority ($\approx$ 85\%) of \CERTBund's IoC overlap occurs when it is a source and not a sink. 
%%
Exceptions to these general findings do exist, however. 
%
For example, as Figure~\ref{figure:sankey} shows, {\CthulhuSPRL}  is more often a source than a sink, yet its omission yields a high F1 score (92\%). 
%
This may indicate that {\CthulhuSPRL}  shares many similar IoCs with other feeds, despite not having an abundance of exact IoC overlap.


%%
Overall, these findings indicate that our model's ability to detect exploitation events in TI feeds it has not been introduced to yet is dependent on the relationship between the IoCs of the training and testing data. 
%
High accuracy exploitation detection is possible under spatial restrictions if the training data has same/similar IoCs as those present in the testing feed. 
%Otherwise, results may be mediocre at best.

\input{docs/results_tables/TiBERT_feature_ablation}

\textbf{TIBERT feature ablation analysis. } 
We conduct feature ablation analysis to assess the relative contribution of different IoC categories.
%
The classification accuracy, as measured using the F1 score,  for top three IoC categories, 
 equals 40\%, 39\% and 66\% for network activity, payload delivery, and external analysis, respectively. Across all categories, accuracy equals 78\%. 
%
We note that classification accuracy for network activity IoCs is better than both payload delivery and external analysis. 
%
The results are inline with the earlier finding that our TI feed dataset contains the most network activity IoCs (557,532), followed by payload delivery (220,321), and then external analysis (38,531). 
%
Overall, all IoCs of different categories instead of just one, such as network activity, yields the best classification accuracy (78\% vs 66\%).
%
Thus, we conclude that while some IoC categories are more helpful than others, they complement each other and using them together outperforms standalone classification performance. 

\textbf{Applications of TIBERT. }
The exploitation events predicted by TIBERT can be utilized to update the temporal exploitability score of CVSS/EPSS related to the availability of PoC  or fully functional exploits. 
%In particular, the Exploit Code Maturity and Report Confidence. 
We focus specifically on temporal metrics since TIBERT generates predictions based on the past history of a event. The \textit{Exploit Code Maturity} metric describes the maturity level of an exploit. The output of TIBERT can be used to automatically revise this metric, such as updating it from ``Proof of concept code'' to ``Functional exploit exists''. 
%Similarly, the Report Confidence metric describes if a vulnerability is real and exploitable. 
%TIBERT could also automatically increase or decrease this metric such as upgrading it from ``Unknown'' to  ``Reasonable''. 
By temporally analyzing large volumes of loosely structured TI feed data, TIBERT provides a way to automatically improve CVSS/EPSS score quality, saving time and effort of security experts. 


As the accuracy score of TIBERT is 0.78 on average, we acknowledge that false positives and false negatives can impact security operations. 
A false positive exploitation %vulnerability %
can untimely escalate patching, causing transient unplanned system unavailability  and could increase costs. This leads to the misprioritization of vulnerabilities. 
On the other hand, a false negative exploitation could cause security experts to not identify the exploit altogether, leaving the software susceptible to attacks. 
However, since one of the goals of TIBERT is to update CVSS and EPSS scores, and not replace them, these risks are present, but to a lesser degree.  % Note that TIBERT's false positive rate (1\%) is configured to be half that of its false negative rate (2\%). 
%It is also noteworthy that since there are 2 other categories and 19 additional metrics, inaccurate Exploit Code Maturity and Report Confidence metrics within the temporal category does not yield a significant impact on the overall EPSS/CVSS score of the vulnerability. 
Thus, we argue that TIBERT is a useful approach to automatically updating CVSS/EPSS scores with minimal risks on security operations despite its less than perfect accuracy.


%{we want to communicate that false negatives are worse than false positives; add data point reporting our false positive (1\% on avg for TIBERT) vs. false negatives (2\% on avg for TIBERT)}
%
%\hl{take a pass}


\begin{comment}
\subsection{Decision Tree}
\begin{figure}
    \centering
    \includegraphics[width=0.5\columnwidth]{docs/figures/decision_trees/tree_tifeeds(3)(7).png}
    \caption{}
    \label{fig:decisiontree}
\end{figure}
\end{comment}
 
  \textbf{Visualization. } 
  \label{sec:visual}
Figure~\ref{fig:bertdoc2vec} illustrates  Doc2Vec and TI2Vec embeddings.  
%
Using TSNE, we are able to visualize how the embeddings produced by Doc2Vec and TI2Vec spread over the plane.  
%
Each point corresponds to an event.  
%
Green and red points  correspond to non-exploitation and exploitation events, respectively.  
%
Whereas both Doc2Vec and TI2Vec produced two clearly distinguishable clusters, the clusters produced by TI2Vec are  easier to separate using a simple decision tree.
%
%Such additional complexity, in turn, simplifies the classification task.  
%
A simple decision tree, with two levels, is already able to classify the events with a {55\% and 66\% F1-score using Doc2Vec and TI2Vec, respectively.  
%
Those numbers are in agreement with } Table~\ref{table: impact_of_approach}, noting that the average F1-scores of 58\% and 68\% reported in Table~\ref{table: impact_of_approach} {for Doc2Vec and TI2Vec were obtained with  deeper decision trees and the original embeddings. 
%
As expected, using shallow decision trees and the simplified embeddings perturbed by TSNE caused a slight decrease in performance. 
%
It is also worth noting that the accuracy of all considered variations remained roughly 84\%. }


\begin{figure}
    \centering
    \begin{subfigure}[b]{0.47\columnwidth}
        \includegraphics[width=1\columnwidth]{docs/figures/2d_embeddings_plots/doc2vec_plot_Decision Tree.png}
        \caption{Doc2Vec}
     \end{subfigure}
     \begin{subfigure}[b]{0.47\columnwidth}
      \includegraphics[width=1\columnwidth]{docs/figures/2d_embeddings_plots/ti2vec_plot_Decision Tree.png}
      \caption{TI2Vec}
    \end{subfigure}
     \caption{Embeddings   input into a decision tree classifier} % : both embeddings allow for accurate classification, with TI2Vec being roughly 10\% superior in terms of F1 score.} 
     \label{fig:bertdoc2vec}\vspace{-0.2in}
\end{figure}



==> docs/table_rules.tex <==

  \\ 
\hline
(malware\_classification:malware-category="ransomware")+(circl:incident-classification="malware")                                                                                 & 2                                            & 0.70                                  & 2.49  
                                     
\hline
(circl:incident-classification="malware")+(malware\_classification:malware-category="trojan")                                                                                     & 2                                            & 0.68                                  & 2.45                                                          \\ 
\hline
(type:osint)+(ecsirt:malicious-code="ransomware")+(malware\_classification:malware-category="ransomware")                                                                         & 3                                            & 0.67                                  & 2.38                                                          \\ 
\hline
(circl:incident-classification="system-compromise")+(malware\_classification:malware-category="trojan")                                                                           & 2                                            & 0.67                                  & 2.38                                                          \\ 
\hline
(type:osint)+(ecsirt:malicious-code="ransomware")+(malware\_classification:malware-category="ransomware")+(circl:incident-classification="malware")                               & 4                                            & 0.67                                  & 2.38                                                          \\ 
\hline
(cybercrime)+(kill-chain:installation)+(kill-chain:delivery)+(kill-chain:command and control)                                                                                     & 4                                            & 0.67                                  & 2.38                                                          \\ 
\hline
(type:osint)+(circl:topic="finance")+(circl:incident-classification="malware")                                                                                                    & 3                                            & 0.67                                  & 2.38                                                          \\ 
\hline
(type:osint)+(ecsirt:malicious-code="ransomware")+(circl:incident-classification="malware")                                                                                       & 3                                            & 0.67                                  & 2.38                                                          \\ 
\hline
(veris:action:malware:variety="ransomware")+(malware\_classification:malware-category="ransomware")+(dnc:malware-type="ransomware")                                               & 3                                            & 0.67                                  & 2.38                                                          \\ 
\hline
(malware\_classification:malware-category="ransomware")+(enisa:nefarious-activity-abuse="ransomware")+(dnc:malware-type="ransomware")                                             & 3                                            & 0.67                                  & 2.38                                                          \\ 
\hline
(trj=doublepulsar)+(malware\_classification:malware-category="ransomware")+(phishing)                                                                                             & 3                                            & 0.67                                  & 2.38                                                          \\ 
\hline
(cybercrime)+(kill-chain:installation)+(kill-chain:command and control)                                                                                                           & 3                                            & 0.67                                  & 2.38                                                          \\ 
\hline
(cybercrime)+(kill-chain:delivery)+(kill-chain:command and control)                                                                                                               & 3                                            & 0.67                                  & 2.38                                                          \\ 
\hline
(apt)+(ncsc-nl-nds:search="historic")                                                                                                                                             & 2                                            & 0.67                                  & 2.38                                                          \\ 
\hline
(ms-caro-malware-full:malware-family="banker")+(malware\_classification:malware-category="trojan")                                                                                & 2                                            & 0.67                                  & 2.38                                                          \\ 
\hline
(ransomware)+(malware\_classification:malware-category="ransomware")                                                                                                              & 2                                            & 0.67                                  & 2.38                                                          \\ 
\hline
(ncsc-nl-ndn:feed="generic")+(malware\_classification:malware-category="ransomware")                                                                                              & 2                                            & 0.67                                  & 2.38                                                          \\ 
\hline
(relcircl)+(malware)                                                                                                                                                              & 2                                            & 0.67                                  & 2.38                                                          \\ 
\hline
(circl:incident-classification="vulnerability")+(malware\_classification:malware-category="trojan")                                                                               & 2                                            & 0.67                                  & 2.38                                                          \\ 
\hline
(malspam)+(emotet)                                                                                                                                                                & 2                                            & 0.67                                  & 2.38                                                          \\ 
\hline
(cybercrime)+(kill-chain:command and control)                                                                                                                                     & 2                                            & 0.67                                  & 2.38                                                          \\ 
\hline
(malspam)+(danabot)                                                                                                                                                               & 2                                            & 0.67                                  & 2.38                                                          \\ 
\hline
(veris:action:malware:variety="ransomware")+(dnc:malware-type="ransomware")                                                                                                       & 2                                            & 0.67                                  & 2.38                                                          \\ 
\hline
(enisa:nefarious-activity-abuse="ransomware")+(dnc:malware-type="ransomware")                                                                                                     & 2                                            & 0.67                                  & 2.38                                                          \\ 
\hline
(threat type:rat)+(enisa:nefarious-activity-abuse="remote-access-tool")                                                                                                           & 2                                            & 0.67                                  & 2.38                                                          \\ 
\hline
(circl:incident-classification="phishing")+(circl:topic="finance")                                                                                                                & 2                                            & 0.67                                  & 2.38                                                          \\ 
\hline
(certsi:critical-sector="government")+(malware\_classification:malware-category="trojan")                                                                                         & 2                                            & 0.67                                  & 2.38                                                          \\ 
\hline
(circl:incident-classification="spam")+(circl:incident-classification="malware")                                                                                                  & 2                                            & 0.67                                  & 2.38                                                          \\ 
\hline
(emotet)+(circl:incident-classification="malware")                                                                                                                                & 2                                            & 0.67                                  & 2.38                                                          \\ 
\hline
(trj=doublepulsar)+(phishing)                                                                                                                                                     & 2                                            & 0.67                                  & 2.38                                                          \\ 
\hline
(circl:incident-classification="malware")+(malware\_classification:malware-category="worm")                                                                                       & 2                                            & 0.67                                  & 2.38                                                          \\ 
\hline
(circl:topic="industry")                                                                                                                                                          & 1                                            & 0.67                                  & 2.29                                                          \\ 
\hline
(ecsirt:fraud="phishing")                                                                                                                                                         & 1                                            & 0.67                                  & 2.29                                                          \\ 
\hline
(certsi:critical-sector="government")                                                                                                                                             & 1                                            & 0.67                                  & 2.29                                                          \\ 
\hline
(ms-caro-malware:malware-platform="win32")                                                                                                                                        & 1                                            & 0.67                                  & 2.29                                                          \\ 
\hline
(trickbot)                                                                                                                                                                        & 1                                            & 0.67                                  & 2.29                                                          \\ 
\hline
(ms-caro-malware:malware-type="trojan")                                                                                                                                           & 1                                            & 0.67                                  & 2.29                                                          \\ 
\hline
(ecsirt:intrusion-attempts="exploit")                                                                                                                                             & 1                                            & 0.67                                  & 2.29                                                          \\ 
\hline
(threat type:apt)                                                                                                                                                                 & 1                                            & 0.67                                  & 2.29                                                          \\ 
\hline
(locky)                                                                                                                                                                           & 1                                            & 0.67                                  & 2.29                                                          \\ 
\hline
(netwire rat)                                                                                                                                                                     & 1                                            & 0.67                                  & 2.29                                                          \\ 
\hline
(ncsc-nl-ndn:feed="generic")                                                                                                                                                      & 1                                            & 0.64                                  & 2.21                                                          \\ 
\hline
(circl:incident-classification="spam")+(malware\_classification:malware-category="ransomware")                                                                                    & 2                                            & 0.64                                  & 2.28                                                          \\ 
\hline
(estimative-language:likelihood-probability="very-likely")                                                                                                                        & 1                                            & 0.64                                  & 2.18                                                          \\ 
\hline
(kill-chain:installation)                                                                                                                                                         & 1                                            & 0.63                                  & 2.17                                                          \\ 
\hline
(malware\_classification:malware-category="trojan")                                                                                                                               & 1                                            & 0.63                                  & 2.15                                                          \\ 
\hline
(veris:confidence="none")+(type:osint)+(cssa:origin="other")+(cssa:sharing-class="tier-0")                                                                                        & 4                                            & 0.63                                  & 2.23                                                          \\ 
\hline
(veris:confidence="none")+(type:osint)+(cssa:origin="other")                                                                                                                      & 3                                            & 0.63                                  & 2.23                                                          \\ 
\hline
(type:osint)+(veris:confidence="none")+(cssa:sharing-class="tier-0")                                                                                                              & 3                                            & 0.63                                  & 2.23                                                          \\ 
\hline
(type:osint)+(cssa:origin="other")+(cssa:sharing-class="tier-0")                                                                                                                  & 3                                            & 0.63                                  & 2.23                                                          \\ 
\hline
(type:osint)+(veris:confidence="none")                                                                                                                                            & 2                                            & 0.63                                  & 2.23                                                          \\ 
\hline
(type:osint)+(cssa:sharing-class="tier-0")                                                                                                                                        & 2                                            & 0.63                                  & 2.23                                                          \\ 
\hline
(type:osint)+(cssa:origin="other")                                                                                                                                                & 2                                            & 0.63                                  & 2.23                                                          \\ 
\hline
(malware)+(\inThreat:event-src="feed-essential")                                                                                                                                   & 2                                            & 0.63                                  & 2.23                                                          \\ 
\hline
(dnc:malware-type="ransomware")                                                                                                                                                   & 1                                            & 0.63                                  & 2.14                                                          \\ 
\hline
(osint:source-type="blog-post")                                                                                                                                                   & 1                                            & 0.61                                  & 2.09                                                          \\ 
\hline
(circl:incident-classification="malware")                                                                                                                                         & 1                                            & 0.61                                  & 2.09                                                          \\ 
\hline
(enisa:nefarious-activity-abuse="mobile-malware")                                                                                                                                 & 1                                            & 0.60                                  & 2.06                                                          \\ 
\hline
(dnc:malware-type="coinminer")                                                                                                                                                    & 1                                            & 0.60                                  & 2.06                                                          \\ 
\hline
(cybercrime)+(malware)+(inthreat.com:event-src="feed-essential")                                                                                                                      & 3                                            & 0.60                                  & 2.15                                                          \\ 
\hline
(type:osint)+(malware\_classification:malware-category="ransomware")+(circl:incident-classification="malware")                                                                    & 3                                            & 0.60                                  & 2.15                                                          \\ 
\hline
(malware\_classification:malware-category="spyware")+(circl:incident-classification="malware")                                                                                    & 2                                            & 0.60                                  & 2.15                                                          \\ 
\hline
(cybercrime)+(kill-chain:installation)                                                                                                                                            & 2                                            & 0.60                                  & 2.15                                                          \\ 
\hline
(veris:action:social:target="finance")                                                                                                                                            & 1                                            & 0.60                                  & 2.06                                                          \\ 
\hline
(estimative-language:likelihood-probability="likely")                                                                                                                             & 1                                            & 0.60                                  & 2.06                                                          \\ 
\hline
(circl:incident-classification="phishing")                                                                                                                                        & 1                                            & 0.59                                  & 2.03                                                          \\ 
\hline
(phishing)                                                                                                                                                                        & 1                                            & 0.57                                  & 1.96                                                          \\ 
\hline
(kill-chain:installation)+(kill-chain:command and control)                                                                                                                        & 2                                            & 0.57                                  & 2.04                                                          \\ 
\hline
(circl:incident-classification="phishing")+(malware\_classification:malware-category="ransomware")                                                                                & 2                                            & 0.57                                  & 2.04                                                          \\ 
\hline
(apt)+(threat:sofacy/apt28)                                                                                                                                                       & 2                                            & 0.57                                  & 2.04                                                          \\ 
\hline
(malware\_classification:malware-category="ransomware")+(dnc:malware-type="ransomware")                                                                                           & 2                                            & 0.57                                  & 2.04                                                          \\ 
\hline
(kill-chain:command and control)                                                                                                                                                  & 1                                            & 0.56                                  & 1.93                                                          \\ 
\hline
(cert-bund\_bsi:sharing="int. cert community")                                                                                                                                    & 1                                            & 0.56                                  & 1.92                                                          \\ 
\hline
(type:osint)                                                                                                                                                                      & 1                                            & 0.56                                  & 1.91                                                          \\ 
\hline
(kill-chain:installation)+(kill-chain:delivery)+(kill-chain:command and control)                                                                                                  & 3                                            & 0.56                                  & 1.99                                                          \\ 
\hline
(ecsirt:malicious-code="ransomware")+(malware\_classification:malware-category="ransomware")+(circl:incident-classification="malware")                                            & 3                                            & 0.56                                  & 1.99                                                          \\ 
\hline
(kill-chain:delivery)+(kill-chain:command and control)                                                                                                                            & 2                                            & 0.56                                  & 1.99                                                          \\ 
\hline
(malspam)+(circl:incident-classification="malware")                                                                                                                               & 2                                            & 0.56                                  & 1.99                                                          \\ 
\hline
(osint:source-type="microblog-post")                                                                                                                                              & 1                                            & 0.56                                  & 1.91                                                          \\ 
\hline
(type:osint)+(circl:incident-classification="malware")                                                                                                                            & 2                                            & 0.55                                  & 1.97                                                          \\ 
\hline
(kill-chain:delivery)+(kill-chain:installation)                                                                                                                                   & 2                                            & 0.55                                  & 1.95                                                          \\ 
\hline
(kill-chain:delivery)                                                                                                                                                             & 1                                            & 0.55                                  & 1.87                                                          \\ 
\hline
(circl:incident-classification="vulnerability")                                                                                                                                   & 1                                            & 0.53                                  & 1.82                                                          \\ 
\hline
(ecsirt:malicious-code="malware")                                                                                                                                                 & 1                                            & 0.52                                  & 1.79                                                          \\ 
\hline
(malspam)                                                                                                                                                                         & 1                                            & 0.52                                  & 1.77                                                          \\ 
\hline
(apt)                                                                                                                                                                             & 1                                            & 0.50                                  & 1.72                                                          \\ 
\hline
(ncsc-nl-ndn:feed="selected")                                                                                                                                                     & 1                                            & 0.50                                  & 1.72                                                          \\ 
\hline
(ms-caro-malware:malware-platform="linux")                                                                                                                                        & 1                                            & 0.50                                  & 1.72                                                          \\ 
\hline
(banker)                                                                                                                                                                          & 1                                            & 0.50                                  & 1.72                                                          \\ 
\hline
(malware\_classification:malware-category="downloader")                                                                                                                           & 1                                            & 0.50                                  & 1.72                                                          \\ 
\hline
(malspam)+(malware\_classification:malware-category="ransomware")+(circl:incident-classification="malware")                                                                       & 3                                            & 0.50                                  & 1.79                                                          \\ 
\hline
(ms-caro-malware-full:malware-family="banker")                                                                                                                                    & 1                                            & 0.50                                  & 1.72                                                          \\ 
\hline
(nymaim)                                                                                                                                                                          & 1                                            & 0.50                                  & 1.72                                                          \\ 
\hline
(circl:incident-classification="system-compromise")+(circl:incident-classification="malware")                                                                                     & 2                                            & 0.50                                  & 1.79                                                          \\ 
\hline
(osint)+(type:osint)                                                                                                                                                              & 2                                            & 0.50                                  & 1.79                                                          \\ 
\hline
(apt)+(inthreat.com:event-src="feed-essential")                                                                                                                                       & 2                                            & 0.50                                  & 1.79                                                          \\ 
\hline
(malware:pony)                                                                                                                                                                    & 1                                            & 0.50                                  & 1.72                                                          \\ 
\hline
(malware\_classification:malware-category="worm")                                                                                                                                 & 1                                            & 0.50                                  & 1.72                                                          \\ 
\hline
(ransomware)                                                                                                                                                                      & 1                                            & 0.50                                  & 1.72                                                          \\ 
\hline
(cybercrime)+(kill-chain:delivery)+(kill-chain:installation)                                                                                                                      & 3                                            & 0.50                                  & 1.79                                                          \\ 
\hline
(cybercrime)+(kill-chain:delivery)                                                                                                                                                & 2                                            & 0.50                                  & 1.79                                                          \\ 
\hline
(type:osint)+(intelmq:done)                                                                                                                                                       & 2                                            & 0.50                                  & 1.79                                                          \\ 
\hline
(ncsc-nl-nds:search="historic")+(ncsc-nl-ndn:feed="generic")                                                                                                                      & 2                                            & 0.50                                  & 1.79                                                          \\ 
\hline
(trj=doublepulsar)+(malware\_classification:malware-category="ransomware")                                                                                                        & 2                                            & 0.50                                  & 1.79                                                          \\ 
\hline
(malware\_classification:malware-category="ransomware")+(malware\_classification:malware-category="trojan")                                                                       & 2                                            & 0.50                                  & 1.79                                                          \\ 
\hline
(emotet)+(banker)                                                                                                                                                                 & 2                                            & 0.50                                  & 1.79                                                          \\ 
\hline
(intelmq:done)                                                                                                                                                                    & 1                                            & 0.50                                  & 1.72                                                          \\ 
\hline
(osint:certainty="75")                                                                                                                                                            & 1                                            & 0.50                                  & 1.72                                                          \\ 
\hline
(ecsirt:intrusions="compromised")                                                                                                                                                 & 1                                            & 0.50                                  & 1.72                                                          \\ 
\hline
(ecsirt:intrusions="backdoor")                                                                                                                                                    & 1                                            & 0.50                                  & 1.72                                                          \\ 
\hline
(trj=doublepulsar)                                                                                                                                                                & 1                                            & 0.50                                  & 1.72                                                          \\ 
\hline
(veris:action:malware:variety="ransomware")+(ecsirt:malicious-code="ransomware")+(malware\_classification:malware-category="ransomware")+(dnc:malware-type="ransomware")          & 4                                            & 0.50                                  & 1.79                                                          \\ 
\hline
(veris:action:malware:variety="ransomware")+(malware\_classification:malware-category="ransomware")+(enisa:nefarious-activity-abuse="ransomware")+(dnc:malware-type="ransomware") & 4                                            & 0.50                                  & 1.79                                                          \\ 
\hline
(type:osint)+(ecsirt:malicious-code="ransomware")+(malware\_classification:malware-category="ransomware")+(ms-caro-malware:malware-type="ransom")                                 & 4                                            & 0.50                                  & 1.79                                                          \\ 
\hline
(veris:action:malware:variety="ransomware")+(ecsirt:malicious-code="ransomware")+(enisa:nefarious-activity-abuse="ransomware")+(dnc:malware-type="ransomware")                    & 4                                            & 0.50                                  & 1.79                                                          \\ 
\hline
(ecsirt:malicious-code="ransomware")+(malware\_classification:malware-category="ransomware")+(enisa:nefarious-activity-abuse="ransomware")+(dnc:malware-type="ransomware")        & 4                                            & 0.50                                  & 1.79                                                          \\ 
\hline
(cybercrime)+(malware)+(inthreat.com:enrichment="manual")+(inthreat.com:event-src="feed-essential")                                                                                       & 4                                            & 0.50                                  & 1.79                                                          \\ 
\hline
(type:osint)+(ecsirt:malicious-code="ransomware")+(ms-caro-malware:malware-type="ransom")                                                                                         & 3                                            & 0.50                                  & 1.79                                                          \\ 
\hline
(circl:incident-classification="system-compromise")+(circl:incident-classification="malware")+(malware\_classification:malware-category="trojan")                                 & 3                                            & 0.50                                  & 1.79                                                          \\ 
\hline
(cybercrime)+(inthreat.com:enrichment="manual")+(malware)                                                                                                                             & 3                                            & 0.50                                  & 1.79                                                          \\ 
\hline
(ecsirt:malicious-code="ransomware")+(enisa:nefarious-activity-abuse="ransomware")+(dnc:malware-type="ransomware")                                                                & 3                                            & 0.50                                  & 1.79                                                          \\ 
\hline
(emotet)+(cert-bund\_bsi:sharing="int. cert community")+(circl:incident-classification="malware")                                                                                 & 3                                            & 0.50                                  & 1.79                                                          \\ 
\hline
(malware)+(apt)+(inthreat.com:event-src="feed-essential")                                                                                                                             & 3                                            & 0.50                                  & 1.79                                                          \\ 
\hline
(circl:incident-classification="phishing")+(certsi:critical-sector="government")+(malware\_classification:malware-category="trojan")                                              & 3                                            & 0.50                                  & 1.79                                                          \\ 
\hline
(ecsirt:malicious-code="ransomware")+(malware\_classification:malware-category="ransomware")+(dnc:malware-type="ransomware")                                                      & 3                                            & 0.50                                  & 1.79                                                          \\ 
\hline
(veris:action:malware:variety="ransomware")+(ecsirt:malicious-code="ransomware")+(dnc:malware-type="ransomware")                                                                  & 3                                            & 0.50                                  & 1.79                                                          \\ 
\hline
(veris:action:malware:variety="ransomware")+(enisa:nefarious-activity-abuse="ransomware")+(dnc:malware-type="ransomware")                                                         & 3                                            & 0.50                                  & 1.79                                                          \\ 
\hline
(ms-caro-malware-full:malware-family="banker")+(type:osint)+(malware\_classification:malware-category="trojan")                                                                   & 3                                            & 0.50                                  & 1.79                                                          \\ 
\hline
(type:osint)+(malware\_classification:malware-category="ransomware")+(ms-caro-malware:malware-type="ransom")                                                                      & 3                                            & 0.50                                  & 1.79                                                          \\ 
\hline
(malware)+(inthreat.com:enrichment="manual")+(inthreat.com:event-src="feed-essential")                                                                                                    & 3                                            & 0.50                                  & 1.79                                                          \\ 
\hline
(malspam)+(nymaim)+(malware)                                                                                                                                                      & 3                                            & 0.50                                  & 1.79                                                          \\ 
\hline
(malspam)+(type:osint)+(malware\_classification:malware-category="ransomware")                                                                                                    & 3                                            & 0.50                                  & 1.79                                      \end{comment}      
